Code2API: A Tool for Generating Reusable APIs from Stack Overflow Code Snippets

Nowadays, developers often turn to Stack Overflow for solutions to daily problems, however, these code snippets are partial code that cannot be tested and verified properly. One way to test these code snippets is to transform them into APIs (Application Program Interface) that developers can be directly invoked and executed. However, it is often costly and error-prone for developers to manually perform this transformation (referred to as AIPzation task) due to different actions to be taken (e.g., summarizing proper method names, inferring input parameters list and return statements). To help developers quickly reuse code snippets in Stack Overflow, in this paper, we propose Code2API, a Google Chrome extension that uses Large Language Models (LLMs) to automatically perform APIzation of code snippets on Stack Overflow. \toolname guides LLMs through well-designed prompts to generate reusable APIs, using Chain-of-Thought reasoning and few-shot in-context learning to help LLMs understand and solve the APIzation task in a developer-like manner. The evaluation results show that Code2API significantly outperforms the rule-based approach by a large margin.

==> background.tex <==

In this section, we will introduce the background of the our approach, including large language models, in-context learning, and chain-of-thought prompting.

\subsection{Large Language Models}
Large Language Models (LLMs) are a form of artificial intelligence model that contain billions of parameters and are trained on extensive text data. These models are generally categorized into two types: base LLMs and instruction-tuned LLMs. The most prevalent type of base LLMs is the transformer-based model, including models like GPT-3 developed by OpenAI. These models are designed to comprehend and generate human-like text based on the input they receive. They possess the capability to understand context, generate creative content, and even demonstrate a level of common sense reasoning, making them a powerful tool in natural language processing tasks.

Despite the impressive capabilities of large language models, they often require fine-tuning to perform specific tasks effectively. This is where instruction-tuned LLMs come into play. Instruction-tuned LLMs are trained not only on a large corpus of text but also on specific instructions, also known as prompts, to guide their output. They use  instruction-formatted instances to fine-tune base LLMs in the way of supervised learning. These instances include tasks such as summarizing text, translating it into another language, or answering questions about it. After fine-tuning, instruction-tuned LLMs can perform these tasks more efficiently. 
Instruction-tuned large language models can be more versatile and adaptable than base LLMs. They can be utilized in a broader range of applications, as they can be tuned to perform specific tasks based on the prompts they are given. This makes them an invaluable tool in fields like customer service, content creation, and data analysis, where specific, task-oriented outputs are necessary. 
An example of using one of the best instruction-tuned LLMs, ChatGPT, to complete the Java code generation task is illustrated in Figure \ref{fig:chatgpt_demo}. As can be seen, it is user-friendly and allows the use of natural language as the prompt to interact with it and guide it to complete various tasks.

% Large Language Models (LLMs) refer to Transformer language models that contain hundreds of billions (or more) of parameters trained on large amounts of textual data, such as GPT-3, PaLM, GPT3.5, LLaMA. They are typically divided into two categories: base LLMs and instruction-tuned LLMs.
% Base LLMs are usually trained only on large-scale text data in self-supervised learning, and they can handle common Natural language processing tasks. In order to further enhance the capabilities of base LLMs, instruction-tuned LLMs have been proposed. They use instruction-formatted instances to fine-tune base LLMs in supervised learning. After fine-tuning, they can perform a wide range of tasks and provide more accurate and detailed responses based on the instructions(also known as prompts) given. Figure \ref{fig:chatgpt_demo} is an example of using one of the best instruction-tuned LLMs ChatGPT to complete the Java code generation task. As we can see, it is easy to use and we can use natural language as prompts to talk with it and guide it to help us complete various tasks.


\subsection{Few-shot prompting}
Few-shot prompting, also known as in-context learning, is a concept that has gained significant attention in the field of machine learning, particularly in the context of natural language processing (NLP) and deep learning. The term "few-shot" refers to the ability of a model to understand and perform a task after being exposed to only a few examples. This is in contrast to traditional machine learning models that require large amounts of training data to learn a task.

Few-shot prompting has been made possible by recent advances in transformer-based language models, such as GPT-3 developed by OpenAI. These models are pre-trained on a large corpus of text data and can generate human-like text based on a given prompt. The approach involves supplying the model with a prompt that includes a task description and a few task examples, and the model then generates a response based on the prompt. It is particularly effective for tasks that require the model to infer complex patterns or relationships from the input and output data.
Figure \ref{fig:back_demo1} illustrates an instance of few-shot prompting, which uses an example in the prompt to help the model understand the task of calculating the area of a circle.

% In-context learning introduced by GPT-3 is a key feature of large language models. Unlike traditional machine learning models that are trained and then fixed, in-context learning allows the model to adapt its responses based on the context provided during the interaction without additional training. It is particularly effective for tasks that require the model to infer complex patterns or relationships from the input data. In large language models, the context is usually a prompt that contains a task description and a few task examples as demonstrations, hence it is also known as few-shot prompting. In-context learning can help the LLMs quickly understand the task through demonstrations, which allows them to generate more relevant and accurate responses. \ref{fig:back_demo1} is an example of few-shot prompt, which uses an example in the prompt to help the model understand the task of calculating the area of a circle.


\subsection{Chain-of-thought prompting}
% Chain-of-thought prompting is a technique used to guide a language model to generate desired outputs by providing it with a sequence of prompts that mimic a logical thought process. This technique is particularly effective for tasks that require the model to generate outputs that are logically consistent and coherent.
LLMs have demonstrated remarkable capabilities in generating human-like text, understanding context, and even exhibiting creativity. One of the key techniques that have contributed to the success of these models is the concept of chain-of-thought prompting.

Chain-of-thought prompting is a method of interacting with language models that involves providing a series of prompts that guide the model's responses. This technique is based on the idea that large language models can maintain a "chain-of -thought" across multiple prompts, allowing them to generate intermediate inference steps for complex tasks such as commonsense reasoning questions. The use of chain-of-thought prompting has opened up new possibilities for the application of large language models. It has been used to create more interactive and engaging chatbots, to generate more coherent and contextually relevant text, and to explore more complex forms of reasoning and problem-solving. 
\ref{fig:back_demo1} is an example of chain-of-thought prompting, which uses the formula for the area of a circle in the prompt to help the model generate intermediate inference steps for calculating the area of a circle.

% This technique is based on the idea that large language models can maintain a "chain of thought" across multiple prompt, this sentence can be deleted.

%Chain-of-thought prompting is also a technique used in large language models to generate intermediate inference steps for complex tasks such as commonsense reasoning questions. The chain-of-thought is established by providing the model a prompt with a series of steps that are linked together. \ref{fig:back_demo1} is an example of chain-of-thought prompt, which uses the formula for the area of a circle in the prompt to help the model generate intermediate inference steps for calculating the area of a circle.

==> data.tex <==
We present the details of our data collection and construction process.
We build our dataset by collecting data from the top 10,000 repositories (ordered by the number of stars) in Github for Python and Java repositories.
To the best of our knowledge, this is the first and by far the largest dataset for collecting TODO comments from Github repositories. 

\subsection{Data Collection}
\subsubsection{Identifying TODO Related Commits}
We first clone the top 10,000 repositories from Github.
The git repository stores software update history, each update comprises a commit message alongside a \texttt{diff} that represents the differences between the current and previous version of the affected files. 
For each cloned repository, we first checkout all the commits from the repository history. 
Following that, for each commit, if ``TODO'' appears within the \texttt{diff}, we consider this commit as a \emph{TODO related commit}. 
We have identified more than 410K TODO related commits from our Python repositories and more than 350K commits from our Java repositories. 

\subsubsection{Normalize Diff and Commit Message}
This step aims to normalize the commit sequence and remove some semantic-irrelevant information.
After identifying the TODO related commits, we extract the \texttt{diff} and the commit message from the commits and normalize them for later use. 
For the \texttt{diff}, we convert it into lowercase and delete the \texttt{diff} header by using regular expressions. 
Commit IDs within the \texttt{diff} are replaced with ``$\langle$commit\_id$\rangle$'' and commits with a \texttt{diff} larger than 1MB are removed. 
For the commit message, we first lowercase the commit message and retain the first sentences of the \emph{commit message} as the target, since the first sentences are usually the summaries of the entire commit message~\cite{gu2016deep, jiang2017automatically}.
Similar to \texttt{diff} normalization, Github issue IDs and commit IDs are replaced by ``$\langle$issue\_id$\rangle$'' and ``$\langle$commit\_id$\rangle$'' respectively to ensure semantic integrity.
The two examples in Fig.~\ref{fig:data_pre_example} demonstrates the process of normalization.

\subsubsection{Extract TODO Comments} 
This step is responsible for extracting TODO comments from the corresponding \texttt{diff}.  
A \texttt{diff} may contain multiple TODOs. We remove such instances because they are likely to be comment updates which might introduce noise for the later data construction process. 
Hereafter, each \texttt{diff} contains a single TODO comment and pairs with a commit message.  
We then use regular expressions to locate comments within the \texttt{diff} -- if ``TODO'' appears in the comment, then this comment is identified as a TODO comment. 
The TODO comment is extracted out of the \texttt{diff} as \textit{todo\_comment}, and the rest of the \texttt{diff} stay the same, referred to as \emph{code\_change} in this paper. 
It is worth mentioning that the difference label, i.e., ``+'' and ``-'', are deleted from the TODO comment, otherwise our model can learn directly from the difference labels instead of learning the semantics of the TODO comments. 
Until now, we are able to establish $\langle code\_change, todo\_comment, commit\_msg \rangle$ triples. 
% Finally, we have obtained more than \cite{} triples for Python and more than \cite{} triples for Java. 

\begin{figure}
\vspace{0.0cm}
\centerline{\includegraphics[width=0.50\textwidth]{label-example.pdf}}
\vspace*{-0pt}
\caption{Data Preparation Examples}
\label{fig:data_pre_example}
% \vspace{-5pt}
\end{figure}


\subsection{Data Construction}
% We preprocessed the above \cite{} as follows:
\subsubsection{Data Labelling.}
\label{sec:data_label}
In this work, we consider a \texttt{diff} consists of three parts: \textit{LinesAdded}, \textit{LinesRemoved}, and \textit{LinesEqual}. 
\textit{LinesAdded} are the lines that were added to the current version when compared to its previous version. 
Similarly, \textit{LinesRemoved} are the lines that were removed from the current version when compared to its previous version.  \textit{LinesEqual} were the lines that remained unchanged between two versions. 
We automatically label each $\langle code\_change, \\ todo\_comment, commit\_msg \rangle$ triple as follows: 
(i) if \emph{todo\_comment} is within the scope of the \textit{LinesRemoved}, which means the TODO task is already performed by the developer, we label such triple instances as \textbf{Positive Samples}. 
(ii) if \emph{todo\_comment} is within the scope of the \textit{LinesEqual}, which means the \emph{code\_change} is not responsible for resolving the TODO task, we label such triple instances as \textbf{Negative Samples}. 
(iii) if \emph{todo\_comment} is within the scope of the \textit{LinesAdded}, we ignore such triple instances. 
This is reasonable since the \emph{todo\_comment} within the scope of \textit{LinesAdded} corresponds to the first time TODO comments are added.
However, our research focuses on detecting obsolete TODO comments from the existing ones. This requires that the TODO comments have been already added to the source code. 
Fig.~\ref{fig:data_pre_example} demonstrates the data labelling results for a positive sample and a negative sample respectively. 
We found more than 38K triple instances that are considered as positive samples and 35K triple instances that are considered as negative samples for Python, and 33K positive samples and 32K negative samples for Java. 
% because our research focuses on detecting obsolete TODO comments, while

\subsubsection{Manual Checking}
We automatically built our positive and negative training samples via heuristic rules. 
We can not ensure that there are no outlier cases during the label establishment process. 
Therefore, we performed a manual checking step to examine the label of the training sample is correct or not. 
We randomly sampled 200 samples (including 100 positive samples and 100 negative samples) from our dataset. 
Then, the first author manually examined each sample and classified the \emph{todo\_comment} is resolved or not based on checking the associated \emph{code\_change} and \emph{commit\_msg}. 
% It is worth emphasizing that the participant were blinded to which sample is positive or negative.
Finally, 93 of the positive training samples are marked as resolved and all of the negative training samples are marked as unresolved. 
% To mitigate personal bias, we also invited another independent volunteer to do the classification task and measured the level of agreement between the two manual classifiers. 
% We find a high level of agreement with a Cohen`s Kappa coefficient\cite{} of \cite{}, which shows the substantial agreement among different labellers.  
Thus, we are confident in the labels of our provided dataset. 


\subsubsection{Data Splitting}
We split the constructed data samples into three chunks: 80 percent of the triple samples are used for training, 10 percent are used for validation and the rest are held-out for testing. 
The training set is used to adjust the parameters, while the validation set is used to minimize overfitting,
% i.e., verifying that any performance increase over the training dataset actually yields an accuracy increase over the dataset that has not been shown to the model before. 
and the testing set is used only for testing the final solution to confirm the actual predictive power of our model with optimal parameters.
The number of training, validation, test sets of Python and Java dataset are displayed in Table~\ref{tab:data_sta}.
% As a result, our final training, validation and test sets contains 

\begin{table} % \vspace{-0.3cm}
\caption{Data Statistics}
\begin{center}
% \vspace{-3pt}
\begin{tabular}{||c|l|c||}
    \hline  
    \multirow{5}{*}{Python}   & \# TODO Commits  & 416,666  \\ \cline{2-3}
                              & \# Positive samples  & 38,175 \\ \cline{2-3}
                              & \# Negative samples  & 35,995 \\ \cline{2-3}
                              & \# Train Set & 59,336 \\ \cline{2-3}
                              & \# Val\&Test Set & 7,417 \\ \cline{2-3}
    \hline
    \multirow{5}{*}{Java}   & \# TODO Commits  & 351,266  \\ \cline{2-3}
                          & \# Positive samples  & 33,797 \\ \cline{2-3}
                          & \# Negative samples  & 32,490 \\ \cline{2-3}
                          & \# Train Set & 53,029 \\ \cline{2-3}
                          & \# Val\&Test Set & 6,629 \\ \cline{2-3}
    \hline  
\end{tabular}
\label{tab:data_sta}
\end{center}
% \vspace{-5pt}
\end{table}





==> dis.tex <==
%In this section, we perform an manual analysis to investigate the reasons why our approach success, a practical analysis to investigate the practical usage of {\sc TDCleaner}, and the threats to validity of our approach. 
%\subsection{Practical Analysis}

Since the final goal of our approach is detecting and removing the obsolete TODO comments in software projects, we also perform an in-the-wild evaluation to evaluate the effectiveness of {\sc TDCleaner} for removing the stale TODO comments in real world software repositories in Github. 


\begin{figure}
\vspace{0.0cm}
\centerline{\includegraphics[width=0.49\textwidth]{pr-example.pdf}}
% \vspace*{-5pt}
\caption{Pull Request Examples}
\label{fig:example}
% \vspace{-5pt}
\end{figure}

We randomly selected 100 Python repositories hosted on Github; for each Github repository, we first clone the repository from Github to local. 
Following that, we checkout all the commits of the repository to identify the TODO related commits. 
By going through the same steps of normalization, we extract the \textit{todo\_comment}, \textit{code\_change} and \textit{commit\_msg} from \texttt{diff} and commit messages.
We then build $\langle code\_change, todo\_comment, commit\_msg \rangle$ triple and feed the triple as input for {\sc TDCleaner}. 
For each constructed triple input,  
we apply {\sc TDCleaner} to check if the TODO comment has been resolved or not. 
If the TODO comment has been identified as resolved by our approach but not removed accordingly, we regard this TODO comment as obsolete. 

We ran {\sc TDCleaner} on these software projects and {\sc TDCleaner} reported that 23 TODO comments as being obsolete.
We manually checked all of these reported TODO comments, 5 of them are ``intermediate'' obsolete TODO comments, which means they
have been removed in subsequent versions. 
The reason for this phenomenon maybe that developers often clean up the obsolete TODO comments before specific software releases. 
Even though these TODO comments are finally removed during software development before being cleaned up by developers, they may mislead developers, waste their time to check the implementations, complicate the code review and cause the introduction of bugs.
It is necessary to remove the obsolete TODO comments just-in-time or avoid introducing them at all. 

In addition to the 5 ``intermediate'' obsolete TODO comments, there are still 18 ``potential'' obsolete TODO comments dangling in the current version of these projects. 
For each of these ``potential'' obsolete TODO comments, we would like to investigate if it is really an obsolete comment based on developer feedback.
To do this we submitted a pull-request to the corresponding Github repository by removing this ``potential'' obsolete TODO comment. 
To help developers verify the pull-request more easily and confidently, we also notified the developers for the commit for which our approach identifies this TODO comment has been resolved. 
An example of our submitted pull-request is shown in ~\ref{fig:practical_example}.
To avoid subjective bias, the developers don't know the pull-requests are automatically detected by our tool {\sc TDCleaner}. 
We submitted 18 pull-requests and 9 of them have already been confirmed and merged by the developers. 4 of them were closed by developers and the rest of them are still open. 
Fig.~\ref{fig:practical_example} demonstrates three examples we submitted to the developers.
From developers feedback to us we make the following observations:

\begin{figure}
\vspace{0.0cm}
\centerline{\includegraphics[width=0.49\textwidth]{practical-example.pdf}}
% \vspace*{-5pt}
\caption{Practical Analysis Examples}
\label{fig:practical_example}
% \vspace{-10pt}
\end{figure}

\begin{itemize}
    \item For developers who have adopted our pull-request changes, they appreciated the contributions we made to their repositories.
    This signals that our proposed model, i.e., {\sc TDCleaner}, has positive effects to the robustness of the system and may decrease the cost of its development and maintenance.  
    
    \item Some developers expressed their curiosity about how we detected these obsolete TODO comments.
    For example, when we submitted pull-request to the first repository in Fig.~\ref{fig:practical_example}, a developer mentioned, \textit{``Indeed, thank you! I wonder how did you find this? Just browsing the code at leisure time? :)''}. 
    This is because this Github repository contains more than 4,000 commits, it is thus very hard, if not possible, to manually identify an obsolete TODO comment from the huge amount of commits accumulated in the repository.
    This also justifies the importance and necessity of developing a tool to automatically detect the obsolete TODO comments.  
    
    \item Instead of completely removing the obsolete TODO comments, some developers suggested another way of just removing the word ``TODO''. 
    The second example in Fig~\ref{fig:practical_example} presents such a situation. 
    When we submitted the pull-request to remove the obsolete TODO comment, the developer responded \textit{``How about just removing the word "TODO"? The rest of the comment is now good documentation.''}.
    This may be a reasonable approach because the TODO comments often describe the pending tasks that should be done, once the developer completed the task, the rest of the TODO could potentially serve as good documentations for the newly added code.  
    
    \item Not all the pull-requests we submitted are accepted by developers. The third case in Fig~\ref{fig:practical_example} shows such an example, the developer closed our pull-request and commented \textit{``Good catch! However although I've already recorded cv\_weights, I haven't actually utilized it yet. Which means, I haven't applied cv\_weights to get a weighted metrics on the validation set.''} 
    This indicates that sometimes the information is not enough for {\sc TDCleaner} to infer the correct prediction, for such cases, we still need developers to double check the results. 
    
\end{itemize}

\vspace{5pt}
\noindent
\framebox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule}{
\textbf{
How effective is our {\sc TDCleaner} for removing obsolete TODO comments in real Github repositories? -- we conclude that our model is effective for detecting obsolete TODO comments in real word Github repos.}}} 
\vspace{5pt} 




==> fontawesomesymbols-generic.tex <==
\def\faGlass{\faicon{glass}}
\def\faMusic{\faicon{music}}
\def\faSearch{\faicon{search}}
\def\faEnvelopeO{\faicon{envelope-o}}
\def\faHeart{\faicon{heart}}
\def\faStar{\faicon{star}}
\def\faStarO{\faicon{star-o}}
\def\faUser{\faicon{user}}
\def\faFilm{\faicon{film}}
\def\faThLarge{\faicon{th-large}}
\def\faTh{\faicon{th}}
\def\faThList{\faicon{th-list}}
\def\faCheck{\faicon{check}}
\def\faTimes{\faicon{times}}
\def\faSearchPlus{\faicon{search-plus}}
\def\faSearchMinus{\faicon{search-minus}}
\def\faPowerOff{\faicon{power-off}}
\def\faSignal{\faicon{signal}}
\def\faCog{\faicon{cog}}
\def\faTrashO{\faicon{trash-o}}
\def\faHome{\faicon{home}}
\def\faFileO{\faicon{file-o}}
\def\faClockO{\faicon{clock-o}}
\def\faRoad{\faicon{road}}
\def\faDownload{\faicon{download}}
\def\faArrowCircleODown{\faicon{arrow-circle-o-down}}
\def\faArrowCircleOUp{\faicon{arrow-circle-o-up}}
\def\faInbox{\faicon{inbox}}
\def\faPlayCircleO{\faicon{play-circle-o}}
\def\faRepeat{\faicon{repeat}}
\def\faRefresh{\faicon{refresh}}
\def\faListAlt{\faicon{list-alt}}
\def\faLock{\faicon{lock}}
\def\faFlag{\faicon{flag}}
\def\faHeadphones{\faicon{headphones}}
\def\faVolumeOff{\faicon{volume-off}}
\def\faVolumeDown{\faicon{volume-down}}
\def\faVolumeUp{\faicon{volume-up}}
\def\faQrcode{\faicon{qrcode}}
\def\faBarcode{\faicon{barcode}}
\def\faTag{\faicon{tag}}
\def\faTags{\faicon{tags}}
\def\faBook{\faicon{book}}
\def\faBookmark{\faicon{bookmark}}
\def\faPrint{\faicon{print}}
\def\faCamera{\faicon{camera}}
\def\faFont{\faicon{font}}
\def\faBold{\faicon{bold}}
\def\faItalic{\faicon{italic}}
\def\faTextHeight{\faicon{text-height}}
\def\faTextWidth{\faicon{text-width}}
\def\faAlignLeft{\faicon{align-left}}
\def\faAlignCenter{\faicon{align-center}}
\def\faAlignRight{\faicon{align-right}}
\def\faAlignJustify{\faicon{align-justify}}
\def\faList{\faicon{list}}
\def\faOutdent{\faicon{outdent}}
\def\faIndent{\faicon{indent}}
\def\faVideoCamera{\faicon{video-camera}}
\def\faPictureO{\faicon{picture-o}}
\def\faPencil{\faicon{pencil}}
\def\faMapMarker{\faicon{map-marker}}
\def\faAdjust{\faicon{adjust}}
\def\faTint{\faicon{tint}}
\def\faPencilSquareO{\faicon{pencil-square-o}}
\def\faShareSquareO{\faicon{share-square-o}}
\def\faCheckSquareO{\faicon{check-square-o}}
\def\faArrows{\faicon{arrows}}
\def\faStepBackward{\faicon{step-backward}}
\def\faFastBackward{\faicon{fast-backward}}
\def\faBackward{\faicon{backward}}
\def\faPlay{\faicon{play}}
\def\faPause{\faicon{pause}}
\def\faStop{\faicon{stop}}
\def\faForward{\faicon{forward}}
\def\faFastForward{\faicon{fast-forward}}
\def\faStepForward{\faicon{step-forward}}
\def\faEject{\faicon{eject}}
\def\faChevronLeft{\faicon{chevron-left}}
\def\faChevronRight{\faicon{chevron-right}}
\def\faPlusCircle{\faicon{plus-circle}}
\def\faMinusCircle{\faicon{minus-circle}}
\def\faTimesCircle{\faicon{times-circle}}
\def\faCheckCircle{\faicon{check-circle}}
\def\faQuestionCircle{\faicon{question-circle}}
\def\faInfoCircle{\faicon{info-circle}}
\def\faCrosshairs{\faicon{crosshairs}}
\def\faTimesCircleO{\faicon{times-circle-o}}
\def\faCheckCircleO{\faicon{check-circle-o}}
\def\faBan{\faicon{ban}}
\def\faArrowLeft{\faicon{arrow-left}}
\def\faArrowRight{\faicon{arrow-right}}
\def\faArrowUp{\faicon{arrow-up}}
\def\faArrowDown{\faicon{arrow-down}}
\def\faShare{\faicon{share}}
\def\faExpand{\faicon{expand}}
\def\faCompress{\faicon{compress}}
\def\faPlus{\faicon{plus}}
\def\faMinus{\faicon{minus}}
\def\faAsterisk{\faicon{asterisk}}
\def\faExclamationCircle{\faicon{exclamation-circle}}
\def\faGift{\faicon{gift}}
\def\faLeaf{\faicon{leaf}}
\def\faFire{\faicon{fire}}
\def\faEye{\faicon{eye}}
\def\faEyeSlash{\faicon{eye-slash}}
\def\faExclamationTriangle{\faicon{exclamation-triangle}}
\def\faPlane{\faicon{plane}}
\def\faCalendar{\faicon{calendar}}
\def\faRandom{\faicon{random}}
\def\faComment{\faicon{comment}}
\def\faMagnet{\faicon{magnet}}
\def\faChevronUp{\faicon{chevron-up}}
\def\faChevronDown{\faicon{chevron-down}}
\def\faRetweet{\faicon{retweet}}
\def\faShoppingCart{\faicon{shopping-cart}}
\def\faFolder{\faicon{folder}}
\def\faFolderOpen{\faicon{folder-open}}
\def\faArrowsV{\faicon{arrows-v}}
\def\faArrowsH{\faicon{arrows-h}}
\def\faBarChart{\faicon{bar-chart}}
\def\faTwitterSquare{\faicon{twitter-square}}
\def\faFacebookSquare{\faicon{facebook-square}}
\def\faCameraRetro{\faicon{camera-retro}}
\def\faKey{\faicon{key}}
\def\faCogs{\faicon{cogs}}
\def\faComments{\faicon{comments}}
\def\faThumbsOUp{\faicon{thumbs-o-up}}
\def\faThumbsODown{\faicon{thumbs-o-down}}
\def\faStarHalf{\faicon{star-half}}
\def\faHeartO{\faicon{heart-o}}
\def\faSignOut{\faicon{sign-out}}
\def\faLinkedinSquare{\faicon{linkedin-square}}
\def\faThumbTack{\faicon{thumb-tack}}
\def\faExternalLink{\faicon{external-link}}
\def\faSignIn{\faicon{sign-in}}
\def\faTrophy{\faicon{trophy}}
\def\faGithubSquare{\faicon{github-square}}
\def\faUpload{\faicon{upload}}
\def\faLemonO{\faicon{lemon-o}}
\def\faPhone{\faicon{phone}}
\def\faSquareO{\faicon{square-o}}
\def\faBookmarkO{\faicon{bookmark-o}}
\def\faPhoneSquare{\faicon{phone-square}}
\def\faTwitter{\faicon{twitter}}
\def\faFacebook{\faicon{facebook}}
\def\faGithub{\faicon{github}}
\def\faUnlock{\faicon{unlock}}
\def\faCreditCard{\faicon{credit-card}}
\def\faRss{\faicon{rss}}
\def\faHddO{\faicon{hdd-o}}
\def\faBullhorn{\faicon{bullhorn}}
\def\faBell{\faicon{bell}}
\def\faCertificate{\faicon{certificate}}
\def\faHandORight{\faicon{hand-o-right}}
\def\faHandOLeft{\faicon{hand-o-left}}
\def\faHandOUp{\faicon{hand-o-up}}
\def\faHandODown{\faicon{hand-o-down}}
\def\faArrowCircleLeft{\faicon{arrow-circle-left}}
\def\faArrowCircleRight{\faicon{arrow-circle-right}}
\def\faArrowCircleUp{\faicon{arrow-circle-up}}
\def\faArrowCircleDown{\faicon{arrow-circle-down}}
\def\faGlobe{\faicon{globe}}
\def\faWrench{\faicon{wrench}}
\def\faTasks{\faicon{tasks}}
\def\faFilter{\faicon{filter}}
\def\faBriefcase{\faicon{briefcase}}
\def\faArrowsAlt{\faicon{arrows-alt}}
\def\faUsers{\faicon{users}}
\def\faLink{\faicon{link}}
\def\faCloud{\faicon{cloud}}
\def\faFlask{\faicon{flask}}
\def\faScissors{\faicon{scissors}}
\def\faFilesO{\faicon{files-o}}
\def\faPaperclip{\faicon{paperclip}}
\def\faFloppyO{\faicon{floppy-o}}
\def\faSquare{\faicon{square}}
\def\faBars{\faicon{bars}}
\def\faListUl{\faicon{list-ul}}
\def\faListOl{\faicon{list-ol}}
\def\faStrikethrough{\faicon{strikethrough}}
\def\faUnderline{\faicon{underline}}
\def\faTable{\faicon{table}}
\def\faMagic{\faicon{magic}}
\def\faTruck{\faicon{truck}}
\def\faPinterest{\faicon{pinterest}}
\def\faPinterestSquare{\faicon{pinterest-square}}
\def\faGooglePlusSquare{\faicon{google-plus-square}}
\def\faGooglePlus{\faicon{google-plus}}
\def\faMoney{\faicon{money}}
\def\faCaretDown{\faicon{caret-down}}
\def\faCaretUp{\faicon{caret-up}}
\def\faCaretLeft{\faicon{caret-left}}
\def\faCaretRight{\faicon{caret-right}}
\def\faColumns{\faicon{columns}}
\def\faSort{\faicon{sort}}
\def\faSortDesc{\faicon{sort-desc}}
\def\faSortAsc{\faicon{sort-asc}}
\def\faEnvelope{\faicon{envelope}}
\def\faLinkedin{\faicon{linkedin}}
\def\faUndo{\faicon{undo}}
\def\faGavel{\faicon{gavel}}
\def\faTachometer{\faicon{tachometer}}
\def\faCommentO{\faicon{comment-o}}
\def\faCommentsO{\faicon{comments-o}}
\def\faBolt{\faicon{bolt}}
\def\faSitemap{\faicon{sitemap}}
\def\faUmbrella{\faicon{umbrella}}
\def\faClipboard{\faicon{clipboard}}
\def\faLightbulbO{\faicon{lightbulb-o}}
\def\faExchange{\faicon{exchange}}
\def\faCloudDownload{\faicon{cloud-download}}
\def\faCloudUpload{\faicon{cloud-upload}}
\def\faUserMd{\faicon{user-md}}
\def\faStethoscope{\faicon{stethoscope}}
\def\faSuitcase{\faicon{suitcase}}
\def\faBellO{\faicon{bell-o}}
\def\faCoffee{\faicon{coffee}}
\def\faCutlery{\faicon{cutlery}}
\def\faFileTextO{\faicon{file-text-o}}
\def\faBuildingO{\faicon{building-o}}
\def\faHospitalO{\faicon{hospital-o}}
\def\faAmbulance{\faicon{ambulance}}
\def\faMedkit{\faicon{medkit}}
\def\faFighterJet{\faicon{fighter-jet}}
\def\faBeer{\faicon{beer}}
\def\faHSquare{\faicon{h-square}}
\def\faPlusSquare{\faicon{plus-square}}
\def\faAngleDoubleLeft{\faicon{angle-double-left}}
\def\faAngleDoubleRight{\faicon{angle-double-right}}
\def\faAngleDoubleUp{\faicon{angle-double-up}}
\def\faAngleDoubleDown{\faicon{angle-double-down}}
\def\faAngleLeft{\faicon{angle-left}}
\def\faAngleRight{\faicon{angle-right}}
\def\faAngleUp{\faicon{angle-up}}
\def\faAngleDown{\faicon{angle-down}}
\def\faDesktop{\faicon{desktop}}
\def\faLaptop{\faicon{laptop}}
\def\faTablet{\faicon{tablet}}
\def\faMobile{\faicon{mobile}}
\def\faCircleO{\faicon{circle-o}}
\def\faQuoteLeft{\faicon{quote-left}}
\def\faQuoteRight{\faicon{quote-right}}
\def\faSpinner{\faicon{spinner}}
\def\faCircle{\faicon{circle}}
\def\faReply{\faicon{reply}}
\def\faGithubAlt{\faicon{github-alt}}
\def\faFolderO{\faicon{folder-o}}
\def\faFolderOpenO{\faicon{folder-open-o}}
\def\faSmileO{\faicon{smile-o}}
\def\faFrownO{\faicon{frown-o}}
\def\faMehO{\faicon{meh-o}}
\def\faGamepad{\faicon{gamepad}}
\def\faKeyboardO{\faicon{keyboard-o}}
\def\faFlagO{\faicon{flag-o}}
\def\faFlagCheckered{\faicon{flag-checkered}}
\def\faTerminal{\faicon{terminal}}
\def\faCode{\faicon{code}}
\def\faReplyAll{\faicon{reply-all}}
\def\faStarHalfO{\faicon{star-half-o}}
\def\faLocationArrow{\faicon{location-arrow}}
\def\faCrop{\faicon{crop}}
\def\faCodeFork{\faicon{code-fork}}
\def\faChainBroken{\faicon{chain-broken}}
\def\faQuestion{\faicon{question}}
\def\faInfo{\faicon{info}}
\def\faExclamation{\faicon{exclamation}}
\def\faSuperscript{\faicon{superscript}}
\def\faSubscript{\faicon{subscript}}
\def\faEraser{\faicon{eraser}}
\def\faPuzzlePiece{\faicon{puzzle-piece}}
\def\faMicrophone{\faicon{microphone}}
\def\faMicrophoneSlash{\faicon{microphone-slash}}
\def\faShield{\faicon{shield}}
\def\faCalendarO{\faicon{calendar-o}}
\def\faFireExtinguisher{\faicon{fire-extinguisher}}
\def\faRocket{\faicon{rocket}}
\def\faMaxcdn{\faicon{maxcdn}}
\def\faChevronCircleLeft{\faicon{chevron-circle-left}}
\def\faChevronCircleRight{\faicon{chevron-circle-right}}
\def\faChevronCircleUp{\faicon{chevron-circle-up}}
\def\faChevronCircleDown{\faicon{chevron-circle-down}}
\def\faHtml5{\faicon{html5}}
\def\faCss3{\faicon{css3}}
\def\faAnchor{\faicon{anchor}}
\def\faUnlockAlt{\faicon{unlock-alt}}
\def\faBullseye{\faicon{bullseye}}
\def\faEllipsisH{\faicon{ellipsis-h}}
\def\faEllipsisV{\faicon{ellipsis-v}}
\def\faRssSquare{\faicon{rss-square}}
\def\faPlayCircle{\faicon{play-circle}}
\def\faTicket{\faicon{ticket}}
\def\faMinusSquare{\faicon{minus-square}}
\def\faMinusSquareO{\faicon{minus-square-o}}
\def\faLevelUp{\faicon{level-up}}
\def\faLevelDown{\faicon{level-down}}
\def\faCheckSquare{\faicon{check-square}}
\def\faPencilSquare{\faicon{pencil-square}}
\def\faExternalLinkSquare{\faicon{external-link-square}}
\def\faShareSquare{\faicon{share-square}}
\def\faCompass{\faicon{compass}}
\def\faCaretSquareODown{\faicon{caret-square-o-down}}
\def\faCaretSquareOUp{\faicon{caret-square-o-up}}
\def\faCaretSquareORight{\faicon{caret-square-o-right}}
\def\faEur{\faicon{eur}}
\def\faGbp{\faicon{gbp}}
\def\faUsd{\faicon{usd}}
\def\faInr{\faicon{inr}}
\def\faJpy{\faicon{jpy}}
\def\faRub{\faicon{rub}}
\def\faKrw{\faicon{krw}}
\def\faBtc{\faicon{btc}}
\def\faFile{\faicon{file}}
\def\faFileText{\faicon{file-text}}
\def\faSortAlphaAsc{\faicon{sort-alpha-asc}}
\def\faSortAlphaDesc{\faicon{sort-alpha-desc}}
\def\faSortAmountAsc{\faicon{sort-amount-asc}}
\def\faSortAmountDesc{\faicon{sort-amount-desc}}
\def\faSortNumericAsc{\faicon{sort-numeric-asc}}
\def\faSortNumericDesc{\faicon{sort-numeric-desc}}
\def\faThumbsUp{\faicon{thumbs-up}}
\def\faThumbsDown{\faicon{thumbs-down}}
\def\faYoutubeSquare{\faicon{youtube-square}}
\def\faYoutube{\faicon{youtube}}
\def\faXing{\faicon{xing}}
\def\faXingSquare{\faicon{xing-square}}
\def\faYoutubePlay{\faicon{youtube-play}}
\def\faDropbox{\faicon{dropbox}}
\def\faStackOverflow{\faicon{stack-overflow}}
\def\faInstagram{\faicon{instagram}}
\def\faFlickr{\faicon{flickr}}
\def\faAdn{\faicon{adn}}
\def\faBitbucket{\faicon{bitbucket}}
\def\faBitbucketSquare{\faicon{bitbucket-square}}
\def\faTumblr{\faicon{tumblr}}
\def\faTumblrSquare{\faicon{tumblr-square}}
\def\faLongArrowDown{\faicon{long-arrow-down}}
\def\faLongArrowUp{\faicon{long-arrow-up}}
\def\faLongArrowLeft{\faicon{long-arrow-left}}
\def\faLongArrowRight{\faicon{long-arrow-right}}
\def\faApple{\faicon{apple}}
\def\faWindows{\faicon{windows}}
\def\faAndroid{\faicon{android}}
\def\faLinux{\faicon{linux}}
\def\faDribbble{\faicon{dribbble}}
\def\faSkype{\faicon{skype}}
\def\faFoursquare{\faicon{foursquare}}
\def\faTrello{\faicon{trello}}
\def\faFemale{\faicon{female}}
\def\faMale{\faicon{male}}
\def\faGratipay{\faicon{gratipay}}
\def\faSunO{\faicon{sun-o}}
\def\faMoonO{\faicon{moon-o}}
\def\faArchive{\faicon{archive}}
\def\faBug{\faicon{bug}}
\def\faVk{\faicon{vk}}
\def\faWeibo{\faicon{weibo}}
\def\faRenren{\faicon{renren}}
\def\faPagelines{\faicon{pagelines}}
\def\faStackExchange{\faicon{stack-exchange}}
\def\faArrowCircleORight{\faicon{arrow-circle-o-right}}
\def\faArrowCircleOLeft{\faicon{arrow-circle-o-left}}
\def\faCaretSquareOLeft{\faicon{caret-square-o-left}}
\def\faDotCircleO{\faicon{dot-circle-o}}
\def\faWheelchair{\faicon{wheelchair}}
\def\faVimeoSquare{\faicon{vimeo-square}}
\def\faTry{\faicon{try}}
\def\faPlusSquareO{\faicon{plus-square-o}}
\def\faSpaceShuttle{\faicon{space-shuttle}}
\def\faSlack{\faicon{slack}}
\def\faEnvelopeSquare{\faicon{envelope-square}}
\def\faWordpress{\faicon{wordpress}}
\def\faOpenid{\faicon{openid}}
\def\faUniversity{\faicon{university}}
\def\faGraduationCap{\faicon{graduation-cap}}
\def\faYahoo{\faicon{yahoo}}
\def\faGoogle{\faicon{google}}
\def\faReddit{\faicon{reddit}}
\def\faRedditSquare{\faicon{reddit-square}}
\def\faStumbleuponCircle{\faicon{stumbleupon-circle}}
\def\faStumbleupon{\faicon{stumbleupon}}
\def\faDelicious{\faicon{delicious}}
\def\faDigg{\faicon{digg}}
\def\faPiedPiperPp{\faicon{pied-piper-pp}}
\def\faPiedPiperAlt{\faicon{pied-piper-alt}}
\def\faDrupal{\faicon{drupal}}
\def\faJoomla{\faicon{joomla}}
\def\faLanguage{\faicon{language}}
\def\faFax{\faicon{fax}}
\def\faBuilding{\faicon{building}}
\def\faChild{\faicon{child}}
\def\faPaw{\faicon{paw}}
\def\faSpoon{\faicon{spoon}}
\def\faCube{\faicon{cube}}
\def\faCubes{\faicon{cubes}}
\def\faBehance{\faicon{behance}}
\def\faBehanceSquare{\faicon{behance-square}}
\def\faSteam{\faicon{steam}}
\def\faSteamSquare{\faicon{steam-square}}
\def\faRecycle{\faicon{recycle}}
\def\faCar{\faicon{car}}
\def\faTaxi{\faicon{taxi}}
\def\faTree{\faicon{tree}}
\def\faSpotify{\faicon{spotify}}
\def\faDeviantart{\faicon{deviantart}}
\def\faSoundcloud{\faicon{soundcloud}}
\def\faDatabase{\faicon{database}}
\def\faFilePdfO{\faicon{file-pdf-o}}
\def\faFileWordO{\faicon{file-word-o}}
\def\faFileExcelO{\faicon{file-excel-o}}
\def\faFilePowerpointO{\faicon{file-powerpoint-o}}
\def\faFileImageO{\faicon{file-image-o}}
\def\faFileArchiveO{\faicon{file-archive-o}}
\def\faFileAudioO{\faicon{file-audio-o}}
\def\faFileVideoO{\faicon{file-video-o}}
\def\faFileCodeO{\faicon{file-code-o}}
\def\faVine{\faicon{vine}}
\def\faCodepen{\faicon{codepen}}
\def\faJsfiddle{\faicon{jsfiddle}}
\def\faLifeRing{\faicon{life-ring}}
\def\faCircleONotch{\faicon{circle-o-notch}}
\def\faRebel{\faicon{rebel}}
\def\faEmpire{\faicon{empire}}
\def\faGitSquare{\faicon{git-square}}
\def\faGit{\faicon{git}}
\def\faHackerNews{\faicon{hacker-news}}
\def\faTencentWeibo{\faicon{tencent-weibo}}
\def\faQq{\faicon{qq}}
\def\faWeixin{\faicon{weixin}}
\def\faPaperPlane{\faicon{paper-plane}}
\def\faPaperPlaneO{\faicon{paper-plane-o}}
\def\faHistory{\faicon{history}}
\def\faCircleThin{\faicon{circle-thin}}
\def\faHeader{\faicon{header}}
\def\faParagraph{\faicon{paragraph}}
\def\faSliders{\faicon{sliders}}
\def\faShareAlt{\faicon{share-alt}}
\def\faShareAltSquare{\faicon{share-alt-square}}
\def\faBomb{\faicon{bomb}}
\def\faFutbolO{\faicon{futbol-o}}
\def\faTty{\faicon{tty}}
\def\faBinoculars{\faicon{binoculars}}
\def\faPlug{\faicon{plug}}
\def\faSlideshare{\faicon{slideshare}}
\def\faTwitch{\faicon{twitch}}
\def\faYelp{\faicon{yelp}}
\def\faNewspaperO{\faicon{newspaper-o}}
\def\faWifi{\faicon{wifi}}
\def\faCalculator{\faicon{calculator}}
\def\faPaypal{\faicon{paypal}}
\def\faGoogleWallet{\faicon{google-wallet}}
\def\faCcVisa{\faicon{cc-visa}}
\def\faCcMastercard{\faicon{cc-mastercard}}
\def\faCcDiscover{\faicon{cc-discover}}
\def\faCcAmex{\faicon{cc-amex}}
\def\faCcPaypal{\faicon{cc-paypal}}
\def\faCcStripe{\faicon{cc-stripe}}
\def\faBellSlash{\faicon{bell-slash}}
\def\faBellSlashO{\faicon{bell-slash-o}}
\def\faTrash{\faicon{trash}}
\def\faCopyright{\faicon{copyright}}
\def\faAt{\faicon{at}}
\def\faEyedropper{\faicon{eyedropper}}
\def\faPaintBrush{\faicon{paint-brush}}
\def\faBirthdayCake{\faicon{birthday-cake}}
\def\faAreaChart{\faicon{area-chart}}
\def\faPieChart{\faicon{pie-chart}}
\def\faLineChart{\faicon{line-chart}}
\def\faLastfm{\faicon{lastfm}}
\def\faLastfmSquare{\faicon{lastfm-square}}
\def\faToggleOff{\faicon{toggle-off}}
\def\faToggleOn{\faicon{toggle-on}}
\def\faBicycle{\faicon{bicycle}}
\def\faBus{\faicon{bus}}
\def\faIoxhost{\faicon{ioxhost}}
\def\faAngellist{\faicon{angellist}}
\def\faCc{\faicon{cc}}
\def\faIls{\faicon{ils}}
\def\faMeanpath{\faicon{meanpath}}
\def\faBuysellads{\faicon{buysellads}}
\def\faConnectdevelop{\faicon{connectdevelop}}
\def\faDashcube{\faicon{dashcube}}
\def\faForumbee{\faicon{forumbee}}
\def\faLeanpub{\faicon{leanpub}}
\def\faSellsy{\faicon{sellsy}}
\def\faShirtsinbulk{\faicon{shirtsinbulk}}
\def\faSimplybuilt{\faicon{simplybuilt}}
\def\faSkyatlas{\faicon{skyatlas}}
\def\faCartPlus{\faicon{cart-plus}}
\def\faCartArrowDown{\faicon{cart-arrow-down}}
\def\faDiamond{\faicon{diamond}}
\def\faShip{\faicon{ship}}
\def\faUserSecret{\faicon{user-secret}}
\def\faMotorcycle{\faicon{motorcycle}}
\def\faStreetView{\faicon{street-view}}
\def\faHeartbeat{\faicon{heartbeat}}
\def\faVenus{\faicon{venus}}
\def\faMars{\faicon{mars}}
\def\faMercury{\faicon{mercury}}
\def\faTransgender{\faicon{transgender}}
\def\faTransgenderAlt{\faicon{transgender-alt}}
\def\faVenusDouble{\faicon{venus-double}}
\def\faMarsDouble{\faicon{mars-double}}
\def\faVenusMars{\faicon{venus-mars}}
\def\faMarsStroke{\faicon{mars-stroke}}
\def\faMarsStrokeV{\faicon{mars-stroke-v}}
\def\faMarsStrokeH{\faicon{mars-stroke-h}}
\def\faNeuter{\faicon{neuter}}
\def\faGenderless{\faicon{genderless}}
\def\faFacebookOfficial{\faicon{facebook-official}}
\def\faPinterestP{\faicon{pinterest-p}}
\def\faWhatsapp{\faicon{whatsapp}}
\def\faServer{\faicon{server}}
\def\faUserPlus{\faicon{user-plus}}
\def\faUserTimes{\faicon{user-times}}
\def\faBed{\faicon{bed}}
\def\faViacoin{\faicon{viacoin}}
\def\faTrain{\faicon{train}}
\def\faSubway{\faicon{subway}}
\def\faMedium{\faicon{medium}}
\def\faYCombinator{\faicon{y-combinator}}
\def\faOptinMonster{\faicon{optin-monster}}
\def\faOpencart{\faicon{opencart}}
\def\faExpeditedssl{\faicon{expeditedssl}}
\def\faBatteryFull{\faicon{battery-full}}
\def\faBatteryThreeQuarters{\faicon{battery-three-quarters}}
\def\faBatteryHalf{\faicon{battery-half}}
\def\faBatteryQuarter{\faicon{battery-quarter}}
\def\faBatteryEmpty{\faicon{battery-empty}}
\def\faMousePointer{\faicon{mouse-pointer}}
\def\faICursor{\faicon{i-cursor}}
\def\faObjectGroup{\faicon{object-group}}
\def\faObjectUngroup{\faicon{object-ungroup}}
\def\faStickyNote{\faicon{sticky-note}}
\def\faStickyNoteO{\faicon{sticky-note-o}}
\def\faCcJcb{\faicon{cc-jcb}}
\def\faCcDinersClub{\faicon{cc-diners-club}}
\def\faClone{\faicon{clone}}
\def\faBalanceScale{\faicon{balance-scale}}
\def\faHourglassO{\faicon{hourglass-o}}
\def\faHourglassStart{\faicon{hourglass-start}}
\def\faHourglassHalf{\faicon{hourglass-half}}
\def\faHourglassEnd{\faicon{hourglass-end}}
\def\faHourglass{\faicon{hourglass}}
\def\faHandRockO{\faicon{hand-rock-o}}
\def\faHandPaperO{\faicon{hand-paper-o}}
\def\faHandScissorsO{\faicon{hand-scissors-o}}
\def\faHandLizardO{\faicon{hand-lizard-o}}
\def\faHandSpockO{\faicon{hand-spock-o}}
\def\faHandPointerO{\faicon{hand-pointer-o}}
\def\faHandPeaceO{\faicon{hand-peace-o}}
\def\faTrademark{\faicon{trademark}}
\def\faRegistered{\faicon{registered}}
\def\faCreativeCommons{\faicon{creative-commons}}
\def\faGg{\faicon{gg}}
\def\faGgCircle{\faicon{gg-circle}}
\def\faTripadvisor{\faicon{tripadvisor}}
\def\faOdnoklassniki{\faicon{odnoklassniki}}
\def\faOdnoklassnikiSquare{\faicon{odnoklassniki-square}}
\def\faGetPocket{\faicon{get-pocket}}
\def\faWikipediaW{\faicon{wikipedia-w}}
\def\faSafari{\faicon{safari}}
\def\faChrome{\faicon{chrome}}
\def\faFirefox{\faicon{firefox}}
\def\faOpera{\faicon{opera}}
\def\faInternetExplorer{\faicon{internet-explorer}}
\def\faTelevision{\faicon{television}}
\def\faContao{\faicon{contao}}
\def\fa500Px{\faicon{500px}}
\def\faAmazon{\faicon{amazon}}
\def\faCalendarPlusO{\faicon{calendar-plus-o}}
\def\faCalendarMinusO{\faicon{calendar-minus-o}}
\def\faCalendarTimesO{\faicon{calendar-times-o}}
\def\faCalendarCheckO{\faicon{calendar-check-o}}
\def\faIndustry{\faicon{industry}}
\def\faMapPin{\faicon{map-pin}}
\def\faMapSigns{\faicon{map-signs}}
\def\faMapO{\faicon{map-o}}
\def\faMap{\faicon{map}}
\def\faCommenting{\faicon{commenting}}
\def\faCommentingO{\faicon{commenting-o}}
\def\faHouzz{\faicon{houzz}}
\def\faVimeo{\faicon{vimeo}}
\def\faBlackTie{\faicon{black-tie}}
\def\faFonticons{\faicon{fonticons}}
\def\faRedditAlien{\faicon{reddit-alien}}
\def\faEdge{\faicon{edge}}
\def\faCreditCardAlt{\faicon{credit-card-alt}}
\def\faCodiepie{\faicon{codiepie}}
\def\faModx{\faicon{modx}}
\def\faFortAwesome{\faicon{fort-awesome}}
\def\faUsb{\faicon{usb}}
\def\faProductHunt{\faicon{product-hunt}}
\def\faMixcloud{\faicon{mixcloud}}
\def\faScribd{\faicon{scribd}}
\def\faPauseCircle{\faicon{pause-circle}}
\def\faPauseCircleO{\faicon{pause-circle-o}}
\def\faStopCircle{\faicon{stop-circle}}
\def\faStopCircleO{\faicon{stop-circle-o}}
\def\faShoppingBag{\faicon{shopping-bag}}
\def\faShoppingBasket{\faicon{shopping-basket}}
\def\faHashtag{\faicon{hashtag}}
\def\faBluetooth{\faicon{bluetooth}}
\def\faBluetoothB{\faicon{bluetooth-b}}
\def\faPercent{\faicon{percent}}
\def\faGitlab{\faicon{gitlab}}
\def\faWpbeginner{\faicon{wpbeginner}}
\def\faWpforms{\faicon{wpforms}}
\def\faEnvira{\faicon{envira}}
\def\faUniversalAccess{\faicon{universal-access}}
\def\faWheelchairAlt{\faicon{wheelchair-alt}}
\def\faQuestionCircleO{\faicon{question-circle-o}}
\def\faBlind{\faicon{blind}}
\def\faAudioDescription{\faicon{audio-description}}
\def\faVolumeControlPhone{\faicon{volume-control-phone}}
\def\faBraille{\faicon{braille}}
\def\faAssistiveListeningSystems{\faicon{assistive-listening-systems}}
\def\faAmericanSignLanguageInterpreting{\faicon{american-sign-language-interpreting}}
\def\faDeaf{\faicon{deaf}}
\def\faGlide{\faicon{glide}}
\def\faGlideG{\faicon{glide-g}}
\def\faSignLanguage{\faicon{sign-language}}
\def\faLowVision{\faicon{low-vision}}
\def\faViadeo{\faicon{viadeo}}
\def\faViadeoSquare{\faicon{viadeo-square}}
\def\faSnapchat{\faicon{snapchat}}
\def\faSnapchatGhost{\faicon{snapchat-ghost}}
\def\faSnapchatSquare{\faicon{snapchat-square}}
\def\faPiedPiper{\faicon{pied-piper}}
\def\faFirstOrder{\faicon{first-order}}
\def\faYoast{\faicon{yoast}}
\def\faThemeisle{\faicon{themeisle}}
\def\faGooglePlusOfficial{\faicon{google-plus-official}}
\def\faFontAwesome{\faicon{font-awesome}}
% aliases
\def\faCny{\faicon{cny}}\expandafter\def\csname faicon@cny\endcsname{\faicon{jpy}}
\def\faYCombinatorSquare{\faicon{y-combinator-square}}\expandafter\def\csname faicon@y-combinator-square\endcsname{\faicon{hacker-news}}
\def\faCab{\faicon{cab}}\expandafter\def\csname faicon@cab\endcsname{\faicon{taxi}}
\def\faToggleUp{\faicon{toggle-up}}\expandafter\def\csname faicon@toggle-up\endcsname{\faicon{caret-square-o-up}}
\def\faLifeBuoy{\faicon{life-buoy}}\expandafter\def\csname faicon@life-buoy\endcsname{\faicon{life-ring}}
\def\faFileZipO{\faicon{file-zip-o}}\expandafter\def\csname faicon@file-zip-o\endcsname{\faicon{file-archive-o}}
\def\faBitcoin{\faicon{bitcoin}}\expandafter\def\csname faicon@bitcoin\endcsname{\faicon{btc}}
\def\faAutomobile{\faicon{automobile}}\expandafter\def\csname faicon@automobile\endcsname{\faicon{car}}
\def\faPaste{\faicon{paste}}\expandafter\def\csname faicon@paste\endcsname{\faicon{clipboard}}
\def\faResistance{\faicon{resistance}}\expandafter\def\csname faicon@resistance\endcsname{\faicon{rebel}}
\def\faCopy{\faicon{copy}}\expandafter\def\csname faicon@copy\endcsname{\faicon{files-o}}
\def\faIntersex{\faicon{intersex}}\expandafter\def\csname faicon@intersex\endcsname{\faicon{transgender}}
\def\faHardOfHearing{\faicon{hard-of-hearing}}\expandafter\def\csname faicon@hard-of-hearing\endcsname{\faicon{deaf}}
\def\faMailReply{\faicon{mail-reply}}\expandafter\def\csname faicon@mail-reply\endcsname{\faicon{reply}}
\def\faSortDown{\faicon{sort-down}}\expandafter\def\csname faicon@sort-down\endcsname{\faicon{sort-desc}}
\def\faGe{\faicon{ge}}\expandafter\def\csname faicon@ge\endcsname{\faicon{empire}}
\def\faBattery2{\faicon{battery-2}}\expandafter\def\csname faicon@battery-2\endcsname{\faicon{battery-half}}
\def\faHandStopO{\faicon{hand-stop-o}}\expandafter\def\csname faicon@hand-stop-o\endcsname{\faicon{hand-paper-o}}
\def\faGroup{\faicon{group}}\expandafter\def\csname faicon@group\endcsname{\faicon{users}}
\def\faRotateRight{\faicon{rotate-right}}\expandafter\def\csname faicon@rotate-right\endcsname{\faicon{repeat}}
\def\faWon{\faicon{won}}\expandafter\def\csname faicon@won\endcsname{\faicon{krw}}
\def\faFa{\faicon{fa}}\expandafter\def\csname faicon@fa\endcsname{\faicon{font-awesome}}
\def\faHourglass3{\faicon{hourglass-3}}\expandafter\def\csname faicon@hourglass-3\endcsname{\faicon{hourglass-end}}
\def\faStarHalfEmpty{\faicon{star-half-empty}}\expandafter\def\csname faicon@star-half-empty\endcsname{\faicon{star-half-o}}
\def\faCut{\faicon{cut}}\expandafter\def\csname faicon@cut\endcsname{\faicon{scissors}}
\def\faToggleDown{\faicon{toggle-down}}\expandafter\def\csname faicon@toggle-down\endcsname{\faicon{caret-square-o-down}}
\def\faGooglePlusCircle{\faicon{google-plus-circle}}\expandafter\def\csname faicon@google-plus-circle\endcsname{\faicon{google-plus-official}}
\def\faSheqel{\faicon{sheqel}}\expandafter\def\csname faicon@sheqel\endcsname{\faicon{ils}}
\def\faDashboard{\faicon{dashboard}}\expandafter\def\csname faicon@dashboard\endcsname{\faicon{tachometer}}
\def\faSend{\faicon{send}}\expandafter\def\csname faicon@send\endcsname{\faicon{paper-plane}}
\def\faYc{\faicon{yc}}\expandafter\def\csname faicon@yc\endcsname{\faicon{y-combinator}}
\def\faToggleLeft{\faicon{toggle-left}}\expandafter\def\csname faicon@toggle-left\endcsname{\faicon{caret-square-o-left}}
\def\faWarning{\faicon{warning}}\expandafter\def\csname faicon@warning\endcsname{\faicon{exclamation-triangle}}
\def\faImage{\faicon{image}}\expandafter\def\csname faicon@image\endcsname{\faicon{picture-o}}
\def\faInstitution{\faicon{institution}}\expandafter\def\csname faicon@institution\endcsname{\faicon{university}}
\def\faFileMovieO{\faicon{file-movie-o}}\expandafter\def\csname faicon@file-movie-o\endcsname{\faicon{file-video-o}}
\def\faPhoto{\faicon{photo}}\expandafter\def\csname faicon@photo\endcsname{\faicon{picture-o}}
\def\faFileSoundO{\faicon{file-sound-o}}\expandafter\def\csname faicon@file-sound-o\endcsname{\faicon{file-audio-o}}
\def\faMortarBoard{\faicon{mortar-board}}\expandafter\def\csname faicon@mortar-board\endcsname{\faicon{graduation-cap}}
\def\faGittip{\faicon{gittip}}\expandafter\def\csname faicon@gittip\endcsname{\faicon{gratipay}}
\def\faHourglass2{\faicon{hourglass-2}}\expandafter\def\csname faicon@hourglass-2\endcsname{\faicon{hourglass-half}}
\def\faSupport{\faicon{support}}\expandafter\def\csname faicon@support\endcsname{\faicon{life-ring}}
\def\faEdit{\faicon{edit}}\expandafter\def\csname faicon@edit\endcsname{\faicon{pencil-square-o}}
\def\faHotel{\faicon{hotel}}\expandafter\def\csname faicon@hotel\endcsname{\faicon{bed}}
\def\faSoccerBallO{\faicon{soccer-ball-o}}\expandafter\def\csname faicon@soccer-ball-o\endcsname{\faicon{futbol-o}}
\def\faFilePictureO{\faicon{file-picture-o}}\expandafter\def\csname faicon@file-picture-o\endcsname{\faicon{file-image-o}}
\def\faClose{\faicon{close}}\expandafter\def\csname faicon@close\endcsname{\faicon{times}}
\def\faYcSquare{\faicon{yc-square}}\expandafter\def\csname faicon@yc-square\endcsname{\faicon{hacker-news}}
\def\faShekel{\faicon{shekel}}\expandafter\def\csname faicon@shekel\endcsname{\faicon{ils}}
\def\faDollar{\faicon{dollar}}\expandafter\def\csname faicon@dollar\endcsname{\faicon{usd}}
\def\faUnsorted{\faicon{unsorted}}\expandafter\def\csname faicon@unsorted\endcsname{\faicon{sort}}
\def\faReorder{\faicon{reorder}}\expandafter\def\csname faicon@reorder\endcsname{\faicon{bars}}
\def\faBattery3{\faicon{battery-3}}\expandafter\def\csname faicon@battery-3\endcsname{\faicon{battery-three-quarters}}
\def\faRupee{\faicon{rupee}}\expandafter\def\csname faicon@rupee\endcsname{\faicon{inr}}
\def\faRouble{\faicon{rouble}}\expandafter\def\csname faicon@rouble\endcsname{\faicon{rub}}
\def\faHourglass1{\faicon{hourglass-1}}\expandafter\def\csname faicon@hourglass-1\endcsname{\faicon{hourglass-start}}
\def\faAslInterpreting{\faicon{asl-interpreting}}\expandafter\def\csname faicon@asl-interpreting\endcsname{\faicon{american-sign-language-interpreting}}
\def\faTv{\faicon{tv}}\expandafter\def\csname faicon@tv\endcsname{\faicon{television}}
\def\faSave{\faicon{save}}\expandafter\def\csname faicon@save\endcsname{\faicon{floppy-o}}
\def\faToggleRight{\faicon{toggle-right}}\expandafter\def\csname faicon@toggle-right\endcsname{\faicon{caret-square-o-right}}
\def\faDedent{\faicon{dedent}}\expandafter\def\csname faicon@dedent\endcsname{\faicon{outdent}}
\def\faGear{\faicon{gear}}\expandafter\def\csname faicon@gear\endcsname{\faicon{cog}}
\def\faLegal{\faicon{legal}}\expandafter\def\csname faicon@legal\endcsname{\faicon{gavel}}
\def\faWechat{\faicon{wechat}}\expandafter\def\csname faicon@wechat\endcsname{\faicon{weixin}}
\def\faFacebookF{\faicon{facebook-f}}\expandafter\def\csname faicon@facebook-f\endcsname{\faicon{facebook}}
\def\faFeed{\faicon{feed}}\expandafter\def\csname faicon@feed\endcsname{\faicon{rss}}
\def\faBank{\faicon{bank}}\expandafter\def\csname faicon@bank\endcsname{\faicon{university}}
\def\faTurkishLira{\faicon{turkish-lira}}\expandafter\def\csname faicon@turkish-lira\endcsname{\faicon{try}}
\def\faUnlink{\faicon{unlink}}\expandafter\def\csname faicon@unlink\endcsname{\faicon{chain-broken}}
\def\faChain{\faicon{chain}}\expandafter\def\csname faicon@chain\endcsname{\faicon{link}}
\def\faGears{\faicon{gears}}\expandafter\def\csname faicon@gears\endcsname{\faicon{cogs}}
\def\faRmb{\faicon{rmb}}\expandafter\def\csname faicon@rmb\endcsname{\faicon{jpy}}
\def\faBattery1{\faicon{battery-1}}\expandafter\def\csname faicon@battery-1\endcsname{\faicon{battery-quarter}}
\def\faLifeBouy{\faicon{life-bouy}}\expandafter\def\csname faicon@life-bouy\endcsname{\faicon{life-ring}}
\def\faYen{\faicon{yen}}\expandafter\def\csname faicon@yen\endcsname{\faicon{jpy}}
\def\faBattery4{\faicon{battery-4}}\expandafter\def\csname faicon@battery-4\endcsname{\faicon{battery-full}}
\def\faBattery0{\faicon{battery-0}}\expandafter\def\csname faicon@battery-0\endcsname{\faicon{battery-empty}}
\def\faHandGrabO{\faicon{hand-grab-o}}\expandafter\def\csname faicon@hand-grab-o\endcsname{\faicon{hand-rock-o}}
\def\faMailReplyAll{\faicon{mail-reply-all}}\expandafter\def\csname faicon@mail-reply-all\endcsname{\faicon{reply-all}}
\def\faMobilePhone{\faicon{mobile-phone}}\expandafter\def\csname faicon@mobile-phone\endcsname{\faicon{mobile}}
\def\faRotateLeft{\faicon{rotate-left}}\expandafter\def\csname faicon@rotate-left\endcsname{\faicon{undo}}
\def\faEuro{\faicon{euro}}\expandafter\def\csname faicon@euro\endcsname{\faicon{eur}}
\def\faRuble{\faicon{ruble}}\expandafter\def\csname faicon@ruble\endcsname{\faicon{rub}}
\def\faRa{\faicon{ra}}\expandafter\def\csname faicon@ra\endcsname{\faicon{rebel}}
\def\faStarHalfFull{\faicon{star-half-full}}\expandafter\def\csname faicon@star-half-full\endcsname{\faicon{star-half-o}}
\def\faSortUp{\faicon{sort-up}}\expandafter\def\csname faicon@sort-up\endcsname{\faicon{sort-asc}}
\def\faMailForward{\faicon{mail-forward}}\expandafter\def\csname faicon@mail-forward\endcsname{\faicon{share}}
\def\faSigning{\faicon{signing}}\expandafter\def\csname faicon@signing\endcsname{\faicon{sign-language}}
\def\faFlash{\faicon{flash}}\expandafter\def\csname faicon@flash\endcsname{\faicon{bolt}}
\def\faLifeSaver{\faicon{life-saver}}\expandafter\def\csname faicon@life-saver\endcsname{\faicon{life-ring}}
\def\faFilePhotoO{\faicon{file-photo-o}}\expandafter\def\csname faicon@file-photo-o\endcsname{\faicon{file-image-o}}
\def\faDeafness{\faicon{deafness}}\expandafter\def\csname faicon@deafness\endcsname{\faicon{deaf}}
\def\faBarChartO{\faicon{bar-chart-o}}\expandafter\def\csname faicon@bar-chart-o\endcsname{\faicon{bar-chart}}
\def\faSendO{\faicon{send-o}}\expandafter\def\csname faicon@send-o\endcsname{\faicon{paper-plane-o}}
\def\faNavicon{\faicon{navicon}}\expandafter\def\csname faicon@navicon\endcsname{\faicon{bars}}
\def\faRemove{\faicon{remove}}\expandafter\def\csname faicon@remove\endcsname{\faicon{times}}


==> fontawesomesymbols-pdftex.tex <==
%% start of file `fontawesomesymbols-pdftex.tex'.
\expandafter\def\csname faicon@info\endcsname{{\FAone\symbol{0}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FAone\symbol{1}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FAone\symbol{2}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FAone\symbol{3}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FAone\symbol{4}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FAone\symbol{5}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FAone\symbol{6}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FAone\symbol{7}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FAone\symbol{8}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FAone\symbol{9}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FAone\symbol{10}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FAone\symbol{11}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FAone\symbol{12}}}
\expandafter\def\csname faicon@try\endcsname{{\FAone\symbol{13}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FAone\symbol{14}}}
\expandafter\def\csname faicon@slack\endcsname{{\FAone\symbol{15}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FAone\symbol{16}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FAone\symbol{17}}}
\expandafter\def\csname faicon@openid\endcsname{{\FAone\symbol{18}}}
\expandafter\def\csname faicon@university\endcsname{{\FAone\symbol{19}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FAone\symbol{20}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FAone\symbol{21}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FAone\symbol{22}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FAone\symbol{23}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FAone\symbol{24}}}
\expandafter\def\csname faicon@digg\endcsname{{\FAone\symbol{25}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FAone\symbol{26}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FAone\symbol{27}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FAone\symbol{28}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FAone\symbol{29}}}
\expandafter\def\csname faicon@fax\endcsname{{\FAone\symbol{30}}}
\expandafter\def\csname faicon@building\endcsname{{\FAone\symbol{31}}}
\expandafter\def\csname faicon@child\endcsname{{\FAone\symbol{32}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FAone\symbol{33}}}
\expandafter\def\csname faicon@cube\endcsname{{\FAone\symbol{34}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FAone\symbol{35}}}
\expandafter\def\csname faicon@behance\endcsname{{\FAone\symbol{36}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FAone\symbol{37}}}
\expandafter\def\csname faicon@steam\endcsname{{\FAone\symbol{38}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FAone\symbol{39}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FAone\symbol{40}}}
\expandafter\def\csname faicon@car\endcsname{{\FAone\symbol{41}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FAone\symbol{42}}}
\expandafter\def\csname faicon@tree\endcsname{{\FAone\symbol{43}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FAone\symbol{44}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FAone\symbol{45}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FAone\symbol{46}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FAone\symbol{47}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FAone\symbol{48}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FAone\symbol{49}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FAone\symbol{50}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FAone\symbol{51}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FAone\symbol{52}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FAone\symbol{53}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FAone\symbol{54}}}
\expandafter\def\csname faicon@vine\endcsname{{\FAone\symbol{55}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FAone\symbol{56}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FAone\symbol{57}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FAone\symbol{58}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FAone\symbol{59}}}
\expandafter\def\csname faicon@git\endcsname{{\FAone\symbol{60}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FAone\symbol{61}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FAone\symbol{62}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FAone\symbol{63}}}
\expandafter\def\csname faicon@history\endcsname{{\FAone\symbol{64}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FAone\symbol{65}}}
\expandafter\def\csname faicon@header\endcsname{{\FAone\symbol{66}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FAone\symbol{67}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FAone\symbol{68}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FAone\symbol{69}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FAone\symbol{70}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FAone\symbol{71}}}
\expandafter\def\csname faicon@tty\endcsname{{\FAone\symbol{72}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FAone\symbol{73}}}
\expandafter\def\csname faicon@plug\endcsname{{\FAone\symbol{74}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FAone\symbol{75}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FAone\symbol{76}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FAone\symbol{77}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FAone\symbol{78}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FAone\symbol{79}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FAone\symbol{80}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FAone\symbol{81}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FAone\symbol{82}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FAone\symbol{83}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FAone\symbol{84}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FAone\symbol{85}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FAone\symbol{86}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FAone\symbol{87}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FAone\symbol{88}}}
\expandafter\def\csname faicon@trash\endcsname{{\FAone\symbol{89}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FAone\symbol{90}}}
\expandafter\def\csname faicon@at\endcsname{{\FAone\symbol{91}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FAone\symbol{92}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FAone\symbol{93}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FAone\symbol{94}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FAone\symbol{95}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FAone\symbol{96}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FAone\symbol{97}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FAone\symbol{98}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FAone\symbol{99}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FAone\symbol{100}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FAone\symbol{101}}}
\expandafter\def\csname faicon@bus\endcsname{{\FAone\symbol{102}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FAone\symbol{103}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FAone\symbol{104}}}
\expandafter\def\csname faicon@cc\endcsname{{\FAone\symbol{105}}}
\expandafter\def\csname faicon@ils\endcsname{{\FAone\symbol{106}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FAone\symbol{107}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FAone\symbol{108}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FAone\symbol{109}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FAone\symbol{110}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FAone\symbol{111}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FAone\symbol{112}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FAone\symbol{113}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FAone\symbol{114}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FAone\symbol{115}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FAone\symbol{116}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FAone\symbol{117}}}
\expandafter\def\csname faicon@ship\endcsname{{\FAone\symbol{118}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FAone\symbol{119}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FAone\symbol{120}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FAone\symbol{121}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FAone\symbol{122}}}
\expandafter\def\csname faicon@mars\endcsname{{\FAone\symbol{123}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FAone\symbol{124}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FAone\symbol{125}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FAone\symbol{126}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FAone\symbol{127}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FAone\symbol{128}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FAone\symbol{129}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FAone\symbol{130}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FAone\symbol{131}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FAone\symbol{132}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FAone\symbol{133}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FAone\symbol{134}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FAone\symbol{135}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FAone\symbol{136}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FAone\symbol{137}}}
\expandafter\def\csname faicon@server\endcsname{{\FAone\symbol{138}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FAone\symbol{139}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FAone\symbol{140}}}
\expandafter\def\csname faicon@bed\endcsname{{\FAone\symbol{141}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FAone\symbol{142}}}
\expandafter\def\csname faicon@train\endcsname{{\FAone\symbol{143}}}
\expandafter\def\csname faicon@subway\endcsname{{\FAone\symbol{144}}}
\expandafter\def\csname faicon@medium\endcsname{{\FAone\symbol{145}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FAone\symbol{146}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FAone\symbol{147}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FAone\symbol{148}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FAone\symbol{149}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FAone\symbol{150}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FAone\symbol{151}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FAone\symbol{152}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FAone\symbol{153}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FAone\symbol{154}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FAone\symbol{155}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FAone\symbol{156}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FAone\symbol{157}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FAone\symbol{158}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FAone\symbol{159}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FAone\symbol{160}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FAone\symbol{161}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FAone\symbol{162}}}
\expandafter\def\csname faicon@clone\endcsname{{\FAone\symbol{163}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FAone\symbol{164}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FAone\symbol{165}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FAone\symbol{166}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FAone\symbol{167}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FAone\symbol{168}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FAone\symbol{169}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FAone\symbol{170}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FAone\symbol{171}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FAone\symbol{172}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FAone\symbol{173}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FAone\symbol{174}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FAone\symbol{175}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FAone\symbol{176}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FAone\symbol{177}}}
\expandafter\def\csname faicon@registered\endcsname{{\FAone\symbol{178}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FAone\symbol{179}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FAone\symbol{180}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FAone\symbol{181}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FAone\symbol{182}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FAone\symbol{183}}}
\expandafter\def\csname faicon@safari\endcsname{{\FAone\symbol{184}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FAone\symbol{185}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FAone\symbol{186}}}
\expandafter\def\csname faicon@opera\endcsname{{\FAone\symbol{187}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FAone\symbol{188}}}
\expandafter\def\csname faicon@television\endcsname{{\FAone\symbol{189}}}
\expandafter\def\csname faicon@contao\endcsname{{\FAone\symbol{190}}}
\expandafter\def\csname faicon@500px\endcsname{{\FAone\symbol{191}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FAone\symbol{192}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FAone\symbol{193}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FAone\symbol{194}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FAone\symbol{195}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FAone\symbol{196}}}
\expandafter\def\csname faicon@industry\endcsname{{\FAone\symbol{197}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FAone\symbol{198}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FAone\symbol{199}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FAone\symbol{200}}}
\expandafter\def\csname faicon@map\endcsname{{\FAone\symbol{201}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FAone\symbol{202}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FAone\symbol{203}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FAone\symbol{204}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FAone\symbol{205}}}
\expandafter\def\csname faicon@edge\endcsname{{\FAone\symbol{206}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FAone\symbol{207}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FAone\symbol{208}}}
\expandafter\def\csname faicon@usb\endcsname{{\FAone\symbol{209}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FAone\symbol{210}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FAone\symbol{211}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FAone\symbol{212}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FAone\symbol{213}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FAone\symbol{214}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FAone\symbol{215}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FAone\symbol{216}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FAone\symbol{217}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FAone\symbol{218}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FAone\symbol{219}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FAone\symbol{220}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FAone\symbol{221}}}
\expandafter\def\csname faicon@percent\endcsname{{\FAone\symbol{222}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FAone\symbol{223}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FAone\symbol{224}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FAone\symbol{225}}}
\expandafter\def\csname faicon@envira\endcsname{{\FAone\symbol{226}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FAone\symbol{227}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FAone\symbol{228}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FAone\symbol{229}}}
\expandafter\def\csname faicon@blind\endcsname{{\FAone\symbol{230}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FAone\symbol{231}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FAone\symbol{232}}}
\expandafter\def\csname faicon@adn\endcsname{{\FAone\symbol{233}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FAone\symbol{234}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FAone\symbol{235}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FAone\symbol{236}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FAone\symbol{237}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FAone\symbol{238}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FAone\symbol{239}}}
\expandafter\def\csname faicon@android\endcsname{{\FAone\symbol{240}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FAone\symbol{241}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FAone\symbol{242}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FAone\symbol{243}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FAone\symbol{244}}}
\expandafter\def\csname faicon@apple\endcsname{{\FAone\symbol{245}}}
\expandafter\def\csname faicon@archive\endcsname{{\FAone\symbol{246}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FAone\symbol{247}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FAone\symbol{248}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FAone\symbol{249}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FAone\symbol{250}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FAone\symbol{251}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FAone\symbol{252}}}
\expandafter\def\csname faicon@backward\endcsname{{\FAone\symbol{253}}}
\expandafter\def\csname faicon@ban\endcsname{{\FAone\symbol{254}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FAone\symbol{255}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FAtwo\symbol{0}}}
\expandafter\def\csname faicon@flask\endcsname{{\FAtwo\symbol{1}}}
\expandafter\def\csname faicon@beer\endcsname{{\FAtwo\symbol{2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FAtwo\symbol{3}}}
\expandafter\def\csname faicon@bell\endcsname{{\FAtwo\symbol{4}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FAtwo\symbol{5}}}
\expandafter\def\csname faicon@bold\endcsname{{\FAtwo\symbol{6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FAtwo\symbol{7}}}
\expandafter\def\csname faicon@book\endcsname{{\FAtwo\symbol{8}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FAtwo\symbol{9}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FAtwo\symbol{10}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FAtwo\symbol{11}}}
\expandafter\def\csname faicon@btc\endcsname{{\FAtwo\symbol{12}}}
\expandafter\def\csname faicon@bug\endcsname{{\FAtwo\symbol{13}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FAtwo\symbol{14}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FAtwo\symbol{15}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FAtwo\symbol{16}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FAtwo\symbol{17}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FAtwo\symbol{18}}}
\expandafter\def\csname faicon@camera\endcsname{{\FAtwo\symbol{19}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FAtwo\symbol{20}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FAtwo\symbol{21}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FAtwo\symbol{22}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FAtwo\symbol{23}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FAtwo\symbol{24}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FAtwo\symbol{25}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FAtwo\symbol{26}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FAtwo\symbol{27}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FAtwo\symbol{28}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FAtwo\symbol{29}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FAtwo\symbol{30}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FAtwo\symbol{31}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FAtwo\symbol{32}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FAtwo\symbol{33}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FAtwo\symbol{34}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FAtwo\symbol{35}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FAtwo\symbol{36}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FAtwo\symbol{37}}}
\expandafter\def\csname faicon@circle\endcsname{{\FAtwo\symbol{38}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FAtwo\symbol{39}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FAtwo\symbol{40}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FAtwo\symbol{41}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FAtwo\symbol{42}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FAtwo\symbol{43}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FAtwo\symbol{44}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FAtwo\symbol{45}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FAtwo\symbol{46}}}
\expandafter\def\csname faicon@code\endcsname{{\FAtwo\symbol{47}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FAtwo\symbol{48}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FAtwo\symbol{49}}}
\expandafter\def\csname faicon@cog\endcsname{{\FAtwo\symbol{50}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FAtwo\symbol{51}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FAtwo\symbol{52}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FAtwo\symbol{53}}}
\expandafter\def\csname faicon@columns\endcsname{{\FAtwo\symbol{54}}}
\expandafter\def\csname faicon@comment\endcsname{{\FAtwo\symbol{55}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FAtwo\symbol{56}}}
\expandafter\def\csname faicon@comments\endcsname{{\FAtwo\symbol{57}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FAtwo\symbol{58}}}
\expandafter\def\csname faicon@compass\endcsname{{\FAtwo\symbol{59}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FAtwo\symbol{60}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FAtwo\symbol{61}}}
\expandafter\def\csname faicon@crop\endcsname{{\FAtwo\symbol{62}}}
\expandafter\def\csname faicon@css3\endcsname{{\FAtwo\symbol{63}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FAtwo\symbol{64}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FAtwo\symbol{65}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FAtwo\symbol{66}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FAtwo\symbol{67}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FAtwo\symbol{68}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FAtwo\symbol{69}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FAtwo\symbol{70}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FAtwo\symbol{71}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FAtwo\symbol{72}}}
\expandafter\def\csname faicon@download\endcsname{{\FAtwo\symbol{73}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FAtwo\symbol{74}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FAtwo\symbol{75}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FAtwo\symbol{76}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FAtwo\symbol{77}}}
\expandafter\def\csname faicon@eject\endcsname{{\FAtwo\symbol{78}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FAtwo\symbol{79}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FAtwo\symbol{80}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FAtwo\symbol{81}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FAtwo\symbol{82}}}
\expandafter\def\csname faicon@eur\endcsname{{\FAtwo\symbol{83}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FAtwo\symbol{84}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FAtwo\symbol{85}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FAtwo\symbol{86}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FAtwo\symbol{87}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FAtwo\symbol{88}}}
\expandafter\def\csname faicon@eye\endcsname{{\FAtwo\symbol{89}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FAtwo\symbol{90}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FAtwo\symbol{91}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FAtwo\symbol{92}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FAtwo\symbol{93}}}
\expandafter\def\csname faicon@language\endcsname{{\FAtwo\symbol{94}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FAtwo\symbol{95}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FAtwo\symbol{96}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FAtwo\symbol{97}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FAtwo\symbol{98}}}
\expandafter\def\csname faicon@gg\endcsname{{\FAtwo\symbol{99}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FAtwo\symbol{100}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FAtwo\symbol{101}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FAtwo\symbol{102}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FAtwo\symbol{103}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FAtwo\symbol{104}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FAtwo\symbol{105}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FAtwo\symbol{106}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FAtwo\symbol{107}}}
\expandafter\def\csname faicon@female\endcsname{{\FAtwo\symbol{108}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FAtwo\symbol{109}}}
\expandafter\def\csname faicon@file\endcsname{{\FAtwo\symbol{110}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FAtwo\symbol{111}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FAtwo\symbol{112}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FAtwo\symbol{113}}}
\expandafter\def\csname faicon@film\endcsname{{\FAtwo\symbol{114}}}
\expandafter\def\csname faicon@filter\endcsname{{\FAtwo\symbol{115}}}
\expandafter\def\csname faicon@fire\endcsname{{\FAtwo\symbol{116}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FAtwo\symbol{117}}}
\expandafter\def\csname faicon@flag\endcsname{{\FAtwo\symbol{118}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FAtwo\symbol{119}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FAtwo\symbol{120}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FAtwo\symbol{121}}}
\expandafter\def\csname faicon@folder\endcsname{{\FAtwo\symbol{122}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FAtwo\symbol{123}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FAtwo\symbol{124}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FAtwo\symbol{125}}}
\expandafter\def\csname faicon@font\endcsname{{\FAtwo\symbol{126}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FAtwo\symbol{127}}}
\expandafter\def\csname faicon@forward\endcsname{{\FAtwo\symbol{128}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FAtwo\symbol{129}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FAtwo\symbol{130}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FAtwo\symbol{131}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FAtwo\symbol{132}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FAtwo\symbol{133}}}
\expandafter\def\csname faicon@gift\endcsname{{\FAtwo\symbol{134}}}
\expandafter\def\csname faicon@github\endcsname{{\FAtwo\symbol{135}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FAtwo\symbol{136}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FAtwo\symbol{137}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FAtwo\symbol{138}}}
\expandafter\def\csname faicon@glass\endcsname{{\FAtwo\symbol{139}}}
\expandafter\def\csname faicon@globe\endcsname{{\FAtwo\symbol{140}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FAtwo\symbol{141}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FAtwo\symbol{142}}}
\expandafter\def\csname faicon@users\endcsname{{\FAtwo\symbol{143}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FAtwo\symbol{144}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FAtwo\symbol{145}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FAtwo\symbol{146}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FAtwo\symbol{147}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FAtwo\symbol{148}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FAtwo\symbol{149}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FAtwo\symbol{150}}}
\expandafter\def\csname faicon@heart\endcsname{{\FAtwo\symbol{151}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FAtwo\symbol{152}}}
\expandafter\def\csname faicon@home\endcsname{{\FAtwo\symbol{153}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FAtwo\symbol{154}}}
\expandafter\def\csname faicon@html5\endcsname{{\FAtwo\symbol{155}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FAtwo\symbol{156}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FAtwo\symbol{157}}}
\expandafter\def\csname faicon@indent\endcsname{{\FAtwo\symbol{158}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FAtwo\symbol{159}}}
\expandafter\def\csname faicon@inr\endcsname{{\FAtwo\symbol{160}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FAtwo\symbol{161}}}
\expandafter\def\csname faicon@italic\endcsname{{\FAtwo\symbol{162}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FAtwo\symbol{163}}}
\expandafter\def\csname faicon@key\endcsname{{\FAtwo\symbol{164}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FAtwo\symbol{165}}}
\expandafter\def\csname faicon@krw\endcsname{{\FAtwo\symbol{166}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FAtwo\symbol{167}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FAtwo\symbol{168}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FAtwo\symbol{169}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FAtwo\symbol{170}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FAtwo\symbol{171}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FAtwo\symbol{172}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FAtwo\symbol{173}}}
\expandafter\def\csname faicon@link\endcsname{{\FAtwo\symbol{174}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FAtwo\symbol{175}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FAtwo\symbol{176}}}
\expandafter\def\csname faicon@linux\endcsname{{\FAtwo\symbol{177}}}
\expandafter\def\csname faicon@list\endcsname{{\FAtwo\symbol{178}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FAtwo\symbol{179}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FAtwo\symbol{180}}}
\expandafter\def\csname faicon@lock\endcsname{{\FAtwo\symbol{181}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FAtwo\symbol{182}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FAtwo\symbol{183}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FAtwo\symbol{184}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FAtwo\symbol{185}}}
\expandafter\def\csname faicon@magic\endcsname{{\FAtwo\symbol{186}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FAtwo\symbol{187}}}
\expandafter\def\csname faicon@male\endcsname{{\FAtwo\symbol{188}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FAtwo\symbol{189}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FAtwo\symbol{190}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FAtwo\symbol{191}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FAtwo\symbol{192}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FAtwo\symbol{193}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FAtwo\symbol{194}}}
\expandafter\def\csname faicon@minus\endcsname{{\FAtwo\symbol{195}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FAtwo\symbol{196}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FAtwo\symbol{197}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FAtwo\symbol{198}}}
\expandafter\def\csname faicon@money\endcsname{{\FAtwo\symbol{199}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FAtwo\symbol{200}}}
\expandafter\def\csname faicon@music\endcsname{{\FAtwo\symbol{201}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FAtwo\symbol{202}}}
\expandafter\def\csname faicon@check\endcsname{{\FAtwo\symbol{203}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FAtwo\symbol{204}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FAtwo\symbol{205}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FAtwo\symbol{206}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FAtwo\symbol{207}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FAtwo\symbol{208}}}
\expandafter\def\csname faicon@pause\endcsname{{\FAtwo\symbol{209}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FAtwo\symbol{210}}}
\expandafter\def\csname faicon@phone\endcsname{{\FAtwo\symbol{211}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FAtwo\symbol{212}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FAtwo\symbol{213}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FAtwo\symbol{214}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FAtwo\symbol{215}}}
\expandafter\def\csname faicon@plane\endcsname{{\FAtwo\symbol{216}}}
\expandafter\def\csname faicon@play\endcsname{{\FAtwo\symbol{217}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FAtwo\symbol{218}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FAtwo\symbol{219}}}
\expandafter\def\csname faicon@plus\endcsname{{\FAtwo\symbol{220}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FAtwo\symbol{221}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FAtwo\symbol{222}}}
\expandafter\def\csname faicon@print\endcsname{{\FAtwo\symbol{223}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FAtwo\symbol{224}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FAtwo\symbol{225}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FAtwo\symbol{226}}}
\expandafter\def\csname faicon@question\endcsname{{\FAtwo\symbol{227}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FAtwo\symbol{228}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FAtwo\symbol{229}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FAtwo\symbol{230}}}
\expandafter\def\csname faicon@random\endcsname{{\FAtwo\symbol{231}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FAtwo\symbol{232}}}
\expandafter\def\csname faicon@times\endcsname{{\FAtwo\symbol{233}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FAtwo\symbol{234}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FAtwo\symbol{235}}}
\expandafter\def\csname faicon@renren\endcsname{{\FAtwo\symbol{236}}}
\expandafter\def\csname faicon@bars\endcsname{{\FAtwo\symbol{237}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FAtwo\symbol{238}}}
\expandafter\def\csname faicon@reply\endcsname{{\FAtwo\symbol{239}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FAtwo\symbol{240}}}
\expandafter\def\csname faicon@expand\endcsname{{\FAtwo\symbol{241}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FAtwo\symbol{242}}}
\expandafter\def\csname faicon@compress\endcsname{{\FAtwo\symbol{243}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FAtwo\symbol{244}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FAtwo\symbol{245}}}
\expandafter\def\csname faicon@road\endcsname{{\FAtwo\symbol{246}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FAtwo\symbol{247}}}
\expandafter\def\csname faicon@rss\endcsname{{\FAtwo\symbol{248}}}
\expandafter\def\csname faicon@rub\endcsname{{\FAtwo\symbol{249}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FAtwo\symbol{250}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FAtwo\symbol{251}}}
\expandafter\def\csname faicon@search\endcsname{{\FAtwo\symbol{252}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FAtwo\symbol{253}}}
\expandafter\def\csname faicon@share\endcsname{{\FAtwo\symbol{254}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FAtwo\symbol{255}}}
\expandafter\def\csname faicon@shield\endcsname{{\FAthree\symbol{0}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FAthree\symbol{1}}}
\expandafter\def\csname faicon@square\endcsname{{\FAthree\symbol{2}}}
\expandafter\def\csname faicon@signal\endcsname{{\FAthree\symbol{3}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FAthree\symbol{4}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FAthree\symbol{5}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FAthree\symbol{6}}}
\expandafter\def\csname faicon@skype\endcsname{{\FAthree\symbol{7}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FAthree\symbol{8}}}
\expandafter\def\csname faicon@sort\endcsname{{\FAthree\symbol{9}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FAthree\symbol{10}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FAthree\symbol{11}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FAthree\symbol{12}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FAthree\symbol{13}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FAthree\symbol{14}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FAthree\symbol{15}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FAthree\symbol{16}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FAthree\symbol{17}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FAthree\symbol{18}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FAthree\symbol{19}}}
\expandafter\def\csname faicon@star\endcsname{{\FAthree\symbol{20}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FAthree\symbol{21}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FAthree\symbol{22}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FAthree\symbol{23}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FAthree\symbol{24}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FAthree\symbol{25}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FAthree\symbol{26}}}
\expandafter\def\csname faicon@stop\endcsname{{\FAthree\symbol{27}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FAthree\symbol{28}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FAthree\symbol{29}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FAthree\symbol{30}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FAthree\symbol{31}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FAthree\symbol{32}}}
\expandafter\def\csname faicon@table\endcsname{{\FAthree\symbol{33}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FAthree\symbol{34}}}
\expandafter\def\csname faicon@tag\endcsname{{\FAthree\symbol{35}}}
\expandafter\def\csname faicon@tags\endcsname{{\FAthree\symbol{36}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FAthree\symbol{37}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FAthree\symbol{38}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FAthree\symbol{39}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FAthree\symbol{40}}}
\expandafter\def\csname faicon@th\endcsname{{\FAthree\symbol{41}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FAthree\symbol{42}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FAthree\symbol{43}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FAthree\symbol{44}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FAthree\symbol{45}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FAthree\symbol{46}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FAthree\symbol{47}}}
\expandafter\def\csname faicon@tint\endcsname{{\FAthree\symbol{48}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FAthree\symbol{49}}}
\expandafter\def\csname faicon@trello\endcsname{{\FAthree\symbol{50}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FAthree\symbol{51}}}
\expandafter\def\csname faicon@truck\endcsname{{\FAthree\symbol{52}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FAthree\symbol{53}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FAthree\symbol{54}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FAthree\symbol{55}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FAthree\symbol{56}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FAthree\symbol{57}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FAthree\symbol{58}}}
\expandafter\def\csname faicon@underline\endcsname{{\FAthree\symbol{59}}}
\expandafter\def\csname faicon@undo\endcsname{{\FAthree\symbol{60}}}
\expandafter\def\csname faicon@google\endcsname{{\FAthree\symbol{61}}}
\expandafter\def\csname faicon@paw\endcsname{{\FAthree\symbol{62}}}
\expandafter\def\csname faicon@database\endcsname{{\FAthree\symbol{63}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FAthree\symbol{64}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FAthree\symbol{65}}}
\expandafter\def\csname faicon@empire\endcsname{{\FAthree\symbol{66}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FAthree\symbol{67}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FAthree\symbol{68}}}
\expandafter\def\csname faicon@qq\endcsname{{\FAthree\symbol{69}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FAthree\symbol{70}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FAthree\symbol{71}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FAthree\symbol{72}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FAthree\symbol{73}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FAthree\symbol{74}}}
\expandafter\def\csname faicon@modx\endcsname{{\FAthree\symbol{75}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FAthree\symbol{76}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FAthree\symbol{77}}}
\expandafter\def\csname faicon@braille\endcsname{{\FAthree\symbol{78}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FAthree\symbol{79}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FAthree\symbol{80}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FAthree\symbol{81}}}
\expandafter\def\csname faicon@glide\endcsname{{\FAthree\symbol{82}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FAthree\symbol{83}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FAthree\symbol{84}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FAthree\symbol{85}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FAthree\symbol{86}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FAthree\symbol{87}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FAthree\symbol{88}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FAthree\symbol{89}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FAthree\symbol{90}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FAthree\symbol{91}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FAthree\symbol{92}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FAthree\symbol{93}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FAthree\symbol{94}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FAthree\symbol{95}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FAthree\symbol{96}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FAthree\symbol{97}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FAthree\symbol{98}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FAthree\symbol{99}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FAthree\symbol{100}}}
\expandafter\def\csname faicon@upload\endcsname{{\FAthree\symbol{101}}}
\expandafter\def\csname faicon@usd\endcsname{{\FAthree\symbol{102}}}
\expandafter\def\csname faicon@user\endcsname{{\FAthree\symbol{103}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FAthree\symbol{104}}}
\expandafter\def\csname faicon@venus\endcsname{{\FAthree\symbol{105}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FAthree\symbol{106}}}
\expandafter\def\csname faicon@vk\endcsname{{\FAthree\symbol{107}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FAthree\symbol{108}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FAthree\symbol{109}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FAthree\symbol{110}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FAthree\symbol{111}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FAthree\symbol{112}}}
\expandafter\def\csname faicon@windows\endcsname{{\FAthree\symbol{113}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FAthree\symbol{114}}}
\expandafter\def\csname faicon@xing\endcsname{{\FAthree\symbol{115}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FAthree\symbol{116}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FAthree\symbol{117}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FAthree\symbol{118}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FAthree\symbol{119}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FAthree\symbol{120}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FAthree\symbol{121}}}

%% end of file `fontawesomesymbols-pdftex.tex'.


==> fontawesomesymbols-xeluatex.tex <==
\expandafter\def\csname faicon@glass\endcsname{{\FA\symbol{"F000}}}
\expandafter\def\csname faicon@music\endcsname{{\FA\symbol{"F001}}}
\expandafter\def\csname faicon@search\endcsname{{\FA\symbol{"F002}}}
\expandafter\def\csname faicon@envelope-o\endcsname{{\FA\symbol{"F003}}}
\expandafter\def\csname faicon@heart\endcsname{{\FA\symbol{"F004}}}
\expandafter\def\csname faicon@star\endcsname{{\FA\symbol{"F005}}}
\expandafter\def\csname faicon@star-o\endcsname{{\FA\symbol{"F006}}}
\expandafter\def\csname faicon@user\endcsname{{\FA\symbol{"F007}}}
\expandafter\def\csname faicon@film\endcsname{{\FA\symbol{"F008}}}
\expandafter\def\csname faicon@th-large\endcsname{{\FA\symbol{"F009}}}
\expandafter\def\csname faicon@th\endcsname{{\FA\symbol{"F00A}}}
\expandafter\def\csname faicon@th-list\endcsname{{\FA\symbol{"F00B}}}
\expandafter\def\csname faicon@check\endcsname{{\FA\symbol{"F00C}}}
\expandafter\def\csname faicon@times\endcsname{{\FA\symbol{"F00D}}}
\expandafter\def\csname faicon@search-plus\endcsname{{\FA\symbol{"F00E}}}
\expandafter\def\csname faicon@search-minus\endcsname{{\FA\symbol{"F010}}}
\expandafter\def\csname faicon@power-off\endcsname{{\FA\symbol{"F011}}}
\expandafter\def\csname faicon@signal\endcsname{{\FA\symbol{"F012}}}
\expandafter\def\csname faicon@cog\endcsname{{\FA\symbol{"F013}}}
\expandafter\def\csname faicon@trash-o\endcsname{{\FA\symbol{"F014}}}
\expandafter\def\csname faicon@home\endcsname{{\FA\symbol{"F015}}}
\expandafter\def\csname faicon@file-o\endcsname{{\FA\symbol{"F016}}}
\expandafter\def\csname faicon@clock-o\endcsname{{\FA\symbol{"F017}}}
\expandafter\def\csname faicon@road\endcsname{{\FA\symbol{"F018}}}
\expandafter\def\csname faicon@download\endcsname{{\FA\symbol{"F019}}}
\expandafter\def\csname faicon@arrow-circle-o-down\endcsname{{\FA\symbol{"F01A}}}
\expandafter\def\csname faicon@arrow-circle-o-up\endcsname{{\FA\symbol{"F01B}}}
\expandafter\def\csname faicon@inbox\endcsname{{\FA\symbol{"F01C}}}
\expandafter\def\csname faicon@play-circle-o\endcsname{{\FA\symbol{"F01D}}}
\expandafter\def\csname faicon@repeat\endcsname{{\FA\symbol{"F01E}}}
\expandafter\def\csname faicon@refresh\endcsname{{\FA\symbol{"F021}}}
\expandafter\def\csname faicon@list-alt\endcsname{{\FA\symbol{"F022}}}
\expandafter\def\csname faicon@lock\endcsname{{\FA\symbol{"F023}}}
\expandafter\def\csname faicon@flag\endcsname{{\FA\symbol{"F024}}}
\expandafter\def\csname faicon@headphones\endcsname{{\FA\symbol{"F025}}}
\expandafter\def\csname faicon@volume-off\endcsname{{\FA\symbol{"F026}}}
\expandafter\def\csname faicon@volume-down\endcsname{{\FA\symbol{"F027}}}
\expandafter\def\csname faicon@volume-up\endcsname{{\FA\symbol{"F028}}}
\expandafter\def\csname faicon@qrcode\endcsname{{\FA\symbol{"F029}}}
\expandafter\def\csname faicon@barcode\endcsname{{\FA\symbol{"F02A}}}
\expandafter\def\csname faicon@tag\endcsname{{\FA\symbol{"F02B}}}
\expandafter\def\csname faicon@tags\endcsname{{\FA\symbol{"F02C}}}
\expandafter\def\csname faicon@book\endcsname{{\FA\symbol{"F02D}}}
\expandafter\def\csname faicon@bookmark\endcsname{{\FA\symbol{"F02E}}}
\expandafter\def\csname faicon@print\endcsname{{\FA\symbol{"F02F}}}
\expandafter\def\csname faicon@camera\endcsname{{\FA\symbol{"F030}}}
\expandafter\def\csname faicon@font\endcsname{{\FA\symbol{"F031}}}
\expandafter\def\csname faicon@bold\endcsname{{\FA\symbol{"F032}}}
\expandafter\def\csname faicon@italic\endcsname{{\FA\symbol{"F033}}}
\expandafter\def\csname faicon@text-height\endcsname{{\FA\symbol{"F034}}}
\expandafter\def\csname faicon@text-width\endcsname{{\FA\symbol{"F035}}}
\expandafter\def\csname faicon@align-left\endcsname{{\FA\symbol{"F036}}}
\expandafter\def\csname faicon@align-center\endcsname{{\FA\symbol{"F037}}}
\expandafter\def\csname faicon@align-right\endcsname{{\FA\symbol{"F038}}}
\expandafter\def\csname faicon@align-justify\endcsname{{\FA\symbol{"F039}}}
\expandafter\def\csname faicon@list\endcsname{{\FA\symbol{"F03A}}}
\expandafter\def\csname faicon@outdent\endcsname{{\FA\symbol{"F03B}}}
\expandafter\def\csname faicon@indent\endcsname{{\FA\symbol{"F03C}}}
\expandafter\def\csname faicon@video-camera\endcsname{{\FA\symbol{"F03D}}}
\expandafter\def\csname faicon@picture-o\endcsname{{\FA\symbol{"F03E}}}
\expandafter\def\csname faicon@pencil\endcsname{{\FA\symbol{"F040}}}
\expandafter\def\csname faicon@map-marker\endcsname{{\FA\symbol{"F041}}}
\expandafter\def\csname faicon@adjust\endcsname{{\FA\symbol{"F042}}}
\expandafter\def\csname faicon@tint\endcsname{{\FA\symbol{"F043}}}
\expandafter\def\csname faicon@pencil-square-o\endcsname{{\FA\symbol{"F044}}}
\expandafter\def\csname faicon@share-square-o\endcsname{{\FA\symbol{"F045}}}
\expandafter\def\csname faicon@check-square-o\endcsname{{\FA\symbol{"F046}}}
\expandafter\def\csname faicon@arrows\endcsname{{\FA\symbol{"F047}}}
\expandafter\def\csname faicon@step-backward\endcsname{{\FA\symbol{"F048}}}
\expandafter\def\csname faicon@fast-backward\endcsname{{\FA\symbol{"F049}}}
\expandafter\def\csname faicon@backward\endcsname{{\FA\symbol{"F04A}}}
\expandafter\def\csname faicon@play\endcsname{{\FA\symbol{"F04B}}}
\expandafter\def\csname faicon@pause\endcsname{{\FA\symbol{"F04C}}}
\expandafter\def\csname faicon@stop\endcsname{{\FA\symbol{"F04D}}}
\expandafter\def\csname faicon@forward\endcsname{{\FA\symbol{"F04E}}}
\expandafter\def\csname faicon@fast-forward\endcsname{{\FA\symbol{"F050}}}
\expandafter\def\csname faicon@step-forward\endcsname{{\FA\symbol{"F051}}}
\expandafter\def\csname faicon@eject\endcsname{{\FA\symbol{"F052}}}
\expandafter\def\csname faicon@chevron-left\endcsname{{\FA\symbol{"F053}}}
\expandafter\def\csname faicon@chevron-right\endcsname{{\FA\symbol{"F054}}}
\expandafter\def\csname faicon@plus-circle\endcsname{{\FA\symbol{"F055}}}
\expandafter\def\csname faicon@minus-circle\endcsname{{\FA\symbol{"F056}}}
\expandafter\def\csname faicon@times-circle\endcsname{{\FA\symbol{"F057}}}
\expandafter\def\csname faicon@check-circle\endcsname{{\FA\symbol{"F058}}}
\expandafter\def\csname faicon@question-circle\endcsname{{\FA\symbol{"F059}}}
\expandafter\def\csname faicon@info-circle\endcsname{{\FA\symbol{"F05A}}}
\expandafter\def\csname faicon@crosshairs\endcsname{{\FA\symbol{"F05B}}}
\expandafter\def\csname faicon@times-circle-o\endcsname{{\FA\symbol{"F05C}}}
\expandafter\def\csname faicon@check-circle-o\endcsname{{\FA\symbol{"F05D}}}
\expandafter\def\csname faicon@ban\endcsname{{\FA\symbol{"F05E}}}
\expandafter\def\csname faicon@arrow-left\endcsname{{\FA\symbol{"F060}}}
\expandafter\def\csname faicon@arrow-right\endcsname{{\FA\symbol{"F061}}}
\expandafter\def\csname faicon@arrow-up\endcsname{{\FA\symbol{"F062}}}
\expandafter\def\csname faicon@arrow-down\endcsname{{\FA\symbol{"F063}}}
\expandafter\def\csname faicon@share\endcsname{{\FA\symbol{"F064}}}
\expandafter\def\csname faicon@expand\endcsname{{\FA\symbol{"F065}}}
\expandafter\def\csname faicon@compress\endcsname{{\FA\symbol{"F066}}}
\expandafter\def\csname faicon@plus\endcsname{{\FA\symbol{"F067}}}
\expandafter\def\csname faicon@minus\endcsname{{\FA\symbol{"F068}}}
\expandafter\def\csname faicon@asterisk\endcsname{{\FA\symbol{"F069}}}
\expandafter\def\csname faicon@exclamation-circle\endcsname{{\FA\symbol{"F06A}}}
\expandafter\def\csname faicon@gift\endcsname{{\FA\symbol{"F06B}}}
\expandafter\def\csname faicon@leaf\endcsname{{\FA\symbol{"F06C}}}
\expandafter\def\csname faicon@fire\endcsname{{\FA\symbol{"F06D}}}
\expandafter\def\csname faicon@eye\endcsname{{\FA\symbol{"F06E}}}
\expandafter\def\csname faicon@eye-slash\endcsname{{\FA\symbol{"F070}}}
\expandafter\def\csname faicon@exclamation-triangle\endcsname{{\FA\symbol{"F071}}}
\expandafter\def\csname faicon@plane\endcsname{{\FA\symbol{"F072}}}
\expandafter\def\csname faicon@calendar\endcsname{{\FA\symbol{"F073}}}
\expandafter\def\csname faicon@random\endcsname{{\FA\symbol{"F074}}}
\expandafter\def\csname faicon@comment\endcsname{{\FA\symbol{"F075}}}
\expandafter\def\csname faicon@magnet\endcsname{{\FA\symbol{"F076}}}
\expandafter\def\csname faicon@chevron-up\endcsname{{\FA\symbol{"F077}}}
\expandafter\def\csname faicon@chevron-down\endcsname{{\FA\symbol{"F078}}}
\expandafter\def\csname faicon@retweet\endcsname{{\FA\symbol{"F079}}}
\expandafter\def\csname faicon@shopping-cart\endcsname{{\FA\symbol{"F07A}}}
\expandafter\def\csname faicon@folder\endcsname{{\FA\symbol{"F07B}}}
\expandafter\def\csname faicon@folder-open\endcsname{{\FA\symbol{"F07C}}}
\expandafter\def\csname faicon@arrows-v\endcsname{{\FA\symbol{"F07D}}}
\expandafter\def\csname faicon@arrows-h\endcsname{{\FA\symbol{"F07E}}}
\expandafter\def\csname faicon@bar-chart\endcsname{{\FA\symbol{"F080}}}
\expandafter\def\csname faicon@twitter-square\endcsname{{\FA\symbol{"F081}}}
\expandafter\def\csname faicon@facebook-square\endcsname{{\FA\symbol{"F082}}}
\expandafter\def\csname faicon@camera-retro\endcsname{{\FA\symbol{"F083}}}
\expandafter\def\csname faicon@key\endcsname{{\FA\symbol{"F084}}}
\expandafter\def\csname faicon@cogs\endcsname{{\FA\symbol{"F085}}}
\expandafter\def\csname faicon@comments\endcsname{{\FA\symbol{"F086}}}
\expandafter\def\csname faicon@thumbs-o-up\endcsname{{\FA\symbol{"F087}}}
\expandafter\def\csname faicon@thumbs-o-down\endcsname{{\FA\symbol{"F088}}}
\expandafter\def\csname faicon@star-half\endcsname{{\FA\symbol{"F089}}}
\expandafter\def\csname faicon@heart-o\endcsname{{\FA\symbol{"F08A}}}
\expandafter\def\csname faicon@sign-out\endcsname{{\FA\symbol{"F08B}}}
\expandafter\def\csname faicon@linkedin-square\endcsname{{\FA\symbol{"F08C}}}
\expandafter\def\csname faicon@thumb-tack\endcsname{{\FA\symbol{"F08D}}}
\expandafter\def\csname faicon@external-link\endcsname{{\FA\symbol{"F08E}}}
\expandafter\def\csname faicon@sign-in\endcsname{{\FA\symbol{"F090}}}
\expandafter\def\csname faicon@trophy\endcsname{{\FA\symbol{"F091}}}
\expandafter\def\csname faicon@github-square\endcsname{{\FA\symbol{"F092}}}
\expandafter\def\csname faicon@upload\endcsname{{\FA\symbol{"F093}}}
\expandafter\def\csname faicon@lemon-o\endcsname{{\FA\symbol{"F094}}}
\expandafter\def\csname faicon@phone\endcsname{{\FA\symbol{"F095}}}
\expandafter\def\csname faicon@square-o\endcsname{{\FA\symbol{"F096}}}
\expandafter\def\csname faicon@bookmark-o\endcsname{{\FA\symbol{"F097}}}
\expandafter\def\csname faicon@phone-square\endcsname{{\FA\symbol{"F098}}}
\expandafter\def\csname faicon@twitter\endcsname{{\FA\symbol{"F099}}}
\expandafter\def\csname faicon@facebook\endcsname{{\FA\symbol{"F09A}}}
\expandafter\def\csname faicon@github\endcsname{{\FA\symbol{"F09B}}}
\expandafter\def\csname faicon@unlock\endcsname{{\FA\symbol{"F09C}}}
\expandafter\def\csname faicon@credit-card\endcsname{{\FA\symbol{"F09D}}}
\expandafter\def\csname faicon@rss\endcsname{{\FA\symbol{"F09E}}}
\expandafter\def\csname faicon@hdd-o\endcsname{{\FA\symbol{"F0A0}}}
\expandafter\def\csname faicon@bullhorn\endcsname{{\FA\symbol{"F0A1}}}
\expandafter\def\csname faicon@bell\endcsname{{\FA\symbol{"F0F3}}}
\expandafter\def\csname faicon@certificate\endcsname{{\FA\symbol{"F0A3}}}
\expandafter\def\csname faicon@hand-o-right\endcsname{{\FA\symbol{"F0A4}}}
\expandafter\def\csname faicon@hand-o-left\endcsname{{\FA\symbol{"F0A5}}}
\expandafter\def\csname faicon@hand-o-up\endcsname{{\FA\symbol{"F0A6}}}
\expandafter\def\csname faicon@hand-o-down\endcsname{{\FA\symbol{"F0A7}}}
\expandafter\def\csname faicon@arrow-circle-left\endcsname{{\FA\symbol{"F0A8}}}
\expandafter\def\csname faicon@arrow-circle-right\endcsname{{\FA\symbol{"F0A9}}}
\expandafter\def\csname faicon@arrow-circle-up\endcsname{{\FA\symbol{"F0AA}}}
\expandafter\def\csname faicon@arrow-circle-down\endcsname{{\FA\symbol{"F0AB}}}
\expandafter\def\csname faicon@globe\endcsname{{\FA\symbol{"F0AC}}}
\expandafter\def\csname faicon@wrench\endcsname{{\FA\symbol{"F0AD}}}
\expandafter\def\csname faicon@tasks\endcsname{{\FA\symbol{"F0AE}}}
\expandafter\def\csname faicon@filter\endcsname{{\FA\symbol{"F0B0}}}
\expandafter\def\csname faicon@briefcase\endcsname{{\FA\symbol{"F0B1}}}
\expandafter\def\csname faicon@arrows-alt\endcsname{{\FA\symbol{"F0B2}}}
\expandafter\def\csname faicon@users\endcsname{{\FA\symbol{"F0C0}}}
\expandafter\def\csname faicon@link\endcsname{{\FA\symbol{"F0C1}}}
\expandafter\def\csname faicon@cloud\endcsname{{\FA\symbol{"F0C2}}}
\expandafter\def\csname faicon@flask\endcsname{{\FA\symbol{"F0C3}}}
\expandafter\def\csname faicon@scissors\endcsname{{\FA\symbol{"F0C4}}}
\expandafter\def\csname faicon@files-o\endcsname{{\FA\symbol{"F0C5}}}
\expandafter\def\csname faicon@paperclip\endcsname{{\FA\symbol{"F0C6}}}
\expandafter\def\csname faicon@floppy-o\endcsname{{\FA\symbol{"F0C7}}}
\expandafter\def\csname faicon@square\endcsname{{\FA\symbol{"F0C8}}}
\expandafter\def\csname faicon@bars\endcsname{{\FA\symbol{"F0C9}}}
\expandafter\def\csname faicon@list-ul\endcsname{{\FA\symbol{"F0CA}}}
\expandafter\def\csname faicon@list-ol\endcsname{{\FA\symbol{"F0CB}}}
\expandafter\def\csname faicon@strikethrough\endcsname{{\FA\symbol{"F0CC}}}
\expandafter\def\csname faicon@underline\endcsname{{\FA\symbol{"F0CD}}}
\expandafter\def\csname faicon@table\endcsname{{\FA\symbol{"F0CE}}}
\expandafter\def\csname faicon@magic\endcsname{{\FA\symbol{"F0D0}}}
\expandafter\def\csname faicon@truck\endcsname{{\FA\symbol{"F0D1}}}
\expandafter\def\csname faicon@pinterest\endcsname{{\FA\symbol{"F0D2}}}
\expandafter\def\csname faicon@pinterest-square\endcsname{{\FA\symbol{"F0D3}}}
\expandafter\def\csname faicon@google-plus-square\endcsname{{\FA\symbol{"F0D4}}}
\expandafter\def\csname faicon@google-plus\endcsname{{\FA\symbol{"F0D5}}}
\expandafter\def\csname faicon@money\endcsname{{\FA\symbol{"F0D6}}}
\expandafter\def\csname faicon@caret-down\endcsname{{\FA\symbol{"F0D7}}}
\expandafter\def\csname faicon@caret-up\endcsname{{\FA\symbol{"F0D8}}}
\expandafter\def\csname faicon@caret-left\endcsname{{\FA\symbol{"F0D9}}}
\expandafter\def\csname faicon@caret-right\endcsname{{\FA\symbol{"F0DA}}}
\expandafter\def\csname faicon@columns\endcsname{{\FA\symbol{"F0DB}}}
\expandafter\def\csname faicon@sort\endcsname{{\FA\symbol{"F0DC}}}
\expandafter\def\csname faicon@sort-desc\endcsname{{\FA\symbol{"F0DD}}}
\expandafter\def\csname faicon@sort-asc\endcsname{{\FA\symbol{"F0DE}}}
\expandafter\def\csname faicon@envelope\endcsname{{\FA\symbol{"F0E0}}}
\expandafter\def\csname faicon@linkedin\endcsname{{\FA\symbol{"F0E1}}}
\expandafter\def\csname faicon@undo\endcsname{{\FA\symbol{"F0E2}}}
\expandafter\def\csname faicon@gavel\endcsname{{\FA\symbol{"F0E3}}}
\expandafter\def\csname faicon@tachometer\endcsname{{\FA\symbol{"F0E4}}}
\expandafter\def\csname faicon@comment-o\endcsname{{\FA\symbol{"F0E5}}}
\expandafter\def\csname faicon@comments-o\endcsname{{\FA\symbol{"F0E6}}}
\expandafter\def\csname faicon@bolt\endcsname{{\FA\symbol{"F0E7}}}
\expandafter\def\csname faicon@sitemap\endcsname{{\FA\symbol{"F0E8}}}
\expandafter\def\csname faicon@umbrella\endcsname{{\FA\symbol{"F0E9}}}
\expandafter\def\csname faicon@clipboard\endcsname{{\FA\symbol{"F0EA}}}
\expandafter\def\csname faicon@lightbulb-o\endcsname{{\FA\symbol{"F0EB}}}
\expandafter\def\csname faicon@exchange\endcsname{{\FA\symbol{"F0EC}}}
\expandafter\def\csname faicon@cloud-download\endcsname{{\FA\symbol{"F0ED}}}
\expandafter\def\csname faicon@cloud-upload\endcsname{{\FA\symbol{"F0EE}}}
\expandafter\def\csname faicon@user-md\endcsname{{\FA\symbol{"F0F0}}}
\expandafter\def\csname faicon@stethoscope\endcsname{{\FA\symbol{"F0F1}}}
\expandafter\def\csname faicon@suitcase\endcsname{{\FA\symbol{"F0F2}}}
\expandafter\def\csname faicon@bell-o\endcsname{{\FA\symbol{"F0A2}}}
\expandafter\def\csname faicon@coffee\endcsname{{\FA\symbol{"F0F4}}}
\expandafter\def\csname faicon@cutlery\endcsname{{\FA\symbol{"F0F5}}}
\expandafter\def\csname faicon@file-text-o\endcsname{{\FA\symbol{"F0F6}}}
\expandafter\def\csname faicon@building-o\endcsname{{\FA\symbol{"F0F7}}}
\expandafter\def\csname faicon@hospital-o\endcsname{{\FA\symbol{"F0F8}}}
\expandafter\def\csname faicon@ambulance\endcsname{{\FA\symbol{"F0F9}}}
\expandafter\def\csname faicon@medkit\endcsname{{\FA\symbol{"F0FA}}}
\expandafter\def\csname faicon@fighter-jet\endcsname{{\FA\symbol{"F0FB}}}
\expandafter\def\csname faicon@beer\endcsname{{\FA\symbol{"F0FC}}}
\expandafter\def\csname faicon@h-square\endcsname{{\FA\symbol{"F0FD}}}
\expandafter\def\csname faicon@plus-square\endcsname{{\FA\symbol{"F0FE}}}
\expandafter\def\csname faicon@angle-double-left\endcsname{{\FA\symbol{"F100}}}
\expandafter\def\csname faicon@angle-double-right\endcsname{{\FA\symbol{"F101}}}
\expandafter\def\csname faicon@angle-double-up\endcsname{{\FA\symbol{"F102}}}
\expandafter\def\csname faicon@angle-double-down\endcsname{{\FA\symbol{"F103}}}
\expandafter\def\csname faicon@angle-left\endcsname{{\FA\symbol{"F104}}}
\expandafter\def\csname faicon@angle-right\endcsname{{\FA\symbol{"F105}}}
\expandafter\def\csname faicon@angle-up\endcsname{{\FA\symbol{"F106}}}
\expandafter\def\csname faicon@angle-down\endcsname{{\FA\symbol{"F107}}}
\expandafter\def\csname faicon@desktop\endcsname{{\FA\symbol{"F108}}}
\expandafter\def\csname faicon@laptop\endcsname{{\FA\symbol{"F109}}}
\expandafter\def\csname faicon@tablet\endcsname{{\FA\symbol{"F10A}}}
\expandafter\def\csname faicon@mobile\endcsname{{\FA\symbol{"F10B}}}
\expandafter\def\csname faicon@circle-o\endcsname{{\FA\symbol{"F10C}}}
\expandafter\def\csname faicon@quote-left\endcsname{{\FA\symbol{"F10D}}}
\expandafter\def\csname faicon@quote-right\endcsname{{\FA\symbol{"F10E}}}
\expandafter\def\csname faicon@spinner\endcsname{{\FA\symbol{"F110}}}
\expandafter\def\csname faicon@circle\endcsname{{\FA\symbol{"F111}}}
\expandafter\def\csname faicon@reply\endcsname{{\FA\symbol{"F112}}}
\expandafter\def\csname faicon@github-alt\endcsname{{\FA\symbol{"F113}}}
\expandafter\def\csname faicon@folder-o\endcsname{{\FA\symbol{"F114}}}
\expandafter\def\csname faicon@folder-open-o\endcsname{{\FA\symbol{"F115}}}
\expandafter\def\csname faicon@smile-o\endcsname{{\FA\symbol{"F118}}}
\expandafter\def\csname faicon@frown-o\endcsname{{\FA\symbol{"F119}}}
\expandafter\def\csname faicon@meh-o\endcsname{{\FA\symbol{"F11A}}}
\expandafter\def\csname faicon@gamepad\endcsname{{\FA\symbol{"F11B}}}
\expandafter\def\csname faicon@keyboard-o\endcsname{{\FA\symbol{"F11C}}}
\expandafter\def\csname faicon@flag-o\endcsname{{\FA\symbol{"F11D}}}
\expandafter\def\csname faicon@flag-checkered\endcsname{{\FA\symbol{"F11E}}}
\expandafter\def\csname faicon@terminal\endcsname{{\FA\symbol{"F120}}}
\expandafter\def\csname faicon@code\endcsname{{\FA\symbol{"F121}}}
\expandafter\def\csname faicon@reply-all\endcsname{{\FA\symbol{"F122}}}
\expandafter\def\csname faicon@star-half-o\endcsname{{\FA\symbol{"F123}}}
\expandafter\def\csname faicon@location-arrow\endcsname{{\FA\symbol{"F124}}}
\expandafter\def\csname faicon@crop\endcsname{{\FA\symbol{"F125}}}
\expandafter\def\csname faicon@code-fork\endcsname{{\FA\symbol{"F126}}}
\expandafter\def\csname faicon@chain-broken\endcsname{{\FA\symbol{"F127}}}
\expandafter\def\csname faicon@question\endcsname{{\FA\symbol{"F128}}}
\expandafter\def\csname faicon@info\endcsname{{\FA\symbol{"F129}}}
\expandafter\def\csname faicon@exclamation\endcsname{{\FA\symbol{"F12A}}}
\expandafter\def\csname faicon@superscript\endcsname{{\FA\symbol{"F12B}}}
\expandafter\def\csname faicon@subscript\endcsname{{\FA\symbol{"F12C}}}
\expandafter\def\csname faicon@eraser\endcsname{{\FA\symbol{"F12D}}}
\expandafter\def\csname faicon@puzzle-piece\endcsname{{\FA\symbol{"F12E}}}
\expandafter\def\csname faicon@microphone\endcsname{{\FA\symbol{"F130}}}
\expandafter\def\csname faicon@microphone-slash\endcsname{{\FA\symbol{"F131}}}
\expandafter\def\csname faicon@shield\endcsname{{\FA\symbol{"F132}}}
\expandafter\def\csname faicon@calendar-o\endcsname{{\FA\symbol{"F133}}}
\expandafter\def\csname faicon@fire-extinguisher\endcsname{{\FA\symbol{"F134}}}
\expandafter\def\csname faicon@rocket\endcsname{{\FA\symbol{"F135}}}
\expandafter\def\csname faicon@maxcdn\endcsname{{\FA\symbol{"F136}}}
\expandafter\def\csname faicon@chevron-circle-left\endcsname{{\FA\symbol{"F137}}}
\expandafter\def\csname faicon@chevron-circle-right\endcsname{{\FA\symbol{"F138}}}
\expandafter\def\csname faicon@chevron-circle-up\endcsname{{\FA\symbol{"F139}}}
\expandafter\def\csname faicon@chevron-circle-down\endcsname{{\FA\symbol{"F13A}}}
\expandafter\def\csname faicon@html5\endcsname{{\FA\symbol{"F13B}}}
\expandafter\def\csname faicon@css3\endcsname{{\FA\symbol{"F13C}}}
\expandafter\def\csname faicon@anchor\endcsname{{\FA\symbol{"F13D}}}
\expandafter\def\csname faicon@unlock-alt\endcsname{{\FA\symbol{"F13E}}}
\expandafter\def\csname faicon@bullseye\endcsname{{\FA\symbol{"F140}}}
\expandafter\def\csname faicon@ellipsis-h\endcsname{{\FA\symbol{"F141}}}
\expandafter\def\csname faicon@ellipsis-v\endcsname{{\FA\symbol{"F142}}}
\expandafter\def\csname faicon@rss-square\endcsname{{\FA\symbol{"F143}}}
\expandafter\def\csname faicon@play-circle\endcsname{{\FA\symbol{"F144}}}
\expandafter\def\csname faicon@ticket\endcsname{{\FA\symbol{"F145}}}
\expandafter\def\csname faicon@minus-square\endcsname{{\FA\symbol{"F146}}}
\expandafter\def\csname faicon@minus-square-o\endcsname{{\FA\symbol{"F147}}}
\expandafter\def\csname faicon@level-up\endcsname{{\FA\symbol{"F148}}}
\expandafter\def\csname faicon@level-down\endcsname{{\FA\symbol{"F149}}}
\expandafter\def\csname faicon@check-square\endcsname{{\FA\symbol{"F14A}}}
\expandafter\def\csname faicon@pencil-square\endcsname{{\FA\symbol{"F14B}}}
\expandafter\def\csname faicon@external-link-square\endcsname{{\FA\symbol{"F14C}}}
\expandafter\def\csname faicon@share-square\endcsname{{\FA\symbol{"F14D}}}
\expandafter\def\csname faicon@compass\endcsname{{\FA\symbol{"F14E}}}
\expandafter\def\csname faicon@caret-square-o-down\endcsname{{\FA\symbol{"F150}}}
\expandafter\def\csname faicon@caret-square-o-up\endcsname{{\FA\symbol{"F151}}}
\expandafter\def\csname faicon@caret-square-o-right\endcsname{{\FA\symbol{"F152}}}
\expandafter\def\csname faicon@eur\endcsname{{\FA\symbol{"F153}}}
\expandafter\def\csname faicon@gbp\endcsname{{\FA\symbol{"F154}}}
\expandafter\def\csname faicon@usd\endcsname{{\FA\symbol{"F155}}}
\expandafter\def\csname faicon@inr\endcsname{{\FA\symbol{"F156}}}
\expandafter\def\csname faicon@jpy\endcsname{{\FA\symbol{"F157}}}
\expandafter\def\csname faicon@rub\endcsname{{\FA\symbol{"F158}}}
\expandafter\def\csname faicon@krw\endcsname{{\FA\symbol{"F159}}}
\expandafter\def\csname faicon@btc\endcsname{{\FA\symbol{"F15A}}}
\expandafter\def\csname faicon@file\endcsname{{\FA\symbol{"F15B}}}
\expandafter\def\csname faicon@file-text\endcsname{{\FA\symbol{"F15C}}}
\expandafter\def\csname faicon@sort-alpha-asc\endcsname{{\FA\symbol{"F15D}}}
\expandafter\def\csname faicon@sort-alpha-desc\endcsname{{\FA\symbol{"F15E}}}
\expandafter\def\csname faicon@sort-amount-asc\endcsname{{\FA\symbol{"F160}}}
\expandafter\def\csname faicon@sort-amount-desc\endcsname{{\FA\symbol{"F161}}}
\expandafter\def\csname faicon@sort-numeric-asc\endcsname{{\FA\symbol{"F162}}}
\expandafter\def\csname faicon@sort-numeric-desc\endcsname{{\FA\symbol{"F163}}}
\expandafter\def\csname faicon@thumbs-up\endcsname{{\FA\symbol{"F164}}}
\expandafter\def\csname faicon@thumbs-down\endcsname{{\FA\symbol{"F165}}}
\expandafter\def\csname faicon@youtube-square\endcsname{{\FA\symbol{"F166}}}
\expandafter\def\csname faicon@youtube\endcsname{{\FA\symbol{"F167}}}
\expandafter\def\csname faicon@xing\endcsname{{\FA\symbol{"F168}}}
\expandafter\def\csname faicon@xing-square\endcsname{{\FA\symbol{"F169}}}
\expandafter\def\csname faicon@youtube-play\endcsname{{\FA\symbol{"F16A}}}
\expandafter\def\csname faicon@dropbox\endcsname{{\FA\symbol{"F16B}}}
\expandafter\def\csname faicon@stack-overflow\endcsname{{\FA\symbol{"F16C}}}
\expandafter\def\csname faicon@instagram\endcsname{{\FA\symbol{"F16D}}}
\expandafter\def\csname faicon@flickr\endcsname{{\FA\symbol{"F16E}}}
\expandafter\def\csname faicon@adn\endcsname{{\FA\symbol{"F170}}}
\expandafter\def\csname faicon@bitbucket\endcsname{{\FA\symbol{"F171}}}
\expandafter\def\csname faicon@bitbucket-square\endcsname{{\FA\symbol{"F172}}}
\expandafter\def\csname faicon@tumblr\endcsname{{\FA\symbol{"F173}}}
\expandafter\def\csname faicon@tumblr-square\endcsname{{\FA\symbol{"F174}}}
\expandafter\def\csname faicon@long-arrow-down\endcsname{{\FA\symbol{"F175}}}
\expandafter\def\csname faicon@long-arrow-up\endcsname{{\FA\symbol{"F176}}}
\expandafter\def\csname faicon@long-arrow-left\endcsname{{\FA\symbol{"F177}}}
\expandafter\def\csname faicon@long-arrow-right\endcsname{{\FA\symbol{"F178}}}
\expandafter\def\csname faicon@apple\endcsname{{\FA\symbol{"F179}}}
\expandafter\def\csname faicon@windows\endcsname{{\FA\symbol{"F17A}}}
\expandafter\def\csname faicon@android\endcsname{{\FA\symbol{"F17B}}}
\expandafter\def\csname faicon@linux\endcsname{{\FA\symbol{"F17C}}}
\expandafter\def\csname faicon@dribbble\endcsname{{\FA\symbol{"F17D}}}
\expandafter\def\csname faicon@skype\endcsname{{\FA\symbol{"F17E}}}
\expandafter\def\csname faicon@foursquare\endcsname{{\FA\symbol{"F180}}}
\expandafter\def\csname faicon@trello\endcsname{{\FA\symbol{"F181}}}
\expandafter\def\csname faicon@female\endcsname{{\FA\symbol{"F182}}}
\expandafter\def\csname faicon@male\endcsname{{\FA\symbol{"F183}}}
\expandafter\def\csname faicon@gratipay\endcsname{{\FA\symbol{"F184}}}
\expandafter\def\csname faicon@sun-o\endcsname{{\FA\symbol{"F185}}}
\expandafter\def\csname faicon@moon-o\endcsname{{\FA\symbol{"F186}}}
\expandafter\def\csname faicon@archive\endcsname{{\FA\symbol{"F187}}}
\expandafter\def\csname faicon@bug\endcsname{{\FA\symbol{"F188}}}
\expandafter\def\csname faicon@vk\endcsname{{\FA\symbol{"F189}}}
\expandafter\def\csname faicon@weibo\endcsname{{\FA\symbol{"F18A}}}
\expandafter\def\csname faicon@renren\endcsname{{\FA\symbol{"F18B}}}
\expandafter\def\csname faicon@pagelines\endcsname{{\FA\symbol{"F18C}}}
\expandafter\def\csname faicon@stack-exchange\endcsname{{\FA\symbol{"F18D}}}
\expandafter\def\csname faicon@arrow-circle-o-right\endcsname{{\FA\symbol{"F18E}}}
\expandafter\def\csname faicon@arrow-circle-o-left\endcsname{{\FA\symbol{"F190}}}
\expandafter\def\csname faicon@caret-square-o-left\endcsname{{\FA\symbol{"F191}}}
\expandafter\def\csname faicon@dot-circle-o\endcsname{{\FA\symbol{"F192}}}
\expandafter\def\csname faicon@wheelchair\endcsname{{\FA\symbol{"F193}}}
\expandafter\def\csname faicon@vimeo-square\endcsname{{\FA\symbol{"F194}}}
\expandafter\def\csname faicon@try\endcsname{{\FA\symbol{"F195}}}
\expandafter\def\csname faicon@plus-square-o\endcsname{{\FA\symbol{"F196}}}
\expandafter\def\csname faicon@space-shuttle\endcsname{{\FA\symbol{"F197}}}
\expandafter\def\csname faicon@slack\endcsname{{\FA\symbol{"F198}}}
\expandafter\def\csname faicon@envelope-square\endcsname{{\FA\symbol{"F199}}}
\expandafter\def\csname faicon@wordpress\endcsname{{\FA\symbol{"F19A}}}
\expandafter\def\csname faicon@openid\endcsname{{\FA\symbol{"F19B}}}
\expandafter\def\csname faicon@university\endcsname{{\FA\symbol{"F19C}}}
\expandafter\def\csname faicon@graduation-cap\endcsname{{\FA\symbol{"F19D}}}
\expandafter\def\csname faicon@yahoo\endcsname{{\FA\symbol{"F19E}}}
\expandafter\def\csname faicon@google\endcsname{{\FA\symbol{"F1A0}}}
\expandafter\def\csname faicon@reddit\endcsname{{\FA\symbol{"F1A1}}}
\expandafter\def\csname faicon@reddit-square\endcsname{{\FA\symbol{"F1A2}}}
\expandafter\def\csname faicon@stumbleupon-circle\endcsname{{\FA\symbol{"F1A3}}}
\expandafter\def\csname faicon@stumbleupon\endcsname{{\FA\symbol{"F1A4}}}
\expandafter\def\csname faicon@delicious\endcsname{{\FA\symbol{"F1A5}}}
\expandafter\def\csname faicon@digg\endcsname{{\FA\symbol{"F1A6}}}
\expandafter\def\csname faicon@pied-piper-pp\endcsname{{\FA\symbol{"F1A7}}}
\expandafter\def\csname faicon@pied-piper-alt\endcsname{{\FA\symbol{"F1A8}}}
\expandafter\def\csname faicon@drupal\endcsname{{\FA\symbol{"F1A9}}}
\expandafter\def\csname faicon@joomla\endcsname{{\FA\symbol{"F1AA}}}
\expandafter\def\csname faicon@language\endcsname{{\FA\symbol{"F1AB}}}
\expandafter\def\csname faicon@fax\endcsname{{\FA\symbol{"F1AC}}}
\expandafter\def\csname faicon@building\endcsname{{\FA\symbol{"F1AD}}}
\expandafter\def\csname faicon@child\endcsname{{\FA\symbol{"F1AE}}}
\expandafter\def\csname faicon@paw\endcsname{{\FA\symbol{"F1B0}}}
\expandafter\def\csname faicon@spoon\endcsname{{\FA\symbol{"F1B1}}}
\expandafter\def\csname faicon@cube\endcsname{{\FA\symbol{"F1B2}}}
\expandafter\def\csname faicon@cubes\endcsname{{\FA\symbol{"F1B3}}}
\expandafter\def\csname faicon@behance\endcsname{{\FA\symbol{"F1B4}}}
\expandafter\def\csname faicon@behance-square\endcsname{{\FA\symbol{"F1B5}}}
\expandafter\def\csname faicon@steam\endcsname{{\FA\symbol{"F1B6}}}
\expandafter\def\csname faicon@steam-square\endcsname{{\FA\symbol{"F1B7}}}
\expandafter\def\csname faicon@recycle\endcsname{{\FA\symbol{"F1B8}}}
\expandafter\def\csname faicon@car\endcsname{{\FA\symbol{"F1B9}}}
\expandafter\def\csname faicon@taxi\endcsname{{\FA\symbol{"F1BA}}}
\expandafter\def\csname faicon@tree\endcsname{{\FA\symbol{"F1BB}}}
\expandafter\def\csname faicon@spotify\endcsname{{\FA\symbol{"F1BC}}}
\expandafter\def\csname faicon@deviantart\endcsname{{\FA\symbol{"F1BD}}}
\expandafter\def\csname faicon@soundcloud\endcsname{{\FA\symbol{"F1BE}}}
\expandafter\def\csname faicon@database\endcsname{{\FA\symbol{"F1C0}}}
\expandafter\def\csname faicon@file-pdf-o\endcsname{{\FA\symbol{"F1C1}}}
\expandafter\def\csname faicon@file-word-o\endcsname{{\FA\symbol{"F1C2}}}
\expandafter\def\csname faicon@file-excel-o\endcsname{{\FA\symbol{"F1C3}}}
\expandafter\def\csname faicon@file-powerpoint-o\endcsname{{\FA\symbol{"F1C4}}}
\expandafter\def\csname faicon@file-image-o\endcsname{{\FA\symbol{"F1C5}}}
\expandafter\def\csname faicon@file-archive-o\endcsname{{\FA\symbol{"F1C6}}}
\expandafter\def\csname faicon@file-audio-o\endcsname{{\FA\symbol{"F1C7}}}
\expandafter\def\csname faicon@file-video-o\endcsname{{\FA\symbol{"F1C8}}}
\expandafter\def\csname faicon@file-code-o\endcsname{{\FA\symbol{"F1C9}}}
\expandafter\def\csname faicon@vine\endcsname{{\FA\symbol{"F1CA}}}
\expandafter\def\csname faicon@codepen\endcsname{{\FA\symbol{"F1CB}}}
\expandafter\def\csname faicon@jsfiddle\endcsname{{\FA\symbol{"F1CC}}}
\expandafter\def\csname faicon@life-ring\endcsname{{\FA\symbol{"F1CD}}}
\expandafter\def\csname faicon@circle-o-notch\endcsname{{\FA\symbol{"F1CE}}}
\expandafter\def\csname faicon@rebel\endcsname{{\FA\symbol{"F1D0}}}
\expandafter\def\csname faicon@empire\endcsname{{\FA\symbol{"F1D1}}}
\expandafter\def\csname faicon@git-square\endcsname{{\FA\symbol{"F1D2}}}
\expandafter\def\csname faicon@git\endcsname{{\FA\symbol{"F1D3}}}
\expandafter\def\csname faicon@hacker-news\endcsname{{\FA\symbol{"F1D4}}}
\expandafter\def\csname faicon@tencent-weibo\endcsname{{\FA\symbol{"F1D5}}}
\expandafter\def\csname faicon@qq\endcsname{{\FA\symbol{"F1D6}}}
\expandafter\def\csname faicon@weixin\endcsname{{\FA\symbol{"F1D7}}}
\expandafter\def\csname faicon@paper-plane\endcsname{{\FA\symbol{"F1D8}}}
\expandafter\def\csname faicon@paper-plane-o\endcsname{{\FA\symbol{"F1D9}}}
\expandafter\def\csname faicon@history\endcsname{{\FA\symbol{"F1DA}}}
\expandafter\def\csname faicon@circle-thin\endcsname{{\FA\symbol{"F1DB}}}
\expandafter\def\csname faicon@header\endcsname{{\FA\symbol{"F1DC}}}
\expandafter\def\csname faicon@paragraph\endcsname{{\FA\symbol{"F1DD}}}
\expandafter\def\csname faicon@sliders\endcsname{{\FA\symbol{"F1DE}}}
\expandafter\def\csname faicon@share-alt\endcsname{{\FA\symbol{"F1E0}}}
\expandafter\def\csname faicon@share-alt-square\endcsname{{\FA\symbol{"F1E1}}}
\expandafter\def\csname faicon@bomb\endcsname{{\FA\symbol{"F1E2}}}
\expandafter\def\csname faicon@futbol-o\endcsname{{\FA\symbol{"F1E3}}}
\expandafter\def\csname faicon@tty\endcsname{{\FA\symbol{"F1E4}}}
\expandafter\def\csname faicon@binoculars\endcsname{{\FA\symbol{"F1E5}}}
\expandafter\def\csname faicon@plug\endcsname{{\FA\symbol{"F1E6}}}
\expandafter\def\csname faicon@slideshare\endcsname{{\FA\symbol{"F1E7}}}
\expandafter\def\csname faicon@twitch\endcsname{{\FA\symbol{"F1E8}}}
\expandafter\def\csname faicon@yelp\endcsname{{\FA\symbol{"F1E9}}}
\expandafter\def\csname faicon@newspaper-o\endcsname{{\FA\symbol{"F1EA}}}
\expandafter\def\csname faicon@wifi\endcsname{{\FA\symbol{"F1EB}}}
\expandafter\def\csname faicon@calculator\endcsname{{\FA\symbol{"F1EC}}}
\expandafter\def\csname faicon@paypal\endcsname{{\FA\symbol{"F1ED}}}
\expandafter\def\csname faicon@google-wallet\endcsname{{\FA\symbol{"F1EE}}}
\expandafter\def\csname faicon@cc-visa\endcsname{{\FA\symbol{"F1F0}}}
\expandafter\def\csname faicon@cc-mastercard\endcsname{{\FA\symbol{"F1F1}}}
\expandafter\def\csname faicon@cc-discover\endcsname{{\FA\symbol{"F1F2}}}
\expandafter\def\csname faicon@cc-amex\endcsname{{\FA\symbol{"F1F3}}}
\expandafter\def\csname faicon@cc-paypal\endcsname{{\FA\symbol{"F1F4}}}
\expandafter\def\csname faicon@cc-stripe\endcsname{{\FA\symbol{"F1F5}}}
\expandafter\def\csname faicon@bell-slash\endcsname{{\FA\symbol{"F1F6}}}
\expandafter\def\csname faicon@bell-slash-o\endcsname{{\FA\symbol{"F1F7}}}
\expandafter\def\csname faicon@trash\endcsname{{\FA\symbol{"F1F8}}}
\expandafter\def\csname faicon@copyright\endcsname{{\FA\symbol{"F1F9}}}
\expandafter\def\csname faicon@at\endcsname{{\FA\symbol{"F1FA}}}
\expandafter\def\csname faicon@eyedropper\endcsname{{\FA\symbol{"F1FB}}}
\expandafter\def\csname faicon@paint-brush\endcsname{{\FA\symbol{"F1FC}}}
\expandafter\def\csname faicon@birthday-cake\endcsname{{\FA\symbol{"F1FD}}}
\expandafter\def\csname faicon@area-chart\endcsname{{\FA\symbol{"F1FE}}}
\expandafter\def\csname faicon@pie-chart\endcsname{{\FA\symbol{"F200}}}
\expandafter\def\csname faicon@line-chart\endcsname{{\FA\symbol{"F201}}}
\expandafter\def\csname faicon@lastfm\endcsname{{\FA\symbol{"F202}}}
\expandafter\def\csname faicon@lastfm-square\endcsname{{\FA\symbol{"F203}}}
\expandafter\def\csname faicon@toggle-off\endcsname{{\FA\symbol{"F204}}}
\expandafter\def\csname faicon@toggle-on\endcsname{{\FA\symbol{"F205}}}
\expandafter\def\csname faicon@bicycle\endcsname{{\FA\symbol{"F206}}}
\expandafter\def\csname faicon@bus\endcsname{{\FA\symbol{"F207}}}
\expandafter\def\csname faicon@ioxhost\endcsname{{\FA\symbol{"F208}}}
\expandafter\def\csname faicon@angellist\endcsname{{\FA\symbol{"F209}}}
\expandafter\def\csname faicon@cc\endcsname{{\FA\symbol{"F20A}}}
\expandafter\def\csname faicon@ils\endcsname{{\FA\symbol{"F20B}}}
\expandafter\def\csname faicon@meanpath\endcsname{{\FA\symbol{"F20C}}}
\expandafter\def\csname faicon@buysellads\endcsname{{\FA\symbol{"F20D}}}
\expandafter\def\csname faicon@connectdevelop\endcsname{{\FA\symbol{"F20E}}}
\expandafter\def\csname faicon@dashcube\endcsname{{\FA\symbol{"F210}}}
\expandafter\def\csname faicon@forumbee\endcsname{{\FA\symbol{"F211}}}
\expandafter\def\csname faicon@leanpub\endcsname{{\FA\symbol{"F212}}}
\expandafter\def\csname faicon@sellsy\endcsname{{\FA\symbol{"F213}}}
\expandafter\def\csname faicon@shirtsinbulk\endcsname{{\FA\symbol{"F214}}}
\expandafter\def\csname faicon@simplybuilt\endcsname{{\FA\symbol{"F215}}}
\expandafter\def\csname faicon@skyatlas\endcsname{{\FA\symbol{"F216}}}
\expandafter\def\csname faicon@cart-plus\endcsname{{\FA\symbol{"F217}}}
\expandafter\def\csname faicon@cart-arrow-down\endcsname{{\FA\symbol{"F218}}}
\expandafter\def\csname faicon@diamond\endcsname{{\FA\symbol{"F219}}}
\expandafter\def\csname faicon@ship\endcsname{{\FA\symbol{"F21A}}}
\expandafter\def\csname faicon@user-secret\endcsname{{\FA\symbol{"F21B}}}
\expandafter\def\csname faicon@motorcycle\endcsname{{\FA\symbol{"F21C}}}
\expandafter\def\csname faicon@street-view\endcsname{{\FA\symbol{"F21D}}}
\expandafter\def\csname faicon@heartbeat\endcsname{{\FA\symbol{"F21E}}}
\expandafter\def\csname faicon@venus\endcsname{{\FA\symbol{"F221}}}
\expandafter\def\csname faicon@mars\endcsname{{\FA\symbol{"F222}}}
\expandafter\def\csname faicon@mercury\endcsname{{\FA\symbol{"F223}}}
\expandafter\def\csname faicon@transgender\endcsname{{\FA\symbol{"F224}}}
\expandafter\def\csname faicon@transgender-alt\endcsname{{\FA\symbol{"F225}}}
\expandafter\def\csname faicon@venus-double\endcsname{{\FA\symbol{"F226}}}
\expandafter\def\csname faicon@mars-double\endcsname{{\FA\symbol{"F227}}}
\expandafter\def\csname faicon@venus-mars\endcsname{{\FA\symbol{"F228}}}
\expandafter\def\csname faicon@mars-stroke\endcsname{{\FA\symbol{"F229}}}
\expandafter\def\csname faicon@mars-stroke-v\endcsname{{\FA\symbol{"F22A}}}
\expandafter\def\csname faicon@mars-stroke-h\endcsname{{\FA\symbol{"F22B}}}
\expandafter\def\csname faicon@neuter\endcsname{{\FA\symbol{"F22C}}}
\expandafter\def\csname faicon@genderless\endcsname{{\FA\symbol{"F22D}}}
\expandafter\def\csname faicon@facebook-official\endcsname{{\FA\symbol{"F230}}}
\expandafter\def\csname faicon@pinterest-p\endcsname{{\FA\symbol{"F231}}}
\expandafter\def\csname faicon@whatsapp\endcsname{{\FA\symbol{"F232}}}
\expandafter\def\csname faicon@server\endcsname{{\FA\symbol{"F233}}}
\expandafter\def\csname faicon@user-plus\endcsname{{\FA\symbol{"F234}}}
\expandafter\def\csname faicon@user-times\endcsname{{\FA\symbol{"F235}}}
\expandafter\def\csname faicon@bed\endcsname{{\FA\symbol{"F236}}}
\expandafter\def\csname faicon@viacoin\endcsname{{\FA\symbol{"F237}}}
\expandafter\def\csname faicon@train\endcsname{{\FA\symbol{"F238}}}
\expandafter\def\csname faicon@subway\endcsname{{\FA\symbol{"F239}}}
\expandafter\def\csname faicon@medium\endcsname{{\FA\symbol{"F23A}}}
\expandafter\def\csname faicon@y-combinator\endcsname{{\FA\symbol{"F23B}}}
\expandafter\def\csname faicon@optin-monster\endcsname{{\FA\symbol{"F23C}}}
\expandafter\def\csname faicon@opencart\endcsname{{\FA\symbol{"F23D}}}
\expandafter\def\csname faicon@expeditedssl\endcsname{{\FA\symbol{"F23E}}}
\expandafter\def\csname faicon@battery-full\endcsname{{\FA\symbol{"F240}}}
\expandafter\def\csname faicon@battery-three-quarters\endcsname{{\FA\symbol{"F241}}}
\expandafter\def\csname faicon@battery-half\endcsname{{\FA\symbol{"F242}}}
\expandafter\def\csname faicon@battery-quarter\endcsname{{\FA\symbol{"F243}}}
\expandafter\def\csname faicon@battery-empty\endcsname{{\FA\symbol{"F244}}}
\expandafter\def\csname faicon@mouse-pointer\endcsname{{\FA\symbol{"F245}}}
\expandafter\def\csname faicon@i-cursor\endcsname{{\FA\symbol{"F246}}}
\expandafter\def\csname faicon@object-group\endcsname{{\FA\symbol{"F247}}}
\expandafter\def\csname faicon@object-ungroup\endcsname{{\FA\symbol{"F248}}}
\expandafter\def\csname faicon@sticky-note\endcsname{{\FA\symbol{"F249}}}
\expandafter\def\csname faicon@sticky-note-o\endcsname{{\FA\symbol{"F24A}}}
\expandafter\def\csname faicon@cc-jcb\endcsname{{\FA\symbol{"F24B}}}
\expandafter\def\csname faicon@cc-diners-club\endcsname{{\FA\symbol{"F24C}}}
\expandafter\def\csname faicon@clone\endcsname{{\FA\symbol{"F24D}}}
\expandafter\def\csname faicon@balance-scale\endcsname{{\FA\symbol{"F24E}}}
\expandafter\def\csname faicon@hourglass-o\endcsname{{\FA\symbol{"F250}}}
\expandafter\def\csname faicon@hourglass-start\endcsname{{\FA\symbol{"F251}}}
\expandafter\def\csname faicon@hourglass-half\endcsname{{\FA\symbol{"F252}}}
\expandafter\def\csname faicon@hourglass-end\endcsname{{\FA\symbol{"F253}}}
\expandafter\def\csname faicon@hourglass\endcsname{{\FA\symbol{"F254}}}
\expandafter\def\csname faicon@hand-rock-o\endcsname{{\FA\symbol{"F255}}}
\expandafter\def\csname faicon@hand-paper-o\endcsname{{\FA\symbol{"F256}}}
\expandafter\def\csname faicon@hand-scissors-o\endcsname{{\FA\symbol{"F257}}}
\expandafter\def\csname faicon@hand-lizard-o\endcsname{{\FA\symbol{"F258}}}
\expandafter\def\csname faicon@hand-spock-o\endcsname{{\FA\symbol{"F259}}}
\expandafter\def\csname faicon@hand-pointer-o\endcsname{{\FA\symbol{"F25A}}}
\expandafter\def\csname faicon@hand-peace-o\endcsname{{\FA\symbol{"F25B}}}
\expandafter\def\csname faicon@trademark\endcsname{{\FA\symbol{"F25C}}}
\expandafter\def\csname faicon@registered\endcsname{{\FA\symbol{"F25D}}}
\expandafter\def\csname faicon@creative-commons\endcsname{{\FA\symbol{"F25E}}}
\expandafter\def\csname faicon@gg\endcsname{{\FA\symbol{"F260}}}
\expandafter\def\csname faicon@gg-circle\endcsname{{\FA\symbol{"F261}}}
\expandafter\def\csname faicon@tripadvisor\endcsname{{\FA\symbol{"F262}}}
\expandafter\def\csname faicon@odnoklassniki\endcsname{{\FA\symbol{"F263}}}
\expandafter\def\csname faicon@odnoklassniki-square\endcsname{{\FA\symbol{"F264}}}
\expandafter\def\csname faicon@get-pocket\endcsname{{\FA\symbol{"F265}}}
\expandafter\def\csname faicon@wikipedia-w\endcsname{{\FA\symbol{"F266}}}
\expandafter\def\csname faicon@safari\endcsname{{\FA\symbol{"F267}}}
\expandafter\def\csname faicon@chrome\endcsname{{\FA\symbol{"F268}}}
\expandafter\def\csname faicon@firefox\endcsname{{\FA\symbol{"F269}}}
\expandafter\def\csname faicon@opera\endcsname{{\FA\symbol{"F26A}}}
\expandafter\def\csname faicon@internet-explorer\endcsname{{\FA\symbol{"F26B}}}
\expandafter\def\csname faicon@television\endcsname{{\FA\symbol{"F26C}}}
\expandafter\def\csname faicon@contao\endcsname{{\FA\symbol{"F26D}}}
\expandafter\def\csname faicon@500px\endcsname{{\FA\symbol{"F26E}}}
\expandafter\def\csname faicon@amazon\endcsname{{\FA\symbol{"F270}}}
\expandafter\def\csname faicon@calendar-plus-o\endcsname{{\FA\symbol{"F271}}}
\expandafter\def\csname faicon@calendar-minus-o\endcsname{{\FA\symbol{"F272}}}
\expandafter\def\csname faicon@calendar-times-o\endcsname{{\FA\symbol{"F273}}}
\expandafter\def\csname faicon@calendar-check-o\endcsname{{\FA\symbol{"F274}}}
\expandafter\def\csname faicon@industry\endcsname{{\FA\symbol{"F275}}}
\expandafter\def\csname faicon@map-pin\endcsname{{\FA\symbol{"F276}}}
\expandafter\def\csname faicon@map-signs\endcsname{{\FA\symbol{"F277}}}
\expandafter\def\csname faicon@map-o\endcsname{{\FA\symbol{"F278}}}
\expandafter\def\csname faicon@map\endcsname{{\FA\symbol{"F279}}}
\expandafter\def\csname faicon@commenting\endcsname{{\FA\symbol{"F27A}}}
\expandafter\def\csname faicon@commenting-o\endcsname{{\FA\symbol{"F27B}}}
\expandafter\def\csname faicon@houzz\endcsname{{\FA\symbol{"F27C}}}
\expandafter\def\csname faicon@vimeo\endcsname{{\FA\symbol{"F27D}}}
\expandafter\def\csname faicon@black-tie\endcsname{{\FA\symbol{"F27E}}}
\expandafter\def\csname faicon@fonticons\endcsname{{\FA\symbol{"F280}}}
\expandafter\def\csname faicon@reddit-alien\endcsname{{\FA\symbol{"F281}}}
\expandafter\def\csname faicon@edge\endcsname{{\FA\symbol{"F282}}}
\expandafter\def\csname faicon@credit-card-alt\endcsname{{\FA\symbol{"F283}}}
\expandafter\def\csname faicon@codiepie\endcsname{{\FA\symbol{"F284}}}
\expandafter\def\csname faicon@modx\endcsname{{\FA\symbol{"F285}}}
\expandafter\def\csname faicon@fort-awesome\endcsname{{\FA\symbol{"F286}}}
\expandafter\def\csname faicon@usb\endcsname{{\FA\symbol{"F287}}}
\expandafter\def\csname faicon@product-hunt\endcsname{{\FA\symbol{"F288}}}
\expandafter\def\csname faicon@mixcloud\endcsname{{\FA\symbol{"F289}}}
\expandafter\def\csname faicon@scribd\endcsname{{\FA\symbol{"F28A}}}
\expandafter\def\csname faicon@pause-circle\endcsname{{\FA\symbol{"F28B}}}
\expandafter\def\csname faicon@pause-circle-o\endcsname{{\FA\symbol{"F28C}}}
\expandafter\def\csname faicon@stop-circle\endcsname{{\FA\symbol{"F28D}}}
\expandafter\def\csname faicon@stop-circle-o\endcsname{{\FA\symbol{"F28E}}}
\expandafter\def\csname faicon@shopping-bag\endcsname{{\FA\symbol{"F290}}}
\expandafter\def\csname faicon@shopping-basket\endcsname{{\FA\symbol{"F291}}}
\expandafter\def\csname faicon@hashtag\endcsname{{\FA\symbol{"F292}}}
\expandafter\def\csname faicon@bluetooth\endcsname{{\FA\symbol{"F293}}}
\expandafter\def\csname faicon@bluetooth-b\endcsname{{\FA\symbol{"F294}}}
\expandafter\def\csname faicon@percent\endcsname{{\FA\symbol{"F295}}}
\expandafter\def\csname faicon@gitlab\endcsname{{\FA\symbol{"F296}}}
\expandafter\def\csname faicon@wpbeginner\endcsname{{\FA\symbol{"F297}}}
\expandafter\def\csname faicon@wpforms\endcsname{{\FA\symbol{"F298}}}
\expandafter\def\csname faicon@envira\endcsname{{\FA\symbol{"F299}}}
\expandafter\def\csname faicon@universal-access\endcsname{{\FA\symbol{"F29A}}}
\expandafter\def\csname faicon@wheelchair-alt\endcsname{{\FA\symbol{"F29B}}}
\expandafter\def\csname faicon@question-circle-o\endcsname{{\FA\symbol{"F29C}}}
\expandafter\def\csname faicon@blind\endcsname{{\FA\symbol{"F29D}}}
\expandafter\def\csname faicon@audio-description\endcsname{{\FA\symbol{"F29E}}}
\expandafter\def\csname faicon@volume-control-phone\endcsname{{\FA\symbol{"F2A0}}}
\expandafter\def\csname faicon@braille\endcsname{{\FA\symbol{"F2A1}}}
\expandafter\def\csname faicon@assistive-listening-systems\endcsname{{\FA\symbol{"F2A2}}}
\expandafter\def\csname faicon@american-sign-language-interpreting\endcsname{{\FA\symbol{"F2A3}}}
\expandafter\def\csname faicon@deaf\endcsname{{\FA\symbol{"F2A4}}}
\expandafter\def\csname faicon@glide\endcsname{{\FA\symbol{"F2A5}}}
\expandafter\def\csname faicon@glide-g\endcsname{{\FA\symbol{"F2A6}}}
\expandafter\def\csname faicon@sign-language\endcsname{{\FA\symbol{"F2A7}}}
\expandafter\def\csname faicon@low-vision\endcsname{{\FA\symbol{"F2A8}}}
\expandafter\def\csname faicon@viadeo\endcsname{{\FA\symbol{"F2A9}}}
\expandafter\def\csname faicon@viadeo-square\endcsname{{\FA\symbol{"F2AA}}}
\expandafter\def\csname faicon@snapchat\endcsname{{\FA\symbol{"F2AB}}}
\expandafter\def\csname faicon@snapchat-ghost\endcsname{{\FA\symbol{"F2AC}}}
\expandafter\def\csname faicon@snapchat-square\endcsname{{\FA\symbol{"F2AD}}}
\expandafter\def\csname faicon@pied-piper\endcsname{{\FA\symbol{"F2AE}}}
\expandafter\def\csname faicon@first-order\endcsname{{\FA\symbol{"F2B0}}}
\expandafter\def\csname faicon@yoast\endcsname{{\FA\symbol{"F2B1}}}
\expandafter\def\csname faicon@themeisle\endcsname{{\FA\symbol{"F2B2}}}
\expandafter\def\csname faicon@google-plus-official\endcsname{{\FA\symbol{"F2B3}}}
\expandafter\def\csname faicon@font-awesome\endcsname{{\FA\symbol{"F2B4}}}


==> implem.tex <==


We have implemented {\sc Code2Que} as a standalone web-based tool to assist developers in improving question titles in Stack Overflow.
The source code and data can be found in our Github repository\footnote{\url{https://github.com/beyondacm/Code2Que}}.

\smallskip
\noindent{\itshape\bfseries Data Collection}.
The data source of {\sc Code2Que} is from the Stack Overflow data dump of September 2019\footnote{\url{https://archive.org/details/stackexchange}}. We use the \textit{Python}, \textit{Java}, \textit{Javascript}, \textit{C\#} and \textit{SQL} tags to collect questions associated with the corresponding programming language. We extract the code snippet from each post's body by using $\langle$\textit{code}$\rangle$ tags, and then pair it with its question title if the question score is higher than 1. 
We have collected more than 1 million $\langle$\textit{code snippet}, \textit{question}$\rangle$ pairs from Stack Overflow for different programming languages.

\smallskip
\noindent{\itshape\bfseries Data Preprocessing}.
We preprocess our collected data according to the following steps: We first tokenize the code snippet and question title using the NLTK toolkit~\cite{bird2004nltk} (Step1). After that, to  avoid being overly context-specific, we use regular expressions to replace numbers and strings with special tokens ``NUMBER'' and ``STRING'' in code snippets (Step2). 
For question titles, we only keep the pairs if one of the interrogative keywords (e.g., ``how'', ``what'', ``why'', ``which'') appears in the question (Step3). Following that, we remove pairs where the code snippet and the question title are too long or too short. We set the token range from 16 tokens to 128 tokens for code snippets and from 4 tokens to 16 tokens for question titles respectively.  
The remaining $\langle$\textit{code snippet}, \textit{question}$\rangle$ pairs are added to our training corpus.

\begin{figure}[t]
    \centerline{\includegraphics[width=0.35\textwidth]{homepage-02.png}}
\vspace*{-10pt}
\caption{Homepage of Code2Que}
\vspace*{-0.5cm}
\label{fig:homepage}
\end{figure}

\smallskip
\noindent{\itshape\bfseries Backend Model}.
We use the framework OpenNMT~\cite{opennmt} to train our backend Model. 
We followed our previous experiment settings ~\cite{gao2020generating} for the training process.
The collected $\langle$\textit{question}, \textit{code snippet}$\rangle$ pairs are input into the workflow of our approach described in Section ~\ref{sec:approach}, and the output consists of the trained sequence-to-sequence model and the associated code embeddings which are used by {\sc Code2Que} as the backend model for online recommendation.

\smallskip
\noindent{\itshape\bfseries Frontend User Interface}.
%\subsection{Frontend User Interface}
Fig.~\ref{fig:homepage} shows the query page of {\sc Code2Que}.
{\sc Code2Que} provides an input box for developers to submit their source code snippet. After a developer submits his/her code snippet to the server, the code snippet is preprocessed and passed to our backend model. The outputs are organised into two separate result boxes for the generated question and retrieved questions respectively. For the generated question, {\sc Code2Que} generates a question title according to the code snippet.  For retrieved questions, {\sc Code2Que} returns the top-5 most similar questions in our code base together with the links to their Stack Overflow posts. 

\smallskip
\noindent{\itshape\bfseries System Optimization}.
To meet the efficiency requirement as an online web tool, we optimize the implementations of {\sc Code2Que}: 
(i) Considering that the offline learning model and code embeddings are frequently used in the online recommendation phase, we put them into cache to reduce redundant data loading. (ii) We created an index for the relevant questions in our database to speed up retrieval. (iii) We used locality sensitive hashing for fast nearest neighbour search in our large code embeddings data sets.




% \begin{figure}[t]
%     \centerline{\includegraphics[width=0.43\textwidth]{tool-bug-detection-print.pdf}}
% \vspace*{-10pt}
% \caption{Sample Results of Bug Detection}\vspace*{-0.6cm}
% \label{fig:tool-bug}
% \end{figure}

==> moti.tex <==
% 1.应该被删除的没有被删除
% 2.不应该被删除的被删除了
% In this section, we first show some motivating examples from Stack Overflow of the sorts of problems mentioned above (i.e., query mismatch and information overload), we then present the user scenarios of employing our approach to address these problems. 

We show several motivating examples from popular Github repositories of the sorts of problems mentioned above. We then present user scenarios of employing our proposed approach to address these problems.

\subsection{Motivating Examples}

\begin{figure}
% \vspace{-7pt}
\centerline{\includegraphics[width=0.50\textwidth]{motivating-example.pdf}}
% \vspace*{-5pt}
\caption{Motivating Examples}
\label{fig:moti_example}
% \vspace{-8pt}
\end{figure}


% Considering that developers may not be motivated, may not have time or simply forget to do so, % (As software evolves and development team re-organize) 
Developers change their source code but forget to remove or update associated TODO comments from time to time. 
Fig~\ref{fig:moti_example} shows two examples of stale TODO comments we found in real-world Github repositories. We can see that:
%\begin{itemize}
 %   \item 
    % When changing the source code to perform TODO task, developers ideally update the associated TODO comments (as shown in Fig.~\ref{}), while it is not uncommon for developers to change code without updating TODO comments, which makes the TODO comments become obsolete.  
    
\textbf{Producing obsolete TODO comments is not only done by inexperienced developers:} Even developers within experienced teams (such as Ethereum and Google) may ignore or neglect such updates. 
For example, Motivating Example 1 presents such an obsolete TODO comment example from the \emph{clusterfuzz} project developed by the Google team. 
The TODO comment within the method \texttt{get\_client\_ip} states that ``\textit{remove include\_strategies once refactor is complete}''. 
However, when the task was resolved and \textit{include\_strategies} was removed from the method, the corresponding TODO comment was not updated.
Until the time we report this issue, this stale TODO comment has existed for over 1 year.
During this time, such a comment may hinder  program comprehension, cause miscommunication between developers, and confuse developers who perform the subsequent development. 
% During the software development, the method was modified and \textit{include\_strategies} was removed from the method accordingly. 
% However, within the same commit, the corresponding TODO comment was not removed, leading to the source code and TODO comments to be out-of-sync. % Although such out-of-date comments do not  
    
%    \item 
\textbf{A lot of software bugs are caused by the mismatch between code's implementation and developer's intention:}  
While a stale TODO comment itself might be harmless, it can mislead developers and cause the introduction of bugs in the future. 
For example, in our Motivating Example 2, the task TODO comment was fulfilled and should not be followed any longer. However, since the TODO comment stayed around, other developers can easily misunderstand the software component and violate the assumption and later lead to bugs. 
    % Moreover, the stale TODO comment will become of ever-decreasing accuracy as software growth and evolves. 
%\end{itemize}

\subsection{User Scenarios}
We illustrate a usage scenario of {\sc TDCleaner} as follows:

\textbf{Without Our Tool:}
Consider a developer Bob. 
Daily, when Bob reads other people's code to perform the development, he encounters a few stale TODO comments. 
These out-of-date TODO comments can clutter the code and have a harmful effect for Bob to understand the current state of the code correctly.
Bob may lose confidence in the reliability of the system and even ignore the remainder of useful comments. 
Furthermore, since Bob has no idea that this TODO comment had already been resolved, Bob tries his best to perform the ``pending'' task with respect to this task comment by refactoring the code. 
However, due to his unfamiliarity with the code or the system, these updates are risky and very likely to cause the introduction of bugs in the future. 

\textbf{With Our Tool:}
Now consider Bob adopts our {\sc TDCleaner}. 
Before working on the software, Bob can use our tool to automatically check for the presence of stale TODO comments.
Moreover, {\sc TDCleaner} can identify the specific code change which resolved the TODO comment, thus helping to improve developer's confidence in verifying the obsolete TODO comments. 
With the help of our tool, Bob successfully removes the stale TODO comments in the current software repository efficiently and accurately, which can increase the reliability and maintenance of the system and decrease the likelihood of introducing bugs. 
 

==> pre.tex <==
% In this section, we will provide some definitions of terms and our research problem definition. Here are the definitions of relevant terms.

\begin{figure}
	\centering
	\includegraphics[width = 0.95\linewidth]{figures/moti.pdf}
	\caption{API Examples Generated by APIzator.}
	\label{fig:pre}
\end{figure}


\subsection{Limitations of APIzator}
Terragni et al.~\cite{terragni2021apization} first introduced the task of APIzation. 
That is, for a given Stack Overflow code snippet without method declaration, convert the code snippet into a functional and compilable API. 
To achieve this, the authors proposed a rule-based approach, namely APIzator, to complete this task automatically. 
They claim APIzator can generate ``\textbf{reusable}'' APIs and 81.5\% generated APIs are identical (either method parameters or return statements) to those produced by humans. 
However, this claim is rather shaky because an API can hardly be claimed as ``\textbf{reusable}'' if it only has correct method parameters or correct return statement, crafting a meaningful API method name is undeniably crucial for ensuring the true reusability of an API. 


In this preliminary study, we perform an in-depth analysis of their experimental results. 
Particularly, the first author of this paper manually examined their released evaluation set, which contains 200 API pairs (one generated by APIzator and the other one by human experts). 
The examiner carefully reviewed each linked Stack Overflow post to determine if the APIzator's generated method names were imprecise and misleading. 
As a result, 92.5\% (185) APIs' method names are not applicable in practice. 
If we redefine the criteria of a ``\textbf{reusable}'' API to include not only identical method parameters and return statements but also meaningful method names, \textbf{
the reusable API ratio of APIzator significantly drops from 81.5\% to 1.5\% (only 3 APIs meet this criteria)}. 

The reason for this phenomenon is that APIzator is a rule-based method, it generates method names by naively extracting \texttt{verb + object} from the question title, which is too simple to cover the complex scenarios in practice, resulting in a large number of misleading and meaningless method names. 
Another limitation of APIzator is that it is specifically designed for handling Java code snippets, its manually designed rules and third-party tools can hardly adapt to other programming languages. 

\subsection{Motivating Examples}
We provide two motivating examples from APIzator evaluation results as shown in Fig.~\ref{fig:pre}. 
In the first motivating example, APIzator generates a method named \texttt{get()} for the Stack Overflow post ``\textit{How to get the last Sunday before current date?}'', the method name of this API is \textbf{unclear and meaningless}, developers who want to reuse this API have to carefully read through the method implementation to figure out what the method does. 
Moreover, the APIzator generated method names can even \textbf{mislead developers to misuse API and potentially lead to the introduction of bugs in future code.} 
For example, in motivating example 2, the APIzator naively extracted the \texttt{verb + object} from the question title (i.e., ``\textit{How to remove leading zeros from alphanumeric text}''), making a method name \texttt{removeZero()}  for this post. 
A developer can easily misuse this API by assuming this method removes all zeros from the input string, however, what this code snippet does is only removing prefixed zeros from a string.  
Overall, after manually examining Terragni et al.~\cite{terragni2021apization} released evaluation dataset, 197 out of 200 APIs can not be reused in practice due to their meaningless or misleading method names and limited method implementations, which motivates us to develop more advanced models for APIzation task. 


% \subsection{Motivating Examples}



% \subsection{Interview with Developers}
% \begin{itemize}
    % \item \textbf{SO page}: 
    % A SO page contains a question post and multiple answer posts, the question post consists of a question title, question description, and a series of tags. Each Q\&A post may contain code snippets.
    
    % \item \textbf{JAVA code snippet}: 
    % A JAVA code snippet refers to some ordered Java source code lines.

    % \item \textbf{JAVA method declaration}: 
    % A JAVA method declaration must include the following six properties: (1) modifiers, setting access permissions (such as public) or other specific functions (such as static); (2) return type, set the return value type (void if none); (3) method name, briefly describing the function of the method; (4) parameter list, describing the input parameters required by the method; (5) throws statement, capturing the checking exceptions that the method may throw (If necessary, it can be ignored); (6) method body, which implements the overall functionality of the method.
    
    % \item \textbf{Well-formed JAVA method declaration}: 
    % A well-formed JAVA method declaration is relative to the definition of a illustrative method declaration. The illustrative method declaration usually does not need input parameters, but directly implements the input parameters in the method body in the form of variables, and usually outputs the results directly in the method body, which leads to the fact that the method can only be used for the current input, with poor reusability. To improve reusability, we have the following definition: The method body of a well-formed JAVA method declaration cannot contain any variables that can be rewritten as input parameters, and the necessary calculation results must be returned as return values based on the method function. A well-formed JAVA method declaration is characterized by its parameter list and return statements, which accurately represent the input and output of the method body. If the parameter list contains input parameters, and the return type is not void, the method can produce distinct outputs based on various inputs.In other words, in a well-formed JAVA method declaration, the method body must not contain any variables or literals that can be replaced with input parameters. This ensures that the method's calculations solely rely on the provided input parameters, and the necessary computation results are returned as return values, aligning with the method's purpose.

    % \item \textbf{Compilable JAVA method declaration}: 
    % A compilable JAVA method declaration refers to the JAVA method declaration without compilation errors.
% \end{itemize}

% This paper primarily focuses on the APIzation task for Java code snippets on SO. However, during the evaluation phase, we confirmed that our approach can be readily adapted to support other programming languages, including statically-typed languages like C++ and dynamically-typed languages like PYTHON. Below, we present the problem definition of the JAVA APIzation task, along with its input and output.
% \begin{itemize}
%     \item \textbf{Problem definition}: 
%     Given a JAVA code snippet and its associated context, generate a compilable and well-formed JAVA method declaration that implements the functionality of the input JAVA code snippet within its method body. This process is defined as the JAVA APIzation.
%     \item \textbf{Input}: 
%     In our scenario, the JAVA code snippet comes from a SO page's answer post, its context includes the question title, the question post, and the answer post where it is located.
%     \item \textbf{Output}: 
%     A compilable and well-formed Java method declaration that implements the functionality of the input JAVA code snippet within its method body.
% \end{itemize}


 







==> ref.tex <==
% comment is important 
% what is todo comment 
% what is the problem with todo comment 
% challeges 
% previous work 

% Ex1. https://github.com/expectocode/telegram-export/commit/d03bc0f2147658779ce14820608a8ba09d36e434
% Ex2. https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% Ex3. https://github.com/Scifabric/pybossa/commit/3264aceb725268775e8659a6e6c9129d6a585939
% Ex3. https://github.com/21dotco/two1-python/commit/57ee38740060fc4cefa0a5be73e835ae866b0658
% Ex4. https://github.com/expectocode/telegram-export/commit/5cc109a9eedaaefe3cb21bff1b0bb6edc46c08a1
% Ex5. https://github.com/expectocode/telegram-export/commit/402c48294e7effa76ceac1e57374ecf03066e1ec
% Ex6. https://github.com/pfultz2/cget/commit/38403914ce74ae2a5c36a9271d802f0b2bf2cdd4
% Ex7. https://github.com/pyelasticsearch/pyelasticsearch/commit/cb0b7e9431f5cb8c9f5fe8a2f5033aad23d2fc01
% Ex8. https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% Ex9. https://github.com/Scifabric/pybossa/commit/d006276e39ef0800bba9775e125ca4cdd08e49b7

% Motivation Examples:
% https://github.com/Shmuma/ptan/commit/66290f1c7150948ce20d7a02302b9072abd2a732
% https://github.com/coderholic/pyradio/commit/714d8a565f928363f6bbe655967d4b45f4a8f053 *
% https://github.com/21dotco/two1-python/commit/9cefc94e6b190ec3b23d913fe6189890ac4ec443 * 
% https://github.com/21dotco/two1-python/commit/3e54ba6bac35a5f86f68ff17d3f3823cb3d1521b 
% https://github.com/21dotco/two1-python/commit/89981585fcbb15d1ade2ce0f8019f6ae581bf964
% https://github.com/expectocode/telegram-export/commit/0096d4bf10af2d1ddc3c77922f13465d8affcceb
% https://github.com/pfultz2/cget/commit/4b303b2d043302a2425c223f92a6a870da140144
% https://github.com/tarmstrong/nbdiff/commit/d1373b6fbc37956ff41bd0a4afcb5e75bc21068f
% https://github.com/carefree0910/carefree-learn/commit/dc6fb7b141ca7e0efee5b5714d5c10bf845c18c6 * 
% https://github.com/concurrencylabs/aws-pricing-tools/commit/c6fa9c90949f5484d65899e2022af47262924a95
% https://github.com/inasafe/inasafe/commit/ac93e7f74784aca456868abe89f11ef9b9c267a6
% https://github.com/inasafe/inasafe/commit/7401878ecfbcf3f8050b7620a22b8816d8fd3a6b
% https://github.com/PaulSec/HQLmap/commit/25e07e122c06b1d9860f0734c686854709b85748
% https://github.com/homebysix/recipe-robot/commit/c4dc8c24e035b298bf867c60f07afbc8d0ea8e0a * 
% https://github.com/facebookresearch/ParlAI/commit/566c34205d5e5ff5f2315c612de6215ae79494ee
% https://github.com/iambus/xunlei-lixian/commit/6f6848617325fb3a44e13ab06855acf11bd24e85
% https://github.com/Kozea/WeasyPrint/commit/5a75887a83848fd471f745fa7b9fe224e0abe68d
% https://github.com/LibreScanner/horus/commit/17846848ff88fca25d90aeb1a7288be2e852f40e
% https://github.com/gorakhargosh/watchdog/commit/a9cafbbd1fb6943201cc6070dd072779612ce4ff **  
% https://github.com/jwlodek/py_cui/commit/5aa3e34162bde2d221c1595bb4a2f0463aebc392 
% https://github.com/dexy/dexy/commit/b59c53c70cd7e1081f11ad191e6fb1712e789a0e
% https://github.com/karlicoss/HPI/commit/c0bbb4eaf2365b43422691718efed64ebdef73c6
% https://github.com/conda-forge/staged-recipes/commit/f84bcd0c528607637c3ceafd865320e69ede129d ** 
% https://github.com/faucetsdn/faucet/commit/65d95d97df7870bd6faf12f569f9389f3d214c33 * 
% https://github.com/matrix-org/synapse/commit/806f380a8b448ce03671f1ce07f7dfcbdc5261e1 * 
% https://github.com/Trusted-AI/adversarial-robustness-toolbox/commit/a335b22ef1eff3eb50aac20d22fd4f80f7c2a912 
% https://github.com/more-itertools/more-itertools/commit/59d3ac2cb8ea91ade585b1131c9c819f0530a359
% https://github.com/ansible/ansible/commit/db83c0e7cdac8e86026eeae5314185c667e6da1c * 
% https://github.com/kpreid/shinysdr/commit/bfa746a501f8ff0e585199ae35d20fd46a1858e2 
% https://github.com/pyscf/pyscf/commit/881478b155984f96eff6850171fab510dca5d26c
% https://github.com/SublimeHaskell/SublimeHaskell/commit/f52236c89ae82d3fbcda5eb0a72ec0a1999a49bb * 
% https://github.com/openstack/nova/commit/e8a2a540e574ca2d242b9c2749c1f285498809e7 ***
% https://github.com/conan-io/conan-center-index/commit/ea6996cf915d5a769296817c0e2f9f73496a04ca
% https://github.com/cupy/cupy/commit/f76269726d70d0aae83555c6266973dafc0aec1e
% https://github.com/matplotlib/matplotlib/commit/6a6f8d9fcc9f93fc209f289d851350e29a82764d ***
% https://github.com/google/TensorNetwork/commit/50849ce792a1dcdf2a445af83125d06a5c25df09
% https://github.com/torrvision/crayon/commit/2e3641505174241f9f478e3d17d645c830d41297
% https://github.com/oppia/oppia/commit/a43d4d4c618f48b49622502387dc48c309219228 * 
% https://github.com/zulip/zulip/commit/478e215acd6552fc994bd82c9d78f68b7df627d5
% https://github.com/bridgecrewio/checkov/commit/fb95ac4f6eca2f2267d56e469b1fe3544eed66ea *
% https://github.com/google/jax/commit/bd14f2343aece428df85808d23cace1ede0b2821
% https://github.com/certbot/certbot/commit/7feab30e72f5b2fa6fbf23017cafdfb474b5ab72
% https://github.com/joeyespo/grip/commit/a66ce7e8048d6d108fc1bf6d8d7c12a83e77059
% https://github.com/pantsbuild/pants/commit/4f2db5291cbdb1a9d1dd1f847859725f14a19edd
% https://github.com/Trusted-AI/adversarial-robustness-toolbox/commit/4408c3e800513a4e7b83cf794d5c9af04d838d3c
% https://github.com/johnnykv/heralding/commit/d168b7e6c449cb0c2824a51c6bac98af2485b07e
% https://github.com/MagicStack/httptools/commit/44050b4dab8a7d93f878fe2964b2aa496f1151a6
% https://github.com/priba/nmp_qc/commit/77cf5a108a2c38509d988bf676131498a4f89f8b
% https://github.com/HyperGAN/HyperGAN/commit/20632411876bebb6d1a91a6347fa9f1f78ca47ea
% https://github.com/uma-pi1/kge/commit/2fa6ba193212f79e461843ba008885d648078d97 * 
% https://github.com/asyml/texar/commit/c0796197d5629f53c065477071bb2e4700230544
% https://github.com/mdn/kuma/commit/68a90af2f1397890700ace7a6954420a6cc2a587
% https://github.com/LonamiWebs/Telethon/commit/795cb989099a940a1bd065f8212f5fe650c2bf18
% https://github.com/ethereum/trinity/commit/f172b7a3671df75bf9faa9fbce16f2a0a72c3499 **
% https://github.com/drscotthawley/panotti/commit/073349264d61750b83d35a7ca1907cd0bfa4291c
% https://github.com/great-expectations/great_expectations/commit/8ad46babfeaeef7482aa8e7f42260ba0559a5d49 * 
% https://github.com/python/mypy/commit/a8d52612f781f72ffb5facca2ab8233705bc343d * 
% https://github.com/ICSec/airpwn-ng/commit/2aaeacaaf3d0e251f31c59250f79a0c616fde3bf 
% https://github.com/freenas/freenas/commit/265c92eb77d389e4590a558ba5cc9d4330b4b7ca * 
% https://github.com/aws/chalice/commit/f24e7520212a9c36a0ce4dbde483e9cb64193f31 * 
% https://github.com/cowrie/cowrie/commit/ee177d5482bed7a8908f742e26bb334408df328e * 
% https://github.com/google/clusterfuzz/commit/055b529c4c8958711c0530637fa901e1b935d53a ****  
% https://github.com/openid/python-openid/commit/3b015fb69b956d4b2bd5d7010d89daaf126e8be8 * 
% https://github.com/rootzoll/raspiblitz/commit/26cad6c6ef5cf908cd9d6bfea5d7e43c1fe2a546
% https://github.com/faucetsdn/faucet/commit/d63df4657883fefcbc43d0d3706a05316853d996
% https://github.com/dimagi/commcare-hq/commit/1f4809db8a98d775c4f7a4d3a032e0960aef38f6 * 
% https://github.com/Fuyukai/Kyoukai/commit/4b53baf7a364256940c7a96170e6c6cf1c63f6af 
% https://github.com/rhinstaller/anaconda/commit/711cbaf3ce41bd8dab899ab76fd3efbb89933b37 * 
% https://github.com/tribe29/checkmk/commit/f2115724f29ece525e88ce7005324e17953e0737 * 

% User Study Examples
% https://github.com/carefree0910/carefree-learn/commit/dc6fb7b141ca7e0efee5b5714d5c10bf845c18c6
% https://github.com/ansible/ansible/commit/db83c0e7cdac8e86026eeae5314185c667e6da1c
% https://github.com/bridgecrewio/checkov/commit/fb95ac4f6eca2f2267d56e469b1fe3544eed66ea (resolved)
% https://github.com/MagicStack/httptools/commit/44050b4dab8a7d93f878fe2964b2aa496f1151a6
% https://github.com/uma-pi1/kge/commit/2fa6ba193212f79e461843ba008885d648078d97
% https://github.com/drscotthawley/panotti/commit/073349264d61750b83d35a7ca1907cd0bfa4291c
% https://github.com/turicas/rows/commit/063eff251c5e013589454672af75c21492693fd2
% https://github.com/thonny/thonny/commit/2ef4d21da1f862f4e1ea464de05f8992bd61e09f
% https://github.com/dcos/dcos/commit/3dc98580365b70d0dd0fd2f29589384e0e922d87
% https://github.com/ctpbee/ctpbee/blob/master/ctpbee/constant.py
% https://github.com/openstack/nova/commit/f86f7ab64360d2294a855f9e770dfd6ac87832e5
% https://github.com/scipy/scipy/commit/0ca705543cda72346f16ff620a4295ae6974243b
% https://github.com/mozilla/MozDef/commit/b8f9aa8d10f0d854c20d1b7805043eed8249008e
% https://github.com/FasterXML/jackson-databind/commit/659408c3f5a0cf7d5cd9e5079ffa1ed828848f2a
% https://github.com/apache/flink/blob/master/flink-streaming-java/src/main/java/org/apache/flink/streaming/runtime/tasks/StreamTask.java
% https://github.com/grpc/grpc-java/commit/bb0c0e53c2e823154e153c240368e078d846af45
% https://github.com/LMAX-Exchange/disruptor/commit/85905a0f48db8a0997eb1a5c0bf5ec878d399345
% 

%undel 
% https://github.com/yt-project/yt/commit/1fcddfcdf042036e848d27bf5510c4cd41d370e2
% https://github.com/Azure/azure-cli/commit/6f28feb63eae5d9d9764ed98381f2f516dbcd66d
% https://github.com/milesrichardson/ParsePy/commit/7f651474398fc77de4313a0b8668401ab2fb7119
% https://github.com/netenglabs/suzieq/blob/master/tests/utilities/update_sqcmds.py
% https://github.com/netenglabs/suzieq/commit/ea68fd9f0fba9973b2b8d700c7d6087de77f3741
% 

% \subsection{Qualitative Analysis}
% https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% https://github.com/1200wd/bitcoinlib/commit/307660c6f9521324cb75fa11c04654439aa40da8
% https://github.com/inasafe/inasafe/commit/5ca100c6752b53e6bad1f9af8f0d7a1e466b71f5 (introduction)
% https://github.com/1200wd/bitcoinlib/commit/355c1e1c513d39a00c229edda18809d266deebb3
% https://github.com/trufont/trufont/commit/ab1e70f2b2543c60259b7be127f70d062c51d0cb
% https://github.com/trufont/trufont/commit/772a09ae5e0b03595be92e9313223134cbcdfe4b
% https://github.com/imagej/imagej/commit/bb2e21c3fb7bf5539baa8bc6acfeb43f8429bccc
% https://github.com/imagej/imagej/commit/f14486df058a95bde62241f80c599ed880010b3c
% https://github.com/imagej/imagej/commit/473dd7e544aad9cb716fb0a6d5f57fa4676d30fa
% https://github.com/imagej/imagej/commit/4699b04efeda49273820815b5d506a33f4ed654d
% https://github.com/spring-projects/spring-batch/commit/d60c726121cd8906c71c5c7e5ade83310816f259
% https://github.com/spring-projects/spring-batch/commit/459f7d575db7b4899ab28336775c511d1e6938d9
% https://github.com/spring-projects/spring-batch/commit/394de964e1f6647309c3b6da7f280929584b0fe0
% https://github.com/spring-projects/spring-batch/commit/843ecf40d20c1a30a465e7b1c10d514824c5860f ****
% https://github.com/AndlyticsProject/andlytics/commit/90cd58c860039c6f463237abcf82867ccdb301e3
% https://github.com/davidmoten/rxjava2-jdbc/commit/65d12c09cffaaf0f5d44cc4907e9c50e16780e2c *** (introduction
% https://github.com/haiwen/seadroid/commit/ffcb11b113dc3a4ca0863df70d14d8764c5fb2be)
% https://github.com/imagej/imagej/commit/f2e46c27441db906788155b687e6f8cde3f2b7b3
% https://github.com/imagej/imagej/commit/844df0e1f36fde635531af7a4a908ad7e60f24c7
% https://github.com/imagej/imagej/commit/6bad6a89acedd2ee695d811a3b29b45f30f28660
% https://github.com/21dotco/two1-python/commit/3e54ba6bac35a5f86f68ff17d3f3823cb3d1521b ***

% https://github.com/pyelasticsearch/pyelasticsearch/commit/ecdd1900e9311eab2f32a431f97df8ea66e6080e
% https://github.com/pyelasticsearch/pyelasticsearch/commit/a3f57d729b8631e7b6c2fe55e10455f2bcc4b581
% https://github.com/Scifabric/pybossa/commit/af7530291f745f715fc445e177faf2afb8dc0633
% drop: https://github.com/Scifabric/pybossa/commit/7845f058c599ce7e26c6b14f3f601041cc24de79
% https://github.com/Games-and-Simulations/sc-docker/commit/33da40b1aab0dc23df7483ab7f0f6efd62eb8757
% https://github.com/timdouglas/sublime-less2css/commit/90f08ea5648d21b8c26971038bfa1fa45a4cc78d
% ??? : https://github.com/carefree0910/carefree-learn/commit/255bf8b754b1b61a2a873c080d0b1788879eca79 
% https://github.com/1200wd/bitcoinlib/commit/5fdbb8f900671fc86d2715027b4017e3b1e5cee5
% case study: https://github.com/1200wd/bitcoinlib/commit/7220d86a2f752594215555064d9dabada7f7e16a
% https://github.com/1200wd/bitcoinlib/commit/0823e9934c405c1233a322aaaf22f3f655eb32b9
% https://github.com/1200wd/bitcoinlib/commit/93d9292b25704a34e5ccf7f2c0d561d391bda2f5
% case study: https://github.com/1200wd/bitcoinlib/commit/f7915de68a0d7401c32f1fa6211f95664e6390d5
% https://github.com/1200wd/bitcoinlib/commit/f5585da0537ec97cb0b2b005fdcf9ed3913face3
% https://github.com/1200wd/bitcoinlib/commit/81948a4dfcb027e88ade92885bb8a180edb52868
% https://github.com/1200wd/bitcoinlib/commit/df11967a000074310f0acb6412ca37cb9189c0b6
% https://github.com/1200wd/bitcoinlib/commit/92fdb13082624e13536d125bd31c8728adcf1995
% https://github.com/1200wd/bitcoinlib/commit/f446fcd660551f0104cf920533526e17b3e32942
% https://github.com/1200wd/bitcoinlib/commit/307660c6f9521324cb75fa11c04654439aa40da8
% https://github.com/1200wd/bitcoinlib/commit/ac62287328336dacc4124c333547e949b92e20e1
% https://github.com/1200wd/bitcoinlib/commit/2edc7fabdc4701328798dc338da4dbeababae765
% https://github.com/webcompat/webcompat.com/commit/c47bcd9b23a1435e31ab49cad0076f5c6181cc7f
% https://github.com/webcompat/webcompat.com/commit/90f5b05945b3b501da6ffcd8301f9342d3bd7f4b
% https://github.com/webcompat/webcompat.com/commit/8457d9ee32bfd9705753f93e9c25dff61351c328
% https://github.com/webcompat/webcompat.com/commit/1a434ffa2cba09b594ac9bda0e1120927da6909b
% https://github.com/webcompat/webcompat.com/commit/eb0cf1c65e10d701308795955eba81e0c403c448
% https://github.com/aromanovich/jsl/commit/a28bee7d057c58810e84b1ea0072f8be2e5ece50
% https://github.com/wordnik/wordnik-python/commit/d0b4fdd9ef61b33a01eff250faee585f5180bb18
% https://github.com/inasafe/inasafe/commit/0227aeaa55c908dd6d81186c3da11baa61fefc6f
% case study: https://github.com/inasafe/inasafe/commit/5ca100c6752b53e6bad1f9af8f0d7a1e466b71f5
% https://github.com/mozilla/foundation.mozilla.org/commit/4ba7516ce7dc74932d40e3ee4d7048a7d4ce1f5c

% Java
% https://github.com/imagej/imagej/commit/ccd67d8d5a55d5674813055a7960fea4bef60b7d
% https://github.com/imagej/imagej/commit/d152ca154cd97067b38bd7a7779c6023e0247d98
% case study: https://github.com/imagej/imagej/commit/8513b489511ff3489b8ccba357b524c5f30d2b6c
% https://github.com/imagej/imagej/commit/a565c5550d0f992b3de0109bf968610a1885f753
% https://github.com/imagej/imagej/commit/3fbd192033119dbe41635e734416d90d26c5bbd2
% https://github.com/imagej/imagej/commit/1777d31b29a554d9b06375afebaab51c6d22e2a0
% https://github.com/shiffman/Most-Pixels-Ever-Processing/commit/2618da39b120e3cce7240d9eb88a63decb4359f4
% case study: https://github.com/marverenic/Jockey/commit/3b7c6b5feb38dffcfabf03f25ffbfff0371e0fe4
% https://github.com/marverenic/Jockey/commit/93d7a9692aec6e6af847a35321750b0f99df18d2
% https://github.com/marverenic/Jockey/commit/647e6d304cced39b7dc18f6195f3258659f72e00
% https://github.com/pf4j/pf4j/commit/f4ddddc61b8643bf4e34ce65b4de9bf2d2bd6831
% 

===========================================


manual determination of a fault's root cause can consume 30 to 40 percent of the total time needed to fix a problem. 
For example, imagine you must compare a log against a libraray of reference logs to identify a recurring defect. 
If the library contains 1 Pbyte of logs, simply reading these logs into memory for the purpose of comparison will take signi

\textit{\textbf{Dealing with information overload.}}
As logs are too large to examine manually and too unstructured to analyze automatically. 
Instead of asking users to search, we provide tools to automatically find ``interesting'' log messages. 
Our goal is to find the ``needles in the haystack'' that might indicate operational problems, without any manual input. 
Modern software systems have become so large and complex that they produce too huge amounts of log data for software engineers to handle manually. 
The logs contain an overwhelming amount of detailed information. 
Moreover, since the lack of knowledge about the bug or missing the context information of the specific bugs, this process is often error prone. 
We convert a log message from unstructured text to data structure that shows the message type and a list of message variables in (name, value) pairs. 

\textit{\textbf{Dealing with imbalanced dataset.}}


\textit{\textbf{Dealing with increased latency.}}
% \begin{itemize}
%     \item \textit{Logs are often too large to examine manually and too unstructured to analyze automatically.} 
%     \item \textit{Low latency.}
%     \item \textit{Data Imbalanced.}
% \end{itemize}
% manually analyzing the logs becomes inefficient. 
% To get the attention of the suitable developers on the bugs quickly, it is essential to assign failed test case to the right reason, so that the developers have the expertise can review, analyze and fix the bugs as quickly as possible. 
% many software failures rely on the different runtime environment which can not be easily reproduced, 


Challenges: 
In order to figure out the causes, testers have to carefully read test logs, each of which may consist of hundreds of test steps and thousands of log lines of text. 
Considering the fact that fact that thousands of test alarms may be produced per day for a production line with several similar products, as we have observed ... 
test alarm cause analysis lays an almost unbearable burden on testers and has become a bottleneck in SIT. 
Realizing the urgent need to alleviate the burden of cause analysis, our collaborators manually build regular expressions over the test logs to analyze test alarm causes. 
The accuracy of their approach is about 20\% - 30\% on different projects. 


However, diagnosing problem causes in software systems bring new challenges for both developers and system operators. One significant problem is that as the system scales, the amount of information operators need to process goes far beyond the level that can be handled manually, and thus there is a huge demand for automatic processing and monitoring data. 



% Any software system can fail, leading to its degraded quality in terms of performance, reliability, or security. 
Finding the failure causes of the software problems is a nontrivial task ... 
To pinpoint a problem's root causes, testers typically examine operational data - logs and traces - generated by the software systems. 
% Importance and Benefits of Test Log analysis 


% Current Approaches and Challenges 

A fundamental activity to achieve software quality is software testing, whose results are typically stored in log files. 
These files contain the richest and more detailed source of information for developers trying to understand failures and identify their potential causes. 
Analyzing and understanding information in log files, however, can be a complex task, depending on the amount of errors and the variety information. 
This paper presents ASTRO, an infrastructure that extracts information from a number of log files that aim at easing and improving the developer's analysis process. 

To determine if the developed software product meets its specifications and works correctly in the environment for which it was designed, developers resort to software testing, whose overall goal is to increase the reliability of a program by checking whether it presents execution errors and revealing them for proper fixing. 

The latter step deserves special attention, since it is the communication point between software testers and the other stackholders. 

Software testing tools usually produce (or can be configured to produce) auxiliary test files known as log files, i.e., documents that contain descriptive execution details of one or more test procedures, comprising data on their actual execution status, in chronological order. 

The information reported in log files is considered by developers as the most important and useful resource to monitor software quality and highlight features, easing debugging process. 
Such files usually describe a test description (if applicable), the test duration, errors identified in the test execution, incident statuses, context information, among others. 

However, due to their rich and detailed information, many log files are large, with a complex structure, making the understanding of their information a challenge task. As the volume of data gets larger, analyzing their contents becomes inefficient, hampering developers in properly understanding failures and their causes. 

This work parts from the assumption that the collection and abstraction of information from log files can ease and speed up the identification of problems identified in test executions. 

log files have the main information about a particular test that was run, but such files can have a complex structure with large volumes of data, hampering the understanding of its information and making its analysis a time-consuming, difficult, and challenging task. 
A log file lists the problems that occurred within a program execution, which may end up not being verified and remain hidden if the log file are not properly handled. 

In an attempt to reduce the number of delivered errors, it is estimated that most companies spend between 50\% - 80\% of their software development effort on testing. 
Besides, locating the errors can be considered as one of the most difficult development task. 
Some techniques can be of great help to reduce the time needed for identifying problems. 
The reducing of this location time can have a significant impact on cost and quality of software development and maintenance. 
Stack traces of the test cases execution are stored in textual format, and their analysis is done after the test case execution. 
These files contain the most important information about the tests performed, so they can not be left aside, and it is necessary to have a good understanding of them. 

Although log files are used mainly for analyzing errors and their causes, they can provide interesting insights in software development.
For instance, combining their information with the information provided by other resources (e.g., version control or issue tracking system), it is possible to assess if tests are being performed according to the plan or schedule, identify which errors are introduced more frequently (providing clues on software development topics that may need more training), reveal team configurations that are more or less error-prone etc.  

========================================

Test automation simplifies the debugging work by providing a detailed, unambiguous log of activities and intermediate test steps. 
This leads to a more organized, structured, and reproducible testing approach. 
Automated execution of test cases reduces the elapsed time for testing, and, thus, it leads to a shorter time to market. 
In short, automation increases the test execution efficiency. However, at the end of test execution, it is important to analyze the test results to determine the number of test cases that passed and failed. 
And, if a test case failed, one analyzes the reasons for its failure. 
In the long run, test automation is cost-effective. It drastically reduces the software maintenance cost. 


========================================

Mistakes and introduced defects occur and may be largely unavoidable. 
Software testing should focus on providing information about a software product and finding as many defects as possible, as early as possible in the development process, under given constraints of cost and schedule. 

Dynamic test execution is a risk mitigation activity. 
Running test cases mitigates risk because if the test passes then the likelihood of the risk occurring is normally lower - and so the risk score is reduced.
Similarly, if the test fails, the risk may increase.
The process of test incident reporting would then be used to determine if the failed test case had resulted in an issue or if it required further investigation. 

========================================

Log files are often very large and can have complex structure. 
Although the process of generating log file is quite simple and straightforward, log file analysis could be a tremendous task that requires enormous computational resources, long time and sophisticated procedures. 
It is useful to research in the field of log files analysis and to design an open, very flexible modular tool, that would be capable of analyze almost any log file and answer any questions, including very complex ones. 
Such analyzer should be programmable, extendable, efficient (because of the volume of log files) and easy to use for end users. 
(1) The log file is an auxiliary output file, distinct from other outputs of the program. Almost all log files are plain text files.
(2) Each record (i.e., a line or a group of lines) in a log file is caused by a given event in the program, like user interaction, function call, input or output procedure etc. 
(3) Records in log files are often parametrized, i.e., they show current values of variables, return values of function calls or any other state information. 
(4) The information reported in log files is the information that programmers consider important or useful for program monitoring and/or locating faults. 

========================================

Large programs or software systems often keep what are called "log files", continuous reports of events that have occurred during the running of the program. 
These log files are typically used for debugging, fault location in production software, regression testing, or administrative information. 

========================================

is a kind of output file generally referred to as a debug file or log file. Such a file records events such as inputs and outputs, values of variables, and parameters of returns of function calls, sequentially as the program is running. 
Programmers inspect log files to identify and diagnose problems in code. We refer to this practice as log file analysis. 

the enormous amount of data collected at run-time gives rise to scalability issues. 
Due to vast amounts of information, it is a very difficult task to successfully navigate through the dynamic data contained in execution traces without getting lost. 




We analyze the the failure reporting capability of event logs collected at different levels of an industrial system. 
For example, even if operating systems logs catch almost all application crashes, they are strongly ineffective in face of silent and erratic failures in the considered system. 

Event logs play an important role in data-driven failure analysis because they contain a large amount of textual information about system behaviour under real workload conditions. 
Understanding system failures through event logs is an important activity in many types of systems, to avoid severe consequences such data and economical loss, damage to the environment. 
Due to unforeseen components interactions or wrong execution of operations process. 
event logs may be inaccurate to obtain information on software failures and their causes. 
Our study provides strong insights into the reporting ability of event logs as affected by the type of faults and failures induced in the system. 
A fault can be achieved by a specific sequence of input, environmental conditions, etc. Activation causes one or more errors, which can propagate in the system and may cause a failure. 


Software failure analysis techniques are valuable to developers: for example, they allow to understand system failure modes, establish the cause of failures, prevent their occurrence, and improve the dependability of future system releases. 

Logs are used for a variety of purposes, such as debugging, configuration handling, access control, monitoring and profiling. 

reported errors, although being useful when logs are used for other purposes, may be misinterpreted as false failure indications, if not supported by a detailed knowledge of the system. 
The focus of this paper is on the use of log event logs to support accurate failure analysis: 

This is especially true in the case of software faults, which are among the main causes of system failures. 
The ambition of this work is to fill the gap in the knowledge about the ability of logs to report software failures and to propose a novel logging approach, named rule-based logging, achieving effective failure detection. 

% Test Log Overview 
The test logs provides a detailed, typically time-based record that serves both as verification that a set of tests were executed, and provides information relating to the success of those tests. 
The focus is typically on the provision of an accurate audit trail, enabling post-execution diagnosis of failures to be undertaken.
This raw data will subsequently be analyzed to help determine the results of some aspect of the test effort.
A test Log usually representing the output resulting from the execution of a Test Suite for a single test cycle run.
Typically, Test Logs have a tabular or spreadsheet-like appearance, with each entry comprising some form of date and time stamp, a description of the event logged, some indication the observed status, and possibly some additional contextual information. 

The test log contains a historical record of events that occurred during a test run or a schedule run, as well as the status of each verification point.
The test log sets a verdict for each run as follows:
(i) Pass indicates that all verification points matched and received the expected response and all the test steps successfully completed. 
(ii) Fail indicates that at lease one did not match the expected response or that the expected response was not received or a Web UI step did not run successfully.
Test log collects raw output captured during a unique execution of one or more tests for a single test cycle run.

This artifact provides a detailed, typically time-based record that serves both as verification that a set of tests were executed, and provides information relating to the success of those tests. The focus is creating an accurate record, which enables a post-execution diagnosis of test results. This raw data will subsequently be analyzed to help determine the results of some aspect of the test effort.
Since this is a collection of raw data for subsequent analysis, it can be represented in a number of ways.
(i) For manual tests, log the actual results on a copy of the manual Test Script 
(ii) For automated tests, direct the output to log files that you can trace back to the automated Test Script
(iii) Track raw results data in a test management tool.

While testing is a critical part of a good continuous delivery pipeline, most people don’t want to sift through thousands of lines of console output to find information about failing tests. To make this easier, Jenkins can record and aggregate test results so long as your test runner can output test result files. 
When there are test failures, it is often useful to grab built artifacts from Jenkins for local analysis and investigation.

Test Artifacts are simply integral part of software testing. These are generally set of documents, which software project tester gets during STLC (Software Testing Life Cycle). Test artifacts are by-products that are generated or created while performing software testing. These generated test artifacts are then shared with clients and testing team or team managers, team leaders, stakeholders associated with project, and also with members of other team.

Test case formats may vary from one organization to another. 
as the volume of your tests goes on increasing, you will find it extremely difficult to manage.
Status (Pass/Fail): If the actual result is not as per the expected result, then mark this test as failed. Otherwise, update it as passed.

Finally set the status as Pass or Fail based on the expected result against the actual result. If the actual and expected results are the same, mention it as Passed. Else make it as Failed. If a test fails, it has to go through the bug life cycle to be fixed.

The different states of a bug in the software bug life cycle (sblc) are as follows:
(i) New. When a tester finds a new defect. He should provide a proper Defect document to the Development team to reproduce and fix the defect. In this state, the status of the defect posted by the tester is “New”.
(ii) Assigned. Defects that are in the status of New will be approved (if valid) and assigned to the development team by Test Lead/Project Lead/Project Manager. Once the defect is assigned then the status of the bug changes to “Assigned”

using a test case can help you identify any issues with software features before you roll them out.
Even just the process of running a functional test case can bring up current errors in your software, so the template can accelerate the diagnosis and help you narrow down a simple ‘pass or fail’ response.


43 Test Case Templates / Examples from TOP Software Companies
When developing software, one of the most important objectives is to minimize the number of bugs for the end-product. Although most bugs are usually removed during the alpha and beta phases of software, it is important that you test it through the entire building phase.
The most effective way to do this is to get a tester who will run the entire program and reported anything unusual back, but there is a lot more to it than that.


(i) Troubleshooting distributed, scalable systems (often composed of volatile infrastructure) depends on adequate logging and search facilities (ii) Techniques such as unique event IDs, transaction tracing, and structured log output, give us visibility into application behaviour and health.
Particularly in the context of distributed systems, cloud, and IoT, we need to consider the time it takes to restore service (often termed 'Mean Time to Recovery', or MTTR) following a failure, as well as the time it takes to determine the cause of problems in upstream (testing) environments.
Although additional logging may result in a 5-10 percent drop in raw runtime execution speed, the detailed information available in a single searchable location helps us to diagnose problems much more quickly, speeding up our incident response and often significantly reducing the time to find that awkward bug!
Events that we expect to occur appear correctly in the log stream.


Test log, a sort of test artifact, is made during test execution and gives detailed data with respect to the achievement of each test performed to approve the quality, functionality, and performance of the product. 
A test log is not just a tested output. Minimal pass/fail output may log the aftereffects of testing, however, a genuine testing log should accomplish more than that. At least, it should log the fundamentals of the testing procedure itself, including test documents utilized, specific test steps as they are performed, and any output messages or flags, with timestamps for every one of these things. In a perfect world, it should likewise log key procedures and factors demonstrating the condition of the framework previously, during, and after the test.

Different segments incorporated into a test log are:
(i) It should incorporate the date and time of when the failure, event or some other significant issue happened.
(ii) Offer a concise depiction of the event logged.
(iii) There should be some sign of the status of different occasions seen by the team.
(iv) Also, additional contextual details and data should be given, any place required and significant.
(v) Give details identified with any errors and anomalies recognized.

Importance of Test logs:
(1) Finding issues with the test procedure itself.
(2) As an aide to standard debugging tools.
(3) Finding discontinuous or difficult-to-follow issues.
(4) Recognizing regression and tracking the historical backdrop of firmly related errors
A detailed testing log may enable you to spot key differences and similarities in the framework state during and after the test, making it conceivable to recognize an old bug and a new however comparable one. Testing log data may likewise be useful in distinguishing a related group of mistakes, in view of how they influence the condition of the system.
From the above discussion, we can infer that the test log report is critical for approving the quality and adequacy of testing. It gives pertinent and precise information that enables the team to test different parts of the product and investigate their product application completely. Henceforth, by making test logs at whatever point test are executed or test scripts are actualized, the team can improve the viability of the product.


The log files provide the information to identify what the errors are, and through the information in the log, infer what to investigate to solve the problem.

IEEE 829 Definition for Test Log:  “To provide a chronological record of relevant details about the execution of tests, e.g. recording which tests cases were run, who ran them, in what order, and whether each test passed or failed.”

Log analysis is one of the most important aspects of performing effective and efficient software testing. End-to-end functionalities and user interfaces may look right but a QA can never be sure about the product until they make sure that there are no errors or exceptions or something unexpected in the application logs.

We at Fleek, make sure that we go through each and every log file generated by our applications and supporting components and analyze the possibility of any hidden bugs or issues that can only be revealed by examining logs thoroughly. One should possess a high understanding of product and technologies used in order to examine the logs effectively.

important points while reviewing the logs.
1. Make sure that logs are writing only meaningful details, otherwise, logs will lose their usefulness.
2. Errors or exceptions must be captured with a full stack trace which can help in understanding and troubleshooting.
3. Details in the log files should have correct levels like the error, warning or info. If these levels are not defined correctly then logs may mislead the troubleshooting process.
4. Log file must NOT have any sensitive information. The sensitivity of data can be defined based upon the nature of the application business. However, there must be strict guidelines on what data need to be captured in the logs.
5. Every log entry must have a timestamp associated with it. The timestamp would be handy to deep dive the investigation on any production incident.
6. Make sure logging is not impacting the performance of the application in any scenario.

log analysis can help in the QA process. 
1. It helps in analyzing the production issues and identifying a possible root cause of the defect. This will help in improving your test plan and reproducing production issues on your QA environments.
2. If you attach the correct log details along with your defect then it would reduce at least 50 of the developer effort in reproducing the defect and fixing it.
3. Effective log analysis will always help you during integration testing and reporting quality defects. During integration testing, it is very important to identify the problematic component. If you are good at reading the log files and analyzing the error/exception then it makes things quicker in finding the exact root cause.
4. Sometimes QA comes across a defect which is not always reproducible and QA seems unable to find the exact pattern or steps which could reproduce a defect. In such cases, application logs can come to the rescue and could help QA to better understand what is causing the defect. QA can easily determine the exact scenario to reproduce defect by analyzing the logs.

Logs are lists of lines of text output from an application in a given environment, such as a test server or production server. They can be helpful for testing purposes because they provide real feedback and insight into an application as it’s being used, as well as information that describes or can even help solve bugs.

Each line of a log corresponds to some event or occurrence in the application. A log line could be informational ("A user successfully logged in at "1:00 PM EST"), a warning ("The current number of users is 90 percent of the total allowed concurrent users"), or an error ("A valid user login failed unexpectedly"). Log entries can be output from the application itself ("The number of logged-in users at a given time has reached a hard-coded limit") or from the application's environment or the system running the application ("The server has run out of memory and cannot allow any more users to log in"). Most logging systems provide a timestamp for each log entry, often to the millisecond, and each log entry follows some standard format. 


Due to the nature of load testing however, the volume of data produced during long (e.g. 7 day) test runs or during stress tests can be enormous and very difficult to properly analyze without the correct tools.
Logentries was designed to take large volumes of log data and very quickly identify if that data contained errors, exceptions, warnings etc. so that test teams could quickly understand system behavior during test runs. 


And log analysis can be used beyond developers and IT operations – to benefit Quality Assurance (QA) teams in the process.




The rest of the paper is organized as follows.
Section~\ref{sec:moti} presents the motivating examples and user scenarios of our study. 
Section~\ref{sec:approach} presents the details of our approach.
Section~\ref{sec:data} presents the data preparation for our approach. 
Section~\ref{sec:eval} presents the baseline methods , the evaluation metrics, and the evaluation results.
Section~\ref{sec:dis} presents the in-the-wild evaluation.
Section~\ref{sec:threats} presents the threats to validity. 
Section~\ref{sec:related} presents the related work.
Section~\ref{sec:con} concludes the paper with possible future work. 


==> related.tex <==
In this section, we present the prior research that is related to this paper.
\subsection{Code generation and API calls generation}
Code generation~\cite{fried2022incoder,feng2020codebert,clement2020pymt5,lu2021codexglue,jiang2023selfevolve,zheng2023codegeex}, a significant area in the field of software engineering and programming, has been the subject of numerous studies and research. The goal of this task is to transform a given natural language description into the required code snippet. With the emergence of the code pre-training model CodeBERT~\cite{feng2020codebert}, more and more work is attempting to solve the code generation task using pre-training methods. For example, Clement et al.~\cite{clement2020pymt5} proposed PYMT5 to complete the task of converting Python methods and method document strings, while Lu et al.~\cite{lu2021codexglue} proposed CodeGPT to generate member functions and member variables in Java classes. Unlike them, the input for the code APIzation task includes not only the natural language description but also the code snippet used to generate the API, so the model needs to consider the code snippet itself to generate the corresponding API. 

Another task related to code APIzation is the generation of API calls~\cite{gu2016deep,huang2018api,zhang2023toolcoder,wei2022clear,wang2023measuring,patil2023gorilla}, which aims to help developers search or generate suitable API calls, and is of great significance to the software development process. The goal of this task is to generate a call to an existing API (i.e., the method name and corresponding parameter list) based on a natural language description. In recent years, Wei et al.~\cite{wei2022clear} proposed CLEAR, which can recommend reasonable API calls without parameter lists from Stack Overflow to users based on their questions, while Wang et at.~\cite{wang2023measuring} and Patil et al.~\cite{patil2023gorilla} used generative models to generate API calls from natural language descriptions respectively. Unlike them, our task is to generate user-defined APIs, which not only need to generate the method name and parameter list, but also the corresponding method body, making it more complex.

\subsection{Large Language Models for Software Engineering}
Large language models(LLMs)~\cite{zhao2023survey,wang2023software,wang2021codet5,touvron2023llama,wang2022self,chowdhery2022palm} have been increasingly utilized in the field of software engineering, demonstrating significant potential in various applications. There are typically two ways to apply LLMs to specific downstream tasks. One is to use the fine-tuning method to adapt the model to the downstream task. For example, Codex~\cite{chen2021evaluating} fine-tuned GPT3~\cite{brown2020language} using Python data collected from Github, and the fine-tuned model can generate Python functions based on function documentation. Thapa et al.~\cite{thapa2022transformer} fine-tuned models like Bert~\cite{devlin2018bert} and GPT2~\cite{radford2019language} to solve software vulnerability detection tasks. Although the fine-tuning method has achieved exciting results in various software engineering tasks, it requires the construction of downstream task datasets and the use of high-performance hardware devices to fine-tune the model, which are both costly and time-consuming. 

Another method of using LLMs is Prompt Engineering~\cite{liu2023pre,feng2023prompting}. This method designs specific prompts to elicit the knowledge in large models used to solve corresponding downstream tasks. Current prompts are mainly divided into two types, hard prompts~\cite{schick2020exploiting,gao2020making,shin2020autoprompt,jiang2020can} and soft prompts~\cite{li2021prefix,han2022ptr,liu2023gpt}. Hard prompts consist of manually defined natural language. A carefully designed hard prompt can guide the large model to complete the corresponding downstream task well without any fine-tuning, effectively avoiding the problems faced by the fine-tuning method. Soft prompts introduce learnable virtual tokens into hard prompts, although they can further improve model performance, they also require data to fine-tune the model. Therefore, this paper focuses on hard prompts. Hard prompts have been used to solve various software engineering tasks, including program repair~\cite{paulenhancing,huang2023chain}, code generation~\cite{dong2023self,tan2023copilot}, test case generation~\cite{siddiq2023exploring,xie2023chatunitest}, etc. Recently, Bareiss et al.~\cite{bareiss2022code} designed specific prompts to guide Codex to solve tasks such as test case generation. Li et al.~\cite{li2023codeie} proposed CodeIE, which transformed information retrieval tasks into code generation tasks and designed corresponding prompts to guide Codex to solve these tasks. To our knowledge, Code2API is the first model to use hard prompts to guide LLMs to solve the code APIzation task.








==> sum.tex <==
We demonstrate {\sc Code2Que}, a web-based tool for improving low-quality question titles in Stack Overflow. 
Developers copy and paste their code snippets into our web application. {\sc Code2Que} automatically generates question titles for the code snippets via a deep sequence-to-sequence model. Developers can utilize the generated questions for their posts. {\sc Code2Que} also searches for related questions with similar problematic code snippets to help developers better understand their problems. Human evaluation results show that for a large number of low-quality questions in Stack Overflow, {\sc Code2Que} can improve the quality of the question titles in terms of \emph{Clearness}, \emph{Fitness}, and \emph{Willingness}. In future work, we will design better models to generate question titles by considering more context information. 

==> threat.tex <==
Several threats to validity are related to our research: 

\noindent\textbf{Threats to internal validity.} 
One threat to internal validity is that the design of prompts can be diverse. For instance, the selection of examples in few-shot learning and the choice of CoTs in chain-of-thought reasoning can both influence model results. While our current prompt may not necessarily be optimal, they have already performed well in the code APIzation task. In the future, we will investigate methods to automatically design high-quality prompts for accomplishing corresponding tasks. 
Another threat is the instability of ChatGPT's output. To reduce the uncertainty of the model's output, we set the corresponding temperature parameter to 0. Nevertheless, the model still has slight instability, which is determined by the implementation of ChatGPT.

\noindent\textbf{Threats to external validity.} 
One threat to external validity is that Code2API is unable to generate APIs for long question-answer posts, as Chatgpt has a maximum input length of 4096 tokens. Considering Chatgpt's support for conversational Q\&A, one potential solution is to employ multi-turn questioning to extract summaries of the question-answer posts in order to reduce their length. These extracted summaries can then be used to replace the original question-answer posts for the APIization task.

\noindent\textbf{Threats to construct validity.} 
One threat to construct validity is that the evaluation of method names in RQ-2 involves a certain degree of subjectivity. However, there is currently no better approach to assess method names. To mitigate this subjectivity, we recruited multiple volunteers with extensive Java programming experience to evaluate the method names.
